Universes without the Weak Force: Astrophysical Processes with Stable Neutrons

We investigate a class of universes in which the weak interaction is not in operation. We consider how astrophysical processes are altered in the absence of weak forces, including Big Bang Nucleosynthesis (BBN), galaxy formation, molecular cloud assembly, star formation, and stellar evolution. Without weak interactions, neutrons no longer decay, and the universe emerges from its early epochs with a mixture of protons, neutrons, deuterium, and helium. The baryon-to-photon ratio must be smaller than the canonical value in our universe to allow free nucleons to survive the BBN epoch without being incorporated into heavier nuclei. At later times, the free neutrons readily combine with protons to make deuterium in sufficiently dense parts of the interstellar medium, and provide a power source before they are incorporated into stars. Almost all of the neutrons are incorporated into deuterium nuclei before stars are formed. As a result, stellar evolution proceeds primarily through strong interactions, with deuterium first burning into helium, and then helium fusing into carbon. Low-mass deuterium-burning stars can be long-lived, and higher mass stars can synthesize the heavier elements necessary for life. Although somewhat different from our own, such universes remain potentially habitable.

==> master <==
@Article{Pudliner:1995wk,
     author    = "Pudliner, B. S. and Pandharipande, V. R. and Carlson, J.
                  and Wiringa, R. B.",
     title     = "Quantum Monte Carlo calculations of $A \leq 6$ nuclei",
     journal   = "Phys. Rev. Lett.",
     volume    = "74",
     year      = "1995",
     pages     = "4396-4399",
     SLACcitation  = "%%CITATION = PRLTA,74,4396;%%"
}
@Article{Nakano:2003qx,
     author    = "Nakano, T. and others",
 collaboration = "LEPS",
     title     = "Observation of S = +1 baryon resonance in photo-production
                  from  neutron",
     journal   = "Phys. Rev. Lett.",
     volume    = "91",
     year      = "2003",
     pages     = "012002",
     SLACcitation  = "%%CITATION = HEP-EX 0301020;%%"
}
@Article{Barth:2003es,
     author    = "Barth, J. and others",
 collaboration = "SAPHIR",
     title     = "Observation of the positive-strangeness pentaquark Theta+
                  in  photoproduction with the SAPHIR detector at ELSA",
     journal   = "Phys. Lett.",
     volume    = "B572",
     year      = "2003",
     pages     = "127-132",
     SLACcitation  = "%%CITATION = HEP-EX 0307083;%%"
}
@Article{Klein:1998xy,
     author    = "Klein, F. J.",
 collaboration = "SAPHIR",
     title     = "{Overview of vector meson photoproduction}",
     journal   = "PiN Newslett.",
     volume    = "14",
     year      = "1998",
     pages     = "141-149",
     SLACcitation  = "%%CITATION = 00076,14,141;%%"
}
@Article{Stepanyan:2003qr,
     author    = "Stepanyan, S. and others",
 collaboration = "CLAS",
     title     = "Observation of an exotic S = +1 baryon in exclusive
                  photoproduction  from the deuteron",
     journal   = "Phys. Rev. Lett.",
     volume    = "91",
     year      = "2003",
     pages     = "252001",
     SLACcitation  = "%%CITATION = HEP-EX 0307018;%%"
}
@Article{Kubarovsky:2003fi,
     author    = "Kubarovsky, V. and others",
 collaboration = "CLAS",
     title     = "Observation of an exotic baryon with S = +1 in
                  photoproduction from the  proton",
     journal   = "Phys. Rev. Lett.",
     volume    = "92",
     year      = "2004",
     pages     = "032001",
     SLACcitation  = "%%CITATION = HEP-EX 0311046;%%"
}
@Article{Barmin:2003vv,
     author    = "Barmin, V. V. and others",
 collaboration = "DIANA",
     title     = "Observation of a baryon resonance with positive strangeness
                  in K+  collisions with Xe nuclei",
     journal   = "Phys. Atom. Nucl.",
     volume    = "66",
     year      = "2003",
     pages     = "1715-1718",
     SLACcitation  = "%%CITATION = HEP-EX 0304040;%%"
}
@Article{Abdel-Bary:2004ts,
     author    = "Abdel-Bary, M. and others",
 collaboration = "COSY-TOF",
     title     = "Evidence for a narrow resonance at 1530-MeV/c**2 in the K0
                  p system of  the reaction p p --> Sigma+ K0 p from the
                  COSY-TOF experiment",
     journal   = "Phys. Lett.",
     volume    = "B595",
     year      = "2004",
     pages     = "127-134",
     SLACcitation  = "%%CITATION = HEP-EX 0403011;%%"
}
@Article{Asratyan:2003cb,
     author    = "Asratyan, A. E. and Dolgolenko, A. G. and Kubantsev, M. A.
                  ",
     title     = "Evidence for formation of a narrow K0(S) p resonance with
                  mass near  1533-MeV in neutrino interactions",
     journal   = "Phys. Atom. Nucl.",
     volume    = "67",
     year      = "2004",
     pages     = "682-687",
     SLACcitation  = "%%CITATION = HEP-EX 0309042;%%"
}
@Article{Airapetian:2003ri,
     author    = "Airapetian, A. and others",
 collaboration = "HERMES",
     title     = "Evidence for a narrow |S| = 1 baryon state at a mass of
                  1528-MeV in  quasi-real photoproduction",
     journal   = "Phys. Lett.",
     volume    = "B585",
     year      = "2004",
     pages     = "213",
     SLACcitation  = "%%CITATION = HEP-EX 0312044;%%"
}
@Article{Chekanov:2004kn,
     author    = "Chekanov, S. and others",
 collaboration = "ZEUS",
     title     = "Evidence for a narrow baryonic state decaying to K0(S) p
                  and K0(S) anti-p in deep inelastic scattering at HERA",
     journal   = "Phys. Lett.",
     volume    = "B591",
     year      = "2004",
     pages     = "7-22",
     SLACcitation  = "%%CITATION = HEP-EX 0403051;%%"
}
@Article{Alt:2003vb,
     author    = "Alt, C. and others",
 collaboration = "NA49",
     title     = "Observation of an exotic S = -2, Q = -2 baryon resonance in
                  proton  proton collisions at the CERN SPS",
     journal   = "Phys. Rev. Lett.",
     volume    = "92",
     year      = "2004",
     pages     = "042003",
     SLACcitation  = "%%CITATION = HEP-EX 0310014;%%"
}
@Article{Aslanyan:2004gs,
     author    = "Aslanyan, P. Zh. and Emelyanenko, V. N. and Rikhkvitzkaya,
                  G. G.",
     title     = "Observation of S = +1 narrow resonances in the system K0(S)
                  p from p + C-3_H-8 collision at 10-GeV/c",
     journal   = "Nucl. Phys.",
     volume    = "A755",
     year      = "2005",
     pages     = "375-378",
     SLACcitation  = "%%CITATION = HEP-EX 0403044;%%"
}
@Article{Dzierba:2004db,
     author    = "Dzierba, Alex R. and Meyer, Curtis A. and Szczepaniak, Adam
                  P.",
     title     = "Reviewing the evidence for pentaquarks",
     journal   = "J. Phys. Conf. Ser.",
     volume    = "9",
     year      = "2005",
     pages     = "192-204",
     SLACcitation  = "%%CITATION = HEP-EX 0412077;%%"
}
@Unpublished{diVita,
     author    = "Battaglieri, Marco and De Vita and others",
     collaboration = "CLAS",
     year      = "2005",
}
@Article{Strottman:1979qu,
     author    = "Strottman, D.",
     title     = "MULTI - QUARK BARYONS AND THE MIT BAG MODEL",
     journal   = "Phys. Rev.",
     volume    = "D20",
     year      = "1979",
     pages     = "748-767",
     SLACcitation  = "%%CITATION = PHRVA,D20,748;%%"
}
@Article{Weinstein:1982gc,
     author    = "Weinstein, John D. and Isgur, Nathan",
     title     = "DO MULTI - QUARK HADRONS EXIST?",
     journal   = "Phys. Rev. Lett.",
     volume    = "48",
     year      = "1982",
     pages     = "659",
     SLACcitation  = "%%CITATION = PRLTA,48,659;%%"
}
@Article{Praszalowicz:1987em,
     author    = "Praszalowicz, Michal",
     title     = "SU(3) SKYRMION",
     year      = "1987",
     note      = "Talk presented at the Cracow Workshop on Skyrmions and
                  Anomalies, Mogilany, Poland, Feb 20-24, 1987"
}
@Article{Lipkin:1987sk,
     author    = "Lipkin, Harry J.",
     title     = "NEW POSSIBILITIES FOR EXOTIC HADRONS: ANTICHARMED STRANGE
                  BARYONS",
     journal   = "Phys. Lett.",
     volume    = "B195",
     year      = "1987",
     pages     = "484",
     SLACcitation  = "%%CITATION = PHLTA,B195,484;%%"
}
@Article{Carlson:1991zt,
     author    = "Carlson, J. and Pandharipande, V. R.",
     title     = "Absence of exotic hadrons in flux tube quark models",
     journal   = "Phys. Rev.",
     volume    = "D43",
     year      = "1991",
     pages     = "1652-1658",
     SLACcitation  = "%%CITATION = PHRVA,D43,1652;%%"
}
@Article{Diakonov:1997mm,
     author    = "Diakonov, Dmitri and Petrov, Victor and Polyakov, Maxim V.
                  ",
     title     = "Exotic anti-decuplet of baryons: Prediction from chiral
                  solitons",
     journal   = "Z. Phys.",
     volume    = "A359",
     year      = "1997",
     pages     = "305-314",
     SLACcitation  = "%%CITATION = HEP-PH 9703373;%%"
}
@Article{Jaffe:2003sg,
     author    = "Jaffe, Robert L. and Wilczek, Frank",
     title     = "Diquarks and exotic spectroscopy",
     journal   = "Phys. Rev. Lett.",
     volume    = "91",
     year      = "2003",
     pages     = "232003",
     SLACcitation  = "%%CITATION = HEP-PH 0307341;%%"
}
@Article{Karliner:2003dt,
     author    = "Karliner, Marek and Lipkin, Harry J.",
     title     = "A Diquark-Triquark Model for the KN Pentaquark",
     journal   = "Phys. Lett.",
     volume    = "B575",
     year      = "2003",
     pages     = "249-255",
     SLACcitation  = "%%CITATION = HEP-PH 0402260;%%"
}
@Article{Carlson:2003pn,
     author    = "Carlson, Carl E. and Carone, Christopher D. and Kwee, Herry
                  J. and Nazaryan, Vahagn",
     title     = "Phenomenology of the pentaquark antidecuplet",
     journal   = "Phys. Lett.",
     volume    = "B573",
     year      = "2003",
     pages     = "101-108",
     SLACcitation  = "%%CITATION = HEP-PH 0307396;%%"
}
@Article{Hiyama:2005cf,
     author    = "Hiyama, E. and Kamimura, M. and Hosaka, A. and Toki, H. and
                  Yahiro, M.",
     title     = "Five-body calculation of resonance and scattering states of
                  pentaquark system",
     year      = "2005",
     SLACcitation  = "%%CITATION = HEP-PH 0507105;%%"
}
@Article{Eidelman:2004wy,
     author    = "Eidelman, S. and others",
 collaboration = "Particle Data Group",
     title     = "Review of particle physics",
     journal   = "Phys. Lett.",
     volume    = "B592",
     year      = "2004",
     pages     = "1",
     SLACcitation  = "%%CITATION = PHLTA,B592,1;%%"
}
@Article{Mathur:2004jr,
     author    = "Mathur, N. and others",
     title     = "A study of pentaquarks on the lattice with overlap
                  fermions",
     journal   = "Phys. Rev.",
     volume    = "D70",
     year      = "2004",
     pages     = "074508",
     SLACcitation  = "%%CITATION = HEP-PH 0406196;%%"
}
@Article{Lasscock:2005tt,
     author    = "Lasscock, B. G. and others",
     title     = "Search for the pentaquark resonance signature in lattice
                  QCD",
     journal   = "Phys. Rev.",
     volume    = "D72",
     year      = "2005",
     pages     = "014502",
     SLACcitation  = "%%CITATION = HEP-LAT 0503008;%%"
}
@Article{Capstick:2003iq,
     author    = "Capstick, Simon and Page, Philip R. and Roberts, Winston",
     title     = "Interpretation of the Theta+ as an isotensor resonance with
                  weakly  decaying partners",
     journal   = "Phys. Lett.",
     volume    = "B570",
     year      = "2003",
     pages     = "185-190",
     SLACcitation  = "%%CITATION = HEP-PH 0307019;%%"
}
@PhDThesis{Paris:2000phd,
  AUTHOR     = {Mark W. Paris},
  YEAR       = {2000},
  TITLE      = {Quantum Monte Carlo calculations of three and six-quark states},
  SCHOOL     = {University of Illinois at Urbana-Champaign}
}
@Article{Paris:2000bj,
     author    = "Paris, M. W. and Pandharipande, Vijay R.",
     title     = "Quantum Monte Carlo calculations of six-quark states",
     journal   = "Phys. Rev.",
     volume    = "C62",
     year      = "2000",
     pages     = "015201",
     SLACcitation  = "%%CITATION = NUCL-TH 0002041;%%"
}
@Article{Pandharipande:1981la,
     author    = "J. Lomnitz-Adler and V. R. Pandharipande and R. A. Smith",
     title     = "Monte Carlo calculations of triton and 4He nuclei with the Reid potential", 
     journal   = "Nuc.\ Phys.\ A", 
     volume    = "361", 
     year      = "1981",
     pages     = "399-411",
}
@InProceedings{ Lewart:1991,
  AUTHOR       = {D.S. Lewart and V.R. Pandharipande},
  YEAR         = {1991},
  TITLE        = {Variational Monte Carlo studies of many-body systems},
  BOOKTITLE    = {Monte Carlo Methods in Theortical Physics, },
  editor       = {S. Caracciolo and A. Fabrocini},
  publisher    = {ETS Editrice},
  address      = {Pisa},
  pages        = {1--33}
 }
@Article{Isgur:1984bm,
     author    = "Isgur, Nathan and Paton, Jack",
     title     = "A FLUX TUBE MODEL FOR HADRONS IN QCD",
     journal   = "Phys. Rev.",
     volume    = "D31",
     year      = "1985",
     pages     = "2910",
     SLACcitation  = "%%CITATION = PHRVA,D31,2910;%%"
}
@Book{Hamermesh,
  AUTHOR     = {M. Hamermesh},
  YEAR       = {1989},
  TITLE      = {Group Theory and Its Application to Physical Problems},
  PUBLISHER  = {Dover},
  address    = {New York}
}
@Article{Jenkins:1991ts,
     author    = "Jenkins, Elizabeth",
     title     = "Baryon masses in chiral perturbation theory",
     journal   = "Nucl. Phys.",
     volume    = "B368",
     year      = "1992",
     pages     = "190-203",
     SLACcitation  = "%%CITATION = NUPHA,B368,190;%%"
}
@Article{Thomas:1999mu,
     author    = "Thomas, Anthony W. and Krein, G.",
     title     = "Chiral corrections in hadron spectroscopy",
     journal   = "Phys. Lett.",
     volume    = "B456",
     year      = "1999",
     pages     = "5-8",
     SLACcitation  = "%%CITATION = NUCL-TH 9902013;%%"
}
@Article{Tanabe:1985rz,
     author    = "Tanabe, H. and Ohta, K.",
     title     = "DYNAMICAL MODEL FOR PION PHOTOPRODUCTION IN THE DELTA
                  REGION",
     journal   = "Phys. Rev.",
     volume    = "C31",
     year      = "1985",
     pages     = "1876-1884",
     SLACcitation  = "%%CITATION = PHRVA,C31,1876;%%"
}
@Article{Sato:1991rp,
     author    = "Sato, T. and Doi, M. and Odagawa, N. and Ohtsubo, H.",
     title     = "pi N N system and the method of unitary transformation",
     journal   = "Few Body Syst. Suppl.",
     volume    = "5",
     year      = "1992",
     pages     = "254-259",
     SLACcitation  = "%%CITATION = FBSSE,5,254;%%"
}
@Article{Kobayashi:1997fm,
     author    = "Kobayashi, M. and Sato, T. and Ohtsubo, H.",
     title     = "Effective interactions for mesons and baryons in nuclei",
     journal   = "Prog. Theor. Phys.",
     volume    = "98",
     year      = "1997",
     pages     = "927-951",
     SLACcitation  = "%%CITATION = PTPKA,98,927;%%"
}
@Article{Gross:1992tj,
     author    = "Gross, Franz and Surya, Yohanes",
     title     = "Unitary, relativistic resonance model for pi N scattering",
     journal   = "Phys. Rev.",
     volume    = "C47",
     year      = "1993",
     pages     = "703-723",
     SLACcitation  = "%%CITATION = PHRVA,C47,703;%%"
}
@Article{Surya:1995ur,
     author    = "Surya, Yohanes and Gross, Franz",
     title     = "Unitary, gauge invariant, relativistic resonance model for
                  pion photoproduction",
     journal   = "Phys. Rev.",
     volume    = "C53",
     year      = "1996",
     pages     = "2422-2448",
     SLACcitation  = "%%CITATION = PHRVA,C53,2422;%%"
}
@Article{Sato:1996gk,
     author    = "Sato, T. and Lee, T. S. H.",
     title     = "Meson-exchange model for pi N scattering and gamma N --> pi
                  N  reaction",
     journal   = "Phys. Rev.",
     volume    = "C54",
     year      = "1996",
     pages     = "2660-2684",
     SLACcitation  = "%%CITATION = NUCL-TH 9606009;%%"
}
@Article{Yoshimoto:1999dr,
     author    = "Yoshimoto, T. and Sato, T. and Arima, M. and Lee, T. S. H.
                  ",
     title     = "Dynamical test of constituent quark models with pi N
                  reactions",
     journal   = "Phys. Rev.",
     volume    = "C61",
     year      = "2000",
     pages     = "065203",
     SLACcitation  = "%%CITATION = NUCL-TH 9908048;%%"
}
@Article{Sato:2000jf,
     author    = "Sato, T. and Lee, T. S. H.",
     title     = "Dynamical study of the Delta excitation in N(e,e' pi)
                  reactions",
     journal   = "Phys. Rev.",
     volume    = "C63",
     year      = "2001",
     pages     = "055201",
     SLACcitation  = "%%CITATION = NUCL-TH 0010025;%%"
}
@Article{Lee:1983xu,
     author    = "Lee, T. S. H.",
     title     = "MESON EXCHANGE HAMILTONIAN FOR N N SCATTERING UP TO 1-GEV
                  AND DELTA NUCLEUS DYNAMICS",
     journal   = "Phys. Rev. Lett.",
     volume    = "50",
     year      = "1983",
     pages     = "1571-1574",
     SLACcitation  = "%%CITATION = PRLTA,50,1571;%%"
}
@Article{Lee:1984us,
     author    = "Lee, T. S. H.",
     title     = "MESON THEORY OF NUCLEON NUCLEON SCATTERING UP TO 2-GEV",
     journal   = "Phys. Rev.",
     volume    = "C29",
     year      = "1984",
     pages     = "195-203",
     SLACcitation  = "%%CITATION = PHRVA,C29,195;%%"
}
@Article{Kamalov:1999hs,
     author    = "Kamalov, S. S. and Yang, Shin Nan",
     title     = "Pion cloud and the Q**2 dependence of gamma* N <--> Delta
                  transition  form factors",
     journal   = "Phys. Rev. Lett.",
     volume    = "83",
     year      = "1999",
     pages     = "4494-4497",
     SLACcitation  = "%%CITATION = NUCL-TH 9904072;%%"
}
@Article{Chen:2002mn,
     author    = "Chen, Guan-Yeu and Kamalov, Sabit and Yang, Shin Nan and
                  Drechsel, Dieter and Tiator, Lothar",
     title     = "Excitation of S(11) resonances in pion scattering and pion
                  photoproduction on the proton",
     journal   = "Nucl. Phys.",
     volume    = "A723",
     year      = "2003",
     pages     = "447-463",
     SLACcitation  = "%%CITATION = NUCL-TH 0210013;%%"
}
@Article{Chiang:2001pw,
     author    = "Chiang, Wen-Tai and Tabakin, F. and Lee, T. S. H. and
                  Saghai, B.",
     title     = "Coupled-channel study of gamma p --> K+ Lambda",
     journal   = "Phys. Lett.",
     volume    = "B517",
     year      = "2001",
     pages     = "101-108",
     SLACcitation  = "%%CITATION = NUCL-TH 0104052;%%"
}
@Article{Kamalov:2000en,
     author    = "Kamalov, Sabit S. and Yang, Shin Nan and Drechsel, Dieter
                  and Hanstein, Olaf and Tiator, Lothar",
     title     = "gamma* N --> Delta transition form factors: A new analysis
                  of the JLab  data on p(e,e' p)pi0 at Q**2 = 2.8-(GeV/c)**2
                  and 4.0-(GeV/c)**2",
     journal   = "Phys. Rev.",
     volume    = "C64",
     year      = "2001",
     pages     = "032201",
     SLACcitation  = "%%CITATION = NUCL-TH 0006068;%%"
}
@Article{Fuda:2003pd,
     author    = "Fuda, Michael G. and Alharbi, Hamoud",
     title     = "Photoproduction of mesons from the nucleon",
     journal   = "Phys. Rev.",
     volume    = "C68",
     year      = "2003",
     pages     = "064002",
     SLACcitation  = "%%CITATION = PHRVA,C68,064002;%%"
}
@Article{Kaiser:1995eg,
     author    = "Kaiser, Norbert and Siegel, P. B. and Weise, W.",
     title     = "Chiral dynamics and the low-energy kaon - nucleon
                  interaction",
     journal   = "Nucl. Phys.",
     volume    = "A594",
     year      = "1995",
     pages     = "325-345",
     SLACcitation  = "%%CITATION = NUCL-TH 9505043;%%"
}
@Article{Oset:1997it,
     author    = "Oset, E. and Ramos, A.",
     title     = "Non perturbative chiral approach to s-wave anti-K N
                  interactions",
     journal   = "Nucl. Phys.",
     volume    = "A635",
     year      = "1998",
     pages     = "99-120",
     SLACcitation  = "%%CITATION = NUCL-TH 9711022;%%"
}
@Unpublished{Paris:2005q3,
     author    = "Mark W. Paris",
     title     = "Quantum Monte Carlo calculations of s-- and p--wave
                  baryon states",
     year      = "2005",
     note      = "in preparation"
}
@Unpublished{LeeParis:2005,
     author    = "Mark W. Paris and {T.-S.H. Lee}",
     title     = "Quantum Monte Carlo calculations of strong and 
                  electromagnetic transition form factors",
     year      = "2005",
     note      = "in preparation"
}
@Article{Paris:2005q5,
     author    = "Mark W. Paris",
     title     = "Variational Monte Carlo study of pentaquark states",
     journal   = "Phys. Rev. Lett.",
     volume    = "95",
     year      = "2005",
     pages     = "202002",
}
@Article{JLab,
     author    = "Mecking, B. A. and others",
 collaboration = "CLAS",
     title     = "The CEBAF Large Acceptance Spectrometer (CLAS)",
     journal   = "Nucl. Instrum. Meth.",
     volume    = "A503",
     year      = "2003",
     pages     = "513-553",
     SLACcitation  = "%%CITATION = NUIMA,A503,513;%%"
}
@Article{MAMI,
     author    = "Friedrich, J. and Herminghaus, H. and Walcher, T.",
     title     = "MAMI in operation: The Mainz microtron and the research
                  program. (In German)",
     journal   = "Phys. Bl.",
     volume    = "47",
     year      = "1991",
     pages     = "291-294",
     SLACcitation  = "%%CITATION = PHBLA,47,291;%%"
}
@Article{Bates,
     author    = "Dolfini, S. M. and others",
     title     = "Design of an 830-MeV/c out-of-plane spectrometer",
     journal   = "Nucl. Instrum. Meth.",
     volume    = "A344",
     year      = "1994",
     pages     = "571-582",
     SLACcitation  = "%%CITATION = NUIMA,A344,571;%%"
}
@Article{GRAAL,
     author    = "F. Ghio and others",
     title     = "The GRAAL high resolution BGO calorimeter and its 
                  energy calibration and monitoring system",
     journal   = "Nucl. Instrum. Meth.",
     volume    = "A404",
     year      = "1998",
     pages     = "71-86",
}
@Article{LEGS,
     author    = "Thorn, C. E. and others",
     title     = "THE LEGS ELECTRON SPECTROMETER FOR TAGGING BACKSCATTERED
                  PHOTONS",
     journal   = "Nucl. Instrum. Meth.",
     volume    = "A285",
     year      = "1989",
     pages     = "447-458",
     SLACcitation  = "%%CITATION = NUIMA,A285,447;%%"
}
@Article{LEPS,
     author    = "Nakano, T.",
     collaboration = "LEPS",
     title     = "Laser-electron photon project at SPring-8",
     journal   = "Mod. Phys. Lett.",
     volume    = "A18",
     year      = "2003",
     pages     = "208-214",
     SLACcitation  = "%%CITATION = MPLAE,A18,208;%%"
}
@Article{ELSA,
     author    = "Paul, E. and others",
     title     = "Physics with real photons at SAPHIR: Experiment, results
                  and future plans",
     journal   = "Prog. Part. Nucl. Phys.",
     volume    = "34",
     year      = "1995",
     pages     = "201-210",
     SLACcitation  = "%%CITATION = PPNPD,34,201;%%"
}
@Article{Trotter:1959,
     author    = "Trotter, H. F.",
     title     = "",
     journal   = "Proc. Am. Math. Soc.",
     volume    = "10",
     year      = "1959",
     pages     = "545"
}
@Article{Capstick:1992th,
     author    = "Capstick, Simon and Roberts, Winston",
     title     = "N pi decays of baryons in a relativized model",
     journal   = "Phys. Rev.",
     volume    = "D47",
     year      = "1993",
     pages     = "1994-2010",
     SLACcitation  = "%%CITATION = PHRVA,D47,1994;%%"
}
@Article{Roberts:1992js,
     author    = "Roberts, W. and Silvestre- Brac, B.",
     title     = "General method of calculation of any hadronic decay in the
                  p wave triplet model",
     journal   = "Few Body Syst.",
     volume    = "11",
     year      = "1992",
     pages     = "171-193",
     SLACcitation  = "%%CITATION = APASA,11,171;%%"
}
@Article{Kumano:1988ga,
     author    = "Kumano, S. and Pandharipande, V. R.",
     title     = "DECAY OF MESONS IN FLUX TUBE QUARK MODEL",
     journal   = "Phys. Rev.",
     volume    = "D38",
     year      = "1988",
     pages     = "146-151",
     SLACcitation  = "%%CITATION = PHRVA,D38,146;%%"
}
@Article{MSL,
     author    = "Matsuyama, A. and Sato, T. and Lee, T. -S. H.",
     title     = "Dynamical coupled-channel model of meson production
                  reactions in the nucleon resonance region",
     journal   = "Phys. Rept.",
     volume    = "439",
     year      = "2007",
     pages     = "193-253",
     SLACcitation  = "%%CITATION = NUCL-TH/0608051;%%"
}
@Article{OTL,
     author    = "Oh, Yong-seok and Titov, Alexander I. and Lee, T. S. H.",
     title     = "Nucleon resonances in omega photoproduction",
     journal   = "Phys. Rev.",
     volume    = "C63",
     year      = "2001",
     pages     = "025201",
     SLACcitation  = "%%CITATION = NUCL-TH/0006057;%%"
}
@Article{PDG,
     author    = "Yao, W. -M. and others",
 collaboration = "Particle Data Group",
     title     = "Review of particle physics",
     journal   = "J. Phys.",
     volume    = "G33",
     year      = "2006",
     pages     = "1-1232",
     SLACcitation  = "%%CITATION = JPHGB,G33,1;%%"
}
@Article{SKO,
     author    = "Kobayashi, M. and Sato, T. and Ohtsubo, H.",
     title     = "Effective interactions for mesons and baryons in nuclei",
     journal   = "Prog. Theor. Phys.",
     volume    = "98",
     year      = "1997",
     pages     = "927-951",
     SLACcitation  = "%%CITATION = PTPKA,98,927;%%"
}
@Article{Barth:2003kv,
     author    = "Barth, J. and others",
     title     = "Low-energy of photoproduciton of omega-mesons",
     journal   = "Eur. Phys. J.",
     volume    = "A18",
     year      = "2003",
     pages     = "117-127",
     SLACcitation  = "%%CITATION = EPHJA,A18,117;%%"
}
@Article{Williams:2005em,
     author    = "Williams, M. and Applegate, D. and Bellis, M. and Meyer, C.
                  A. and Krahn, Z.",
     title     = "The Carnegie Mellon University program for studying baryon
                  resonance photoproduction using partial wave analysis",
     note      = "Prepared for International Workshop on the Physics of
                  Excited Baryons (NSTAR 05), Tallahassee, Florida, 10-15 Oct",
     year      = "2005"
}
@Article{Jacob:1959at,
     author    = "Jacob, M. and Wick, G. C.",
     title     = "On the general theory of collisions for particles with
                  spin",
     journal   = "Ann. Phys.",
     volume    = "7",
     year      = "1959",
     pages     = "404-428",
     SLACcitation  = "%%CITATION = APNYA,7,404;%%"
}
@Article{Karami:1979ib,
     author    = "Karami, H. and others",
     title     = "ELASTIC SCATTERING AND OMEGA MESON PRODUCTION NEAR THE
                  THRESHOLD OF PI- P $\to$ OMEGA N",
     journal   = "Nucl. Phys.",
     volume    = "B154",
     year      = "1979",
     pages     = "503-518",
     SLACcitation  = "%%CITATION = NUPHA,B154,503;%%"
}
@Article{Hanhart:1998wx,
     author    = "Hanhart, C. and Kudryavtsev, Alexander E.",
     title     = "On momentum dependence of the reaction pi- p --> omega n
                  near  threshold",
     journal   = "Eur. Phys. J.",
     volume    = "A6",
     year      = "1999",
     pages     = "325-328",
     SLACcitation  = "%%CITATION = NUCL-TH/9812022;%%"
}
@Article{Hanhart:2001ft,
     author    = "Hanhart, C. and Sibirtsev, A. and Speth, J.",
     title     = "The reaction pi N --> omega N revisited: The omega N
                  scattering length",
     year      = "2001",
     SLACcitation  = "%%CITATION = HEP-PH/0107245;%%"
}
@Article{James:1975dr,
     author    = "James, F. and Roos, M.",
     title     = "Minuit: A System for Function Minimization and Analysis of
                  the Parameter Errors and Correlations",
     journal   = "Comput. Phys. Commun.",
     volume    = "10",
     year      = "1975",
     pages     = "343-367",
     SLACcitation  = "%%CITATION = CPHCB,10,343;%%"
}
@Article{Bosted:1994tm,
     author    = "Bosted, Peter E.",
     title     = "An Empirical fit to the nucleon electromagnetic form-
                  factors",
     journal   = "Phys. Rev.",
     volume    = "C51",
     year      = "1995",
     pages     = "409-411",
     SLACcitation  = "%%CITATION = PHRVA,C51,409;%%"
}
@Article{Shklyar:2004ba,
     author    = "Shklyar, V. and Lenske, H. and Mosel, U. and Penner, G.",
     title     = "Coupled-channel analysis of the omega-meson production in
                  pi N and  gamma N reactions for cm energies up to 2-GeV",
     journal   = "Phys. Rev.",
     volume    = "C71",
     year      = "2005",
     pages     = "055206",
     SLACcitation  = "%%CITATION = NUCL-TH/0412029;%%"
}
@Article{Nakayama:1998zv,
     author    = "Nakayama, K. and Szczurek, A. and Hanhart, C. and
                  Haidenbauer, J. and Speth, J.",
     title     = "Production of omega mesons in proton proton collisions",
     journal   = "Phys. Rev.",
     volume    = "C57",
     year      = "1998",
     pages     = "1580-1587",
     SLACcitation  = "%%CITATION = NUCL-TH/9802013;%%"
}
@Article{Hohler:1976ax,
     author    = "Hohler, G. and others",
     title     = "Analysis of Electromagnetic Nucleon Form-Factors",
     journal   = "Nucl. Phys.",
     volume    = "B114",
     year      = "1976",
     pages     = "505",
     SLACcitation  = "%%CITATION = NUPHA,B114,505;%%"
}
@Article{Machleidt:1987hj,
     author    = "Machleidt, R. and Holinde, K. and Elster, C.",
     title     = "The Bonn Meson Exchange Model for the Nucleon Nucleon
                  Interaction",
     journal   = "Phys. Rept.",
     volume    = "149",
     year      = "1987",
     pages     = "1-89",
     SLACcitation  = "%%CITATION = PRPLC,149,1;%%"
}
@Article{JuliaDiaz:2007fa,
     author    = "Julia-Diaz, B. and Lee, T. -S. H. and Matsuyama, A. and
                  Sato, T. and Smith, L. C.",
     title     = "Dynamical Coupled-Channels Effects on Pion
                  Photoproduction",
     year      = "2007"
}
@Article{JuliaDiaz:2007kz,
     author    = "Julia-Diaz, B. and Lee, T. -S. H. and Matsuyama, A. and
                  Sato, T.",
     title     = "{Dynamical Coupled-Channel Model of $\pi N$ Scattering in
                  the W $\leq$ 2 GeV Nucleon Resonance Region}",
     journal   = "Phys. Rev.",
     volume    = "C76",
     year      = "2007",
     pages     = "065201"
}
@Article{Danburg:1971ui,
     author    = "Danburg, J. S. and others",
     title     = "Production and decay of eta and omega mesons in the
                  reaction pi+ d $\to$ (p)p pi+ pi- pi0 between 1.1 and 2.4
                  gev/c",
     journal   = "Phys. Rev.",
     volume    = "D2",
     year      = "1970",
     pages     = "2564-2588",
     SLACcitation  = "%%CITATION = PHRVA,D2,2564;%%"
}
@Article{Ajaka:2006bn,
     author    = "Ajaka, J. and others",
     title     = "Evidence for nucleon-resonance excitation in omega-meson
                  photoproduction",
     journal   = "Phys. Rev. Lett.",
     volume    = "96",
     year      = "2006",
     pages     = "132003",
     SLACcitation  = "%%CITATION = PRLTA,96,132003;%%"
}
@Article{Hourany:2005wh,
     author    = "Hourany, E.",
 collaboration = "GRAAL",
     title     = "Photoproduction of the omega meson on the nucleon",
     journal   = "Nucl. Phys.",
     volume    = "A755",
     year      = "2005",
     pages     = "447-450",
     SLACcitation  = "%%CITATION = NUPHA,A755,447;%%"
}
@Article{Zhao:1998rt,
     author    = "Zhao, Qiang and Li, Zhen-ping and Bennhold, C.",
     title     = "omega and rho photoproduction with an effective quark model
                  Lagrangian",
     journal   = "Phys. Lett.",
     volume    = "B436",
     year      = "1998",
     pages     = "42-48",
     SLACcitation  = "%%CITATION = NUCL-TH/9803015;%%"
}
@Article{Muehlich:2006nn,
     author    = "Muehlich, P. and Shklyar, V. and Leupold, S. and Mosel, U.
                  and Post, M.",
     title     = "The spectral function of the omega meson in nuclear matter
                  from a coupled-channel resonance model",
     journal   = "Nucl. Phys.",
     volume    = "A780",
     year      = "2006",
     pages     = "187-205",
     SLACcitation  = "%%CITATION = NUCL-TH/0607061;%%"
}
@Article{Brown:1991kk,
     author    = "Brown, G. E. and Rho, Mannque",
     title     = "Scaling effective Lagrangians in a dense medium",
     journal   = "Phys. Rev. Lett.",
     volume    = "66",
     year      = "1991",
     pages     = "2720-2723",
     SLACcitation  = "%%CITATION = PRLTA,66,2720;%%"
}
@Article{Tuchitani:2004ur,
     author    = "Tuchitani, Kunito and others",
     title     = "Effective meson masses, effective meson nucleon couplings
                  and neutron  star radii",
     journal   = "Int. J. Mod. Phys.",
     volume    = "E14",
     year      = "2005",
     pages     = "955-985",
     SLACcitation  = "%%CITATION = NUCL-TH/0407004;%%"
}
@Article{Titov:1998bw,
     author    = "Titov, Alexander I. and Oh, Yong-seok and Yang, Shin Nan
                  and Morii, Tosiyuki",
     title     = "Photoproduction of Phi meson from proton: Polarization
                  observables and  the strangeness in the nucleon",
     journal   = "Phys. Rev.",
     volume    = "C58",
     year      = "1998",
     pages     = "2429-2449",
     SLACcitation  = "%%CITATION = NUCL-TH/9804043;%%"
}
@Article{Cohen,
     author    = "Cohen, I.\ Bernard",
     title     = "An Interview with Einstein",
     journal   = "Sci. Am.",
     volume    = "193",
     year      = "1955",
     pages     = "68-73",
     note      = "``Einstein said that at the beginning of the century 
                  only a few scientists had been philosophically minded, 
                  but today physicists are almost all philosophers, 
                  although `they are apt to be bad philosophers.'~''"
}
@Article{Arndt:2006bf,
     author    = "Arndt, R. A. and Briscoe, W. J. and Strakovsky, I. I. and
                  Workman, R. L.",
     title     = "{Extended partial-wave analysis of pi N scattering data}",
     journal   = "Phys. Rev.",
     volume    = "C74",
     year      = "2006",
     pages     = "045205"
}
@Article{Usov:2005wy,
     author    = "Usov, A. and Scholten, O.",
     title     = "{K Lambda and K Sigma photoproduction in a coupled channels
                  framework}",
     journal   = "Phys. Rev.",
     volume    = "C72",
     year      = "2005",
     pages     = "025205",
     SLACcitation  = "%%CITATION = NUCL-TH/0503013;%%"
}
@Article{Tabakin:1970sa,
     author    = "M.\ Haftel and F.\ Tabakin",
     title     = "Nuclear saturation and the smoothness of 
                   nucleon-nucleon potentials",
     journal   = "Nucl. Phys.",
     volume    = "A158",
     year      = "1979",
     pages     = "1"
}
@PhDThesis{Williams:2007phd,
  AUTHOR     = {Mike Williams},
  YEAR       = {2007},
  TITLE      = {Measurement of Differential Cross Sections and Spin Density 
                Matrix Elements along with a Partial Wave Analysis for
                omega photoproduction using CLAS at Jefferson Lab},
  SCHOOL     = {Carnegie Mellon University},
  URL        = {http://www.jlab.org/~mwill}
}
@Article{Trnka:2005ey,
     author    = "Trnka, D. and others",
 collaboration = "CBELSA/TAPS",
     title     = "{First observation of in-medium modifications of the omega
                  meson}",
     journal   = "Phys. Rev. Lett.",
     volume    = "94",
     year      = "2005",
     pages     = "192303",
     SLACcitation  = "%%CITATION = NUCL-EX/0504010;%%"
}
@Article{Schillaci:1969hq,
     author    = "Schillaci, M. E. and Silbar, R. R. and Young, J. E.",
     title     = "{Pion production in nucleon-nucleon collisions at
                  threshold}",
     journal   = "Phys. Rev.",
     volume    = "179",
     year      = "1969",
     pages     = "1539-1545",
     SLACcitation  = "%%CITATION = PHRVA,179,1539;%%"
}
@Article{Lee:1993xh,
     author    = "Lee, T. S. H. and Riska, D. O.",
     title     = "{Short range exchange contributions to the cross-section
                  for p p $\to$ p p pi0 near threshold}",
     journal   = "Phys. Rev. Lett.",
     volume    = "70",
     year      = "1993",
     pages     = "2237-2240",
     SLACcitation  = "%%CITATION = PRLTA,70,2237;%%"
}
@Article{Koltun:1965yk,
     author    = "Koltun, D. S. and Reitan, A.",
     title     = "{Production and absorption of S-wave pions at low energy by
                  two nucleons}",
     journal   = "Phys. Lett.",
     volume    = "141",
     year      = "1966",
     pages     = "1413-1418",
     SLACcitation  = "%%CITATION = PHLTA,141,1413;%%"
}
@Article{Miller:1991pi,
     author    = "Miller, G. A. and Sauer, P. U.",
     title     = "{Total cross-section for p + p $\to$ p + p + pi0 near
                  threshold}",
     journal   = "Phys. Rev.",
     volume    = "C44",
     year      = "1991",
     pages     = "1725-1727",
     SLACcitation  = "%%CITATION = PHRVA,C44,1725;%%"
}
@Article{SAID,
  author     = "{Center for Nuclear Studies}",
  year       = {2010},
  note       = {{\em Scattering Analysis Interactive Database}},
  url        = {http://gwdac.phys.gwu.edu/}
}
@Article{Jones:1972ky,
     author    = "Jones, H. F. and Scadron, M. D.",
     title     = "{Multipole gamma N Delta form-factors and resonant
                  photoproduction and electroproduction}",
     journal   = "Ann. Phys.",
     volume    = "81",
     year      = "1973",
     pages     = "1-14"
}

%G0DXS

@Article{Fuchs:1996ja,
     author    = "Fuchs, M. and others",
     title     = "{Neutral pion photoproduction from the proton near
                  threshold}",
     journal   = "Phys. Lett.",
     volume    = "B368",
     year      = "1996",
     pages     = "20-25",
     SLACcitation  = "%%CITATION = PHLTA,B368,20;%%"
}
@Article{Genzel:1973jy,
     author    = "Genzel, H. and Hilger, E. and Knop, G. and Kemen, H. and
                  Wedemeyer, R.",
     title     = "{PHOTOPRODUCTION OF NEUTRAL PIONS ON HYDROGEN. 4.
                  COMBINATION OF THE CROSS-SECTION DATA OF ALL BONN
                  EXPERIMENTS ON THE pi0 PHOTOPRODUCTION BELOW 500-MeV}",
     journal   = "Z. Phys.",
     volume    = "268",
     year      = "1974",
     pages     = "43",
     SLACcitation  = "%%CITATION = ZEPYA,268,43;%%"
}
@Article{Beck:1997ew,
     author    = "Beck, R. and others",
     title     = "{Measurement of the E2/M1 ratio in the N $\to$ Delta
                  transition using the reaction p(gamma(pol.),p)pi0}",
     journal   = "Phys. Rev. Lett.",
     volume    = "78",
     year      = "1997",
     pages     = "606-609",
     SLACcitation  = "%%CITATION = PRLTA,78,606;%%"
}
@Article{Argan:1975pi,
     author    = "Argan, P. and others",
     title     = "{Two-body photodisintegration of $^3$He and $^4$He in
                   the $\Delta(1236)$ region}",
     journal   = "Nuc. Phys.",
     volume    = "A237",
     year      = "1975",
     pages     = "447-464"
}
@Article{Aleksandrov:1978ex,
     author    = "Aleksandrov, Yu. A. and Kozlov, V. A. and Pavlovskaya, V. V
                  ",
     title     = "{STUDY OF NEUTRAL PION PHOTOPRODUCTION ON HYDROGEN IN DELTA
                  (1232) VICINITY. (IN RUSSIAN)}",
     journal   = "Yad. Fiz.",
     volume    = "28",
     year      = "1978",
     pages     = "670-674",
     SLACcitation  = "%%CITATION = YAFIA,28,670;%%"
}
@Article{Ahrens:2004pf,
     author    = "Ahrens, J. and others",
 collaboration = "GDH and A2",
     title     = "{Helicity dependence of the gamma p $\to$ N pi channels and
                  multipole analysis in the Delta region}",
     journal   = "Eur. Phys. J.",
     volume    = "A21",
     year      = "2004",
     pages     = "323-333",
     SLACcitation  = "%%CITATION = EPHJA,A21,323;%%"
}
@Article{Dougan:1977zw,
     author    = "Dougan, P. and Ramsay, V. and Stiefler, W.",
     title     = "{Cross-Sections for Deuteron Photodisintegration from 74-
                  MeV to 241-MeV}",
     journal   = "Z. Phys.",
     volume    = "A280",
     year      = "1977",
     pages     = "341-348",
     SLACcitation  = "%%CITATION = ZEPYA,A280,341;%%"
}
@Article{Aleksandrov:1977tj,
     author    = "Aleksandrov, Yu. A. and Kozlov, V. A. and Maikov, V. N. and
                  Pavlovskaya, V. V",
     title     = "{Photoproduction of pi0 Mesons on Hydrogen at 320-MeV
                  Energy}",
     journal   = "Yad. Fiz.",
     volume    = "25",
     year      = "1977",
     pages     = "80-84",
     SLACcitation  = "%%CITATION = YAFIA,25,80;%%"
}
@Article{Bartholomy:2004uz,
     author    = "Bartholomy, O. and others",
 collaboration = "CB-ELSA",
     title     = "{Neutral pion photoproduction off protons in the energy
                  range 0.3-GeV <  E(gamma) < 3-GeV}",
     journal   = "Phys. Rev. Lett.",
     volume    = "94",
     year      = "2005",
     pages     = "012003",
     SLACcitation  = "%%CITATION = HEP-EX/0407022;%%"
}
@Article{Dougan:1975pa,
     author    = "Dougan, P. and Ramsay, V. and Stiefler, W.",
     title     = "{Cross-Sections for the Photoproduction of pi0 Mesons from
                  Hydrogen from 238-MeV to 922-MeV}",
     journal   = "Z. Phys.",
     volume    = "A276",
     year      = "1976",
     pages     = "155-160",
     SLACcitation  = "%%CITATION = ZEPYA,A276,155;%%"
}
@Article{Yoshioka:1980vu,
     author    = "Yoshioka, M. and others",
     title     = "{DIFFERENTIAL CROSS-SECTIONS OF NEUTRAL PION
                  PHOTOPRODUCTION FROM HYDROGEN IN THE ENERGY REGION FROM
                  390-MEV TO 975-MEV}",
     journal   = "Nucl. Phys.",
     volume    = "B168",
     year      = "1980",
     pages     = "222-242",
     SLACcitation  = "%%CITATION = NUPHA,B168,222;%%"
}
@Article{Hemmi:1973nf,
     author    = "Hemmi, Y. and others",
     title     = "{Neutral pion photoproduction from protons at forward
                  angles in the energy region between 350 mev and 1175 mev}",
     journal   = "Phys. Lett.",
     volume    = "B43",
     year      = "1973",
     pages     = "79-84",
     SLACcitation  = "%%CITATION = PHLTA,B43,79;%%"
}
@Article{Worlock:1960pi,
     author    = "Worlock, R.M.",
     title     = "{Photoproduction of neutral pions at energies
                  600 to 800 MeV}",
     journal   = "Phys. Rev.",
     volume    = "117",
     year      = "1960",
     pages     = "537-543"
}
@Article{Arai:1977kb,
     author    = "Arai, I. and others",
     title     = "{Differential Cross-Sections for Single Pion
                  Photoproduction from Protons in the Energy Range Between
                  500-MeV and 930-MeV}",
     journal   = "J. Phys. Soc. Jap.",
     volume    = "43",
     year      = "1977",
     pages     = "363-368",
     SLACcitation  = "%%CITATION = JUPSA,43,363;%%"
}
@Article{Feller:1974yd,
     author    = "Feller, P. and others",
     title     = "{Photoproduction of neutral pions off hydrogen at photon
                  energies between 0.55 and 2.2 gev at a cm-angle of 120
                  degrees}",
     journal   = "Phys. Lett.",
     volume    = "B49",
     year      = "1974",
     pages     = "197-200",
     SLACcitation  = "%%CITATION = PHLTA,B49,197;%%"
}
@Article{Hemmi:1973ii,
     author    = "Hemmi, Y. and others",
     title     = "{Photoproduction of neutral pions off neutrons in the
                  energy region between 500 mev and 900 mev}",
     journal   = "Nucl. Phys.",
     volume    = "B55",
     year      = "1973",
     pages     = "333-362",
     SLACcitation  = "%%CITATION = NUPHA,B55,333;%%"
}
@Article{Ahrens:2002gu,
     author    = "Ahrens, J. and others",
 collaboration = "GDH",
     title     = "{The helicity amplitudes A(1/2) and A(3/2) for the
                  D(13)(1520) resonance  obtained from the gamma(pol.)
                  p(pol.) --> p pi0 reaction}",
     journal   = "Phys. Rev. Lett.",
     volume    = "88",
     year      = "2002",
     pages     = "232002",
     SLACcitation  = "%%CITATION = HEP-EX/0203006;%%"
}
@Article{Krusche:1999tv,
     author    = "Krusche, B. and others",
     title     = "{Single and double pi0 photoproduction from the deuteron}",
     journal   = "Eur. Phys. J.",
     volume    = "A6",
     year      = "1999",
     pages     = "309-324",
     SLACcitation  = "%%CITATION = EPHJA,A6,309;%%"
}
@Article{Althoff:1979mc,
     author    = "Althoff, K. H. and others",
     title     = "{PHOTOPRODUCTION OF NEUTRAL PIONS IN THE REGION OF THE
                  FOURTH NUCLEON RESONANCE}",
     journal   = "Zeit. Phys.",
     volume    = "C1",
     year      = "1979",
     pages     = "257",
     SLACcitation  = "%%CITATION = ZEPYA,C1,257;%%"
}

@Article{Althoff:1979mb,
     author    = "Althoff, K. H. and others",
     title     = "{PHOTOPRODUCTION OF NEUTRAL PIONS AT BACKWARD ANGLES IN THE
                  RESONANCE REGION AND THE eta - CUSP}",
     journal   = "Zeit. Phys.",
     volume    = "C1",
     year      = "1979",
     pages     = "327",
     SLACcitation  = "%%CITATION = ZEPYA,C1,327;%%"
}
@Article{Delcourt:1969dp,
     author    = "Delcourt, B. and Lefrancois, J. and Parrour, G. and
                  Perez-Y-Jorba, J. P. and Sauvage, G.",
     title     = "{Pi-neutral photoproduction on proton at backward angles
                  between 700 mev and 1150 mev}",
     journal   = "Phys. Lett.",
     volume    = "B29",
     year      = "1969",
     pages     = "70-74",
     SLACcitation  = "%%CITATION = PHLTA,B29,70;%%"
}
@Article{DeStaebler:1965sf,
     author    = "DeStaebler, H. C. and Erickson, E. F. and Hearn, Anthony C.
                  and Schaerf, C.",
     title     = "{PHOTOPRODUCTION OF pi0 FROM HYDROGEN NEAR THE SECOND PION
                  - NUCLEON RESONANCE}",
     journal   = "Phys. Rev.",
     volume    = "140",
     year      = "1965",
     pages     = "B336-B348",
     SLACcitation  = "%%CITATION = PHRVA,140,B336;%%"
}
@Article{Becks:1973ws,
     author    = "Becks, H. and others",
     title     = "{Backward photoproduction of neutral pions off hydrogen at
                  photon energies between 0.4 and 2.2 gev}",
     journal   = "Nucl. Phys.",
     volume    = "B60",
     year      = "1973",
     pages     = "267-276",
     SLACcitation  = "%%CITATION = NUPHA,B60,267;%%"
}
@Article{PhysRev.159.1176,
  title = {Photoproduction of $\pi{}^{0}$ from Hydrogen near the Second and Third Pion-Nucleon Resonances},
  author = {Ward, C.  and Kenton, B.  and York, C. },
  journal = {Phys. Rev.},
  volume = {159},
  number = {5},
  pages = {1176--1186},
  numpages = {10},
  year = {1967},
  month = {Jul},
  doi = {10.1103/PhysRev.159.1176},
  publisher = {American Physical Society}
}
@Article{Bartalini:2005wx,
     author    = "Bartalini, O. and others",
 collaboration = "GRAAL",
     title     = "{Measurement of pi0 photoproduction on the proton from 550-
                  MeV to 1500-MeV at GRAAL}",
     journal   = "Eur. Phys. J.",
     volume    = "A26",
     year      = "2005",
     pages     = "399-419",
     SLACcitation  = "%%CITATION = EPHJA,A26,399;%%"
}
@Article{Dugger:2007bt,
     author    = "Dugger, M. and others",
     title     = "{pi0 photoproduction on the proton for photon energies from
                  0.675-GeV to 2.875-GeV}",
     journal   = "Phys. Rev.",
     volume    = "C76",
     year      = "2007",
     pages     = "025211",
     SLACcitation  = "%%CITATION = ARXIV:0705.0816;%%"
}
@Article{Barton:1974sf,
     author    = "Barton, J. S. and others",
     title     = "{The Photoproduction of Neutral Pions from Protons Between
                  0.7-GeV and 1.7-GeV}",
     journal   = "Nucl. Phys.",
     volume    = "B84",
     year      = "1975",
     pages     = "449",
     SLACcitation  = "%%CITATION = NUPHA,B84,449;%%"
}
@Article{Booth:1974ms,
     author    = "Booth, P. S. L. and others",
     title     = "{The Photoproduction of Neutral Pions from Protons at
                  Forward Angles in the Resonance Region}",
     journal   = "Nucl. Phys.",
     volume    = "B84",
     year      = "1975",
     pages     = "437",
     SLACcitation  = "%%CITATION = NUPHA,B84,437;%%"
}
@Article{Abrahamian:1975vs,
     author    = "Abrahamian, L. O. and others",
     title     = "{Inclusive Photoproduction of Protons and pi+- Mesons on
                  Nuclei at Average Energy of gammas=4.28-GeV}",
     journal   = "Sov. J. Nucl. Phys.",
     volume    = "23",
     year      = "1976",
     pages     = "394",
     SLACcitation  = "%%CITATION = SJNCA,23,394;%%"
}
@Article{Husmann:1977ar,
     author    = "Husmann, D. and Jansen, W. and Lohr, B. and Schilling, H.",
     title     = "{Forward Photoproduction of Neutral Pions on Protons in the
                  Third Resonance Region}",
     journal   = "Nucl. Phys.",
     volume    = "B126",
     year      = "1977",
     pages     = "436",
     SLACcitation  = "%%CITATION = NUPHA,B126,436;%%"
}
@Article{Abrahamian:1974jc,
     author    = "Abrahamian, L. O. and others",
     title     = "{Pi0 and pi+ Production with Polarized Photons in the
                  Energy Range 1-GeV - 2-GeV}",
     journal   = "Phys. Lett.",
     volume    = "B48",
     year      = "1974",
     pages     = "463",
     SLACcitation  = "%%CITATION = PHLTA,B48,463;%%"
}
@Article{Brefeld:1975dv,
     author    = "Brefeld, W. and others",
     title     = "{Forward Photoproduction of Neutral Pions from Protons in
                  the Resonance Region}",
     journal   = "Nucl. Phys.",
     volume    = "B100",
     year      = "1975",
     pages     = "93",
     SLACcitation  = "%%CITATION = NUPHA,B100,93;%%"
}

%G+DXS

@Article{Fischer:1970df,
     author    = "Fischer, G. and others",
     title     = "{Photoproduction of positive pions on hydrogen at photon
                  energies between 220 and 425 mev}",
     journal   = "Nucl. Phys.",
     volume    = "B16",
     year      = "1970",
     pages     = "119-124",
     SLACcitation  = "%%CITATION = NUPHA,B16,119;%%"
}
@Article{Fischer:1972mt,
     author    = "Fischer, G. and Von Holtey, G. and Knop, G. and Stuempfig,
                  J.",
     title     = "{Angular distributions of pions from gamma p $\to$ pi+ n at
                  photon energies between 220 and 425 mev}",
     journal   = "Z. Phys.",
     volume    = "253",
     year      = "1972",
     pages     = "38-52",
     SLACcitation  = "%%CITATION = ZEPYA,253,38;%%"
}
@Article{Buechler:1994jg,
     author    = "Buechler, K. and others",
     title     = "{Photoproduction of positive pions from hydrogen with
                  PHOENICS at ELSA}",
     journal   = "Nucl. Phys.",
     volume    = "A570",
     year      = "1994",
     pages     = "580-598",
     SLACcitation  = "%%CITATION = NUPHA,A570,580;%%"
}
@Article{Branford:1999cp,
     author    = "Branford, D. and others",
     title     = "{Nuclear pion photoproduction in the Delta resonance
                  region}",
     journal   = "Phys. Rev.",
     volume    = "C61",
     year      = "2000",
     pages     = "014603",
     SLACcitation  = "%%CITATION = PHRVA,C61,014603;%%"
}
@Article{Fujii:1976jg,
     author    = "Fujii, T. and others",
     title     = "{Photoproduction of Charged pi Mesons from Hydrogen and
                  Deuterium in the Energy Range Between 250-MeV and 790-
                  MeV}",
     journal   = "Nucl. Phys.",
     volume    = "B120",
     year      = "1977",
     pages     = "395",
     SLACcitation  = "%%CITATION = NUPHA,B120,395;%%"
}
@Article{Fujii:1971qe,
     author    = "Fujii, T. and others",
     title     = "{Charged-pi photoproduction at 180 degress in the energy
                  range between 300 and 1200 mev}",
     journal   = "Phys. Rev. Lett.",
     volume    = "26",
     year      = "1971",
     pages     = "1672-1675",
     SLACcitation  = "%%CITATION = PRLTA,26,1672;%%"
}
@Article{Dannhausen:2001yz,
     author    = "Dannhausen, H. W. and others",
     title     = "{Photoproduction of positive pions from hydrogen at large
                  angles in the energy range 0.3-GeV - 2.0-GeV}",
     journal   = "Eur. Phys. J.",
     volume    = "A11",
     year      = "2001",
     pages     = "441-455",
     SLACcitation  = "%%CITATION = EPHJA,A11,441;%%"
}
@Article{Betourne:1968bd,
     author    = "Betourne, C. and Bizot, J. C. and Perez-y-Jorba, J. P. and
                  Treille, Daniel and Schmidt, W.",
     title     = "{POSITIVE PION PHOTOPRODUCTION FROM HYDROGEN FOR INCIDENT
                  PHOTON ENERGIES 300-MEV - 750-MeV}",
     journal   = "Phys. Rev.",
     volume    = "172",
     year      = "1968",
     pages     = "1343-1353",
     SLACcitation  = "%%CITATION = PHRVA,172,1343;%%"
}
@Article{Aleksandrov:1970xq,
     author    = "Aleksandrov, Yu. M. and Grushin, V. F. and Leikin, E. M.
                  and Rotvain, A. Ya.",
     title     = "{Photoproduction of positive pions on protons in the region
                  of resonance p-33(1236)}",
     journal   = "Yad. Fiz.",
     volume    = "12",
     year      = "1970",
     pages     = "770-781",
     SLACcitation  = "%%CITATION = YAFIA,12,770;%%"
}
@Article{Faure:1984qe,
     author    = "Faure, J. L. and others",
     title     = "{CHARGED PION PHOTOPRODUCTION MEASUREMENT ON DEUTERIUM IN
                  THE DELTA (1236) REGION USING A QUASIMONOCHROMATIC PHOTON
                  BEAM}",
     journal   = "Nucl. Phys.",
     volume    = "A424",
     year      = "1984",
     pages     = "383",
     SLACcitation  = "%%CITATION = NUPHA,A424,383;%%"
}
@Article{Durwen:1980mq,
     author    = "Durwen, Ernst Josef",
     title     = "{DIFFERENTIAL CROSS-SECTION OF THE REACTION gamma p $\to$
                  pi+ n AT MEDIUM ANGLES IN THE gamma ENERGY RANGE FROM 0.3-
                  GEV TO 2.0-GEV AND PARAMETRIZATION THROUGH EXPANSION OF THE
                  LEGENDRE POLYNOMIAL}",
     note     = "BONN-IR-80-7"
}
@Article{Althoff:1983te,
     author    = "Althoff, K. H. and others",
     title     = "{POSITIVE PION PHOTOPRODUCTION FROM HYDROGEN AT PHOTON
                  ENERGIES BETWEEN 500-MeV AND 1400-MeV IN FORWARD
                  DIRECTION}",
     journal   = "Z. Phys.",
     volume    = "C18",
     year      = "1983",
     pages     = "199",
     SLACcitation  = "%%CITATION = ZEPYA,C18,199;%%"
}
@Article{PhysRev.159.1195,
  title = {$\pi{}^{+}$ Photoproduction from Hydrogen at Laboratory Energies from 589 to 1269 MeV},
  author = {Ecklund, S. D. and Walker, R. L.},
  journal = {Phys. Rev.},
  volume = {159},
  number = {5},
  pages = {1195--1209},
  numpages = {14},
  year = {1967},
  month = {Jul},
  doi = {10.1103/PhysRev.159.1195},
  publisher = {American Physical Society}
}
@Article{Ahrens:2006gp,
     author    = "Ahrens, J. and others",
     title     = "{Measurement of the helicity dependence for the gamma p
                  $\to$ n pi+ channel in the second resonance region}",
     journal   = "Phys. Rev.",
     volume    = "C74",
     year      = "2006",
     pages     = "045204",
     SLACcitation  = "%%CITATION = PHRVA,C74,045204;%%"
}
@Article{Ekstrand:1972rt,
     author    = "Ekstrand, K. and Browman, A. and Hand, L. and Nordberg, M.
                  E.",
     title     = "{Positive-pion photoproduction in the backward direction}",
     journal   = "Phys. Rev.",
     volume    = "D6",
     year      = "1972",
     pages     = "1-11",
     SLACcitation  = "%%CITATION = PHRVA,D6,1;%%"
}
@Article{PhysRevD.1.1946,
  title = {Photoproduction of Positive Pions at Backward Angles in the Energy Range 1-3 GeV},
  author = {Alvarez, R. A. and Cooperstein, G.  and Kalata, K.  and Lanza, R. C. and Luckey, D. },
  journal = {Phys. Rev. D},
  volume = {1},
  number = {7},
  pages = {1946--1960},
  numpages = {14},
  year = {1970},
  month = {Apr},
  doi = {10.1103/PhysRevD.1.1946},
  publisher = {American Physical Society}
}
@Article{Zhu:2004dy,
     author    = "Zhu, L. Y. and others",
 collaboration = "Jefferson Lab Hall A",
     title     = "{Cross section measurements of charged pion photoproduction
                  in hydrogen  and deuterium from 1.1-GeV to 5.5-GeV}",
     journal   = "Phys. Rev.",
     volume    = "C71",
     year      = "2005",
     pages     = "044603",
     SLACcitation  = "%%CITATION = NUCL-EX/0409018;%%"
}
@Article{PhysRevLett.17.1027,
  title = {Photoproduction of Single Positive Pions Between 1.2 and 3 GeV},
  author = {Buschhorn, G.  and Carroll, J.  and Eandi, R. D. and Heide, P.  and H\"ubner, R.  and Kern, W.  and K\"otz, U.  and Schm\"user, P.  and Skronn, H. J.},
  journal = {Phys. Rev. Lett.},
  volume = {17},
  number = {19},
  pages = {1027--1030},
  numpages = {3},
  year = {1966},
  month = {Nov},
  doi = {10.1103/PhysRevLett.17.1027},
  publisher = {American Physical Society}
}

%G0SIG

@Article{Blanpied:1992nn,
     author    = "Blanpied, G. and others",
 collaboration = "LEGS",
     title     = "{p (gamma (polarized) pi0) reaction and the E2 excitation
                  of the Delta}",
     journal   = "Phys. Rev. Lett.",
     volume    = "69",
     year      = "1992",
     pages     = "1880-1883",
     SLACcitation  = "%%CITATION = PRLTA,69,1880;%%"
}
@Article{Blanpied:2001ae,
     author    = "Blanpied, G. and others",
     title     = "{N ---> Delta transition and proton polarizabilities from
                  measurements of p( gamma polarized , gamma ), p( gamma
                  polarized , pi 0), and p( gamma polarized , pi +)}",
     journal   = "Phys. Rev.",
     volume    = "C64",
     year      = "2001",
     pages     = "025203",
     SLACcitation  = "%%CITATION = PHRVA,C64,025203;%%"
}
@Article{Belyaev:1983xf,
     author    = "Belyaev, A. a. and others",
     title     = "{EXPERIMENTAL STUDIES OF THE SIGMA, T, P POLARIZATION
                  PARAMETERS AND THE GAMMA P $\to$ P PI0 REACTION MULTIPOLE
                  ANALYSIS IN THE FIRST RESONANCE REGION}",
     journal   = "Nucl. Phys.",
     volume    = "B213",
     year      = "1983",
     pages     = "201-222",
     SLACcitation  = "%%CITATION = NUPHA,B213,201;%%"
}
@Article{Barbiellini:1970qu,
     author    = "Barbiellini, G. and others",
     title     = "{Photoproduction of pi0 on protons by polarized gamma
                  rays}",
     journal   = "Phys. Rev.",
     volume    = "184",
     year      = "1969",
     pages     = "1402-1413",
     SLACcitation  = "%%CITATION = PHRVA,184,1402;%%"
}
@Article{Adamian:2000yi,
     author    = "Adamian, F. V. and others",
     title     = "{Measurement of the cross section asymmetry of the reaction
                  gamma p -->  pi0 p in the resonance energy region E(gamma)
                  = 0.5-GeV - 1.1-GeV}",
     journal   = "Phys. Rev.",
     volume    = "C63",
     year      = "2001",
     pages     = "054606",
     SLACcitation  = "%%CITATION = NUCL-EX/0011006;%%"
}
@Article{Knies:1974zx,
     author    = "Knies, G. and others",
     title     = "{Measurement of Asymmetries in Polarized gamma + n $\to$ pi
                  + n, with E(gamma) from 600-MeV to 900-MeV}",
     journal   = "Phys. Rev.",
     volume    = "D10",
     year      = "1974",
     pages     = "2778",
     SLACcitation  = "%%CITATION = PHRVA,D10,2778;%%"
}
@Article{Bussey:1979wt,
     author    = "Bussey, P. J. and others",
     title     = "{POLARIZATION PARAMETERS IN NEUTRAL PION PHOTOPRODUCTION}",
     journal   = "Nucl. Phys.",
     volume    = "B154",
     year      = "1979",
     pages     = "492",
     SLACcitation  = "%%CITATION = NUPHA,B154,492;%%"
}
@Article{Bussey:1975mt,
     author    = "Bussey, P. J. and others",
     title     = "{A Measurement of the Beam Asymmetry Parameter Sigma for
                  Neutral Pion Photoproduction in the Energy Range 1.2-GeV-
                  2.8-GeV}",
     journal   = "Nucl. Phys.",
     volume    = "B104",
     year      = "1976",
     pages     = "253",
     SLACcitation  = "%%CITATION = NUPHA,B104,253;%%"
}

%G+SIG

@Article{Zabaev:1975ag,
     author    = "Zabaev, V. N. and others",
     title     = "{Production of pi+ Mesons Induced by Polarized Photons in
                  the Energy Range 220-MeV-280-MeV}",
     journal   = "Yad. Fiz.",
     volume    = "21",
     year      = "1975",
     pages     = "551-555",
     SLACcitation  = "%%CITATION = YAFIA,21,551;%%"
}
@Article{PhysRev.130.2429,
  title = {Positive Pion Production by Polarized X Rays between 227 and 373 MeV},
  author = {Smith, R. C. and Mozley, R. F.},
  journal = {Phys. Rev.},
  volume = {130},
  number = {6},
  pages = {2429--2440},
  numpages = {11},
  year = {1963},
  month = {Jun},
  doi = {10.1103/PhysRev.130.2429},
  publisher = {American Physical Society}
}
@Article{PhysRev.117.835,
  title = {Positive Pion Production by Polarized Bremsstrahlung},
  author = {Taylor, R. E. and Mozley, R. F.},
  journal = {Phys. Rev.},
  volume = {117},
  number = {3},
  pages = {835--845},
  numpages = {10},
  year = {1960},
  month = {Feb},
  doi = {10.1103/PhysRev.117.835},
  publisher = {American Physical Society}
}
@Article{Ganenko:1976ri,
     author    = "Ganenko, V. B. and others",
     title     = "{Asymmetry Angular Distributions of gamma p $\to$ p pi0
                  Reaction for 250-MeV-650-MeV Energies}",
     journal   = "Yad. Fiz.",
     volume    = "23",
     year      = "1976",
     pages     = "310-322",
     SLACcitation  = "%%CITATION = YAFIA,23,310;%%"
}
@Article{Getman:1981qt,
     author    = "Getman, V. A. and others",
     title     = "{POSITIVE PION PRODUCTION FROM POLARIZED PROTONS BY
                  LINEARLY POLARIZED PHOTONS IN THE ENERGY RANGE 280-MEV -
                  420-MEV}",
     journal   = "Nucl. Phys.",
     volume    = "B188",
     year      = "1981",
     pages     = "397-413",
     SLACcitation  = "%%CITATION = NUPHA,B188,397;%%"
}
@Article{Ajaka:2000rj,
     author    = "Ajaka, J. and others",
 collaboration = "GRAAL",
     title     = "{Precise measurement of Sigma beam asymmetry for positive
                  pion  photoproduction on the proton from 550-MeV to 1100-
                  MeV}",
     journal   = "Phys. Lett.",
     volume    = "B475",
     year      = "2000",
     pages     = "372-377",
     SLACcitation  = "%%CITATION = PHLTA,B475,372;%%"
}
@Article{Alspector:1972pw,
     author    = "Alspector, J. and others",
     title     = "{Pi+- and pi0 production by polarized photons in the
                  resonance region}",
     journal   = "Phys. Rev. Lett.",
     volume    = "28",
     year      = "1972",
     pages     = "1403-1406",
     SLACcitation  = "%%CITATION = PRLTA,28,1403;%%"
}
@Article{Muhlich:2003tj,
     author    = "Muhlich, P. and Falter, T. and Mosel, U.",
     title     = "{Inclusive omega photoproduction off nuclei}",
     journal   = "Eur. Phys. J.",
     volume    = "A20",
     year      = "2004",
     pages     = "499-508",
     SLACcitation  = "%%CITATION = NUCL-TH/0310067;%%"
}
@Article{Chen:2007cy,
     author    = "Chen, Guan Yeu and Kamalov, S. S. and Yang, Shin Nan and
                  Drechsel, D. and Tiator, L.",
     title     = "{Nucleon resonances in \pi N scattering up to energies
                  \sqrt(s) < 2.0 GeV}",
     journal   = "Phys. Rev.",
     volume    = "C76",
     year      = "2007",
     pages     = "035206",
     SLACcitation  = "%%CITATION = NUCL-TH/0703096;%%"
}
@Article{Yang:1985yr,
     author    = "Yang, Shin-Nan",
     title     = "{A PHENOMENOLOGICAL HAMILTONIAN FOR THE PION
                  PHOTOPRODUCTION REACTION AND PI NUCLEUS DYNAMICS}",
     journal   = "J. Phys.",
     volume    = "G11",
     year      = "1985",
     pages     = "L205-L210",
     SLACcitation  = "%%CITATION = JPHGB,G11,L205;%%"
}
@Article{Yang:1989si,
     author    = "Yang, S. N.",
     title     = "{Pion - nucleon interaction and neutral pion
                  photoproduction on the proton near threshold. (Erratum)}",
     journal   = "Phys. Rev.",
     volume    = "C40",
     year      = "1989",
     pages     = "1810-1813",
     SLACcitation  = "%%CITATION = PHRVA,C40,1810;%%"
}
@Article{Lee:1991dd,
     author    = "Lee, Chau- Chen and Yang, Shin- Nan and Lee, T. S. H.",
     title     = "{Meson exchange pi N model and neutral pion photoproduction
                  from protons near threshold}",
     journal   = "J. Phys.",
     volume    = "G17",
     year      = "1991",
     pages     = "L131-L137",
     SLACcitation  = "%%CITATION = JPHGB,G17,L131;%%"
}
@Article{Nozawa:1990vd,
     author    = "Nozawa, S. and Lee, T. S. H.",
     title     = "{ELECTROPRODUCTION OF PIONS ON THE NUCLEON. 2: POLARIZATION
                  OBSERVABLES}",
     journal   = "Nucl. Phys.",
     volume    = "A513",
     year      = "1990",
     pages     = "543-556",
     SLACcitation  = "%%CITATION = NUPHA,A513,543;%%"
}
@Article{Krehl:1999km,
     author    = "Krehl, O. and Hanhart, C. and Krewald, S. and Speth, J.",
     title     = "{What is the structure of the Roper resonance?}",
     journal   = "Phys. Rev.",
     volume    = "C62",
     year      = "2000",
     pages     = "025207",
     SLACcitation  = "%%CITATION = NUCL-TH/9911080;%%"
}
@Article{Hohler:1974ht,
     author    = "Hohler, G. and Pietarinen, E.",
     title     = "{The rho N N Vertex in Vector Dominance Models}",
     journal   = "Nucl. Phys.",
     volume    = "B95",
     year      = "1975",
     pages     = "210",
     doi       = "10.1016/0550-3213(75)90042-5",
     SLACcitation  = "%%CITATION = NUPHA,B95,210;%%"
}
@Article{Pietarinen:1976gt,
     author    = "Pietarinen, E.",
     title     = "{Partial Wave Analysis of pi n Scattering Using Dispersion
                  Relations}",
     note     = "HU-TFT-76-17"
}
@Article{Grein:1977id,
     author    = "Grein, W.",
     title     = "{Analysis of the n n and n anti-N Forward Scattering
                  Amplitudes Including Information from pi pi and pi n
                  Scattering}",
     journal   = "Nucl. Phys.",
     volume    = "B131",
     year      = "1977",
     pages     = "255",
     doi       = "10.1016/0550-3213(77)90372-8",
     SLACcitation  = "%%CITATION = NUPHA,B131,255;%%"
}
@Article{Grein:1979nw,
     author    = "Grein, W. and Kroll, P.",
     title     = "{Two Pion and Three Pion Cut Contributions to Nucleon-
                  Nucleon Scattering}",
     journal   = "Nucl. Phys.",
     volume    = "A338",
     year      = "1980",
     pages     = "332",
     doi       = "10.1016/0375-9474(80)90036-6",
     SLACcitation  = "%%CITATION = NUPHA,A338,332;%%"
}
@Article{Hamilton:1983ri,
     author    = "Hamilton, J. and Oades, G. C.",
     title     = "{THE SHORT RANGE NUCLEON-NUCLEON REPULSION}",
     journal   = "Nucl. Phys.",
     volume    = "A424",
     year      = "1984",
     pages     = "447",
     doi       = "10.1016/0375-9474(84)90005-8",
     SLACcitation  = "%%CITATION = NUPHA,A424,447;%%"
}
@Article{Einstein:1905ve,
     author    = "Einstein, Albert",
     title     = "{On the electrodynamics of moving bodies}",
     journal   = "Annalen Phys.",
     volume    = "17",
     year      = "1905",
     pages     = "891-921",
     doi       = "10.1002/andp.200590006",
     SLACcitation  = "%%CITATION = ANPYA,17,891;%%"
}
@Article{Goldrich:1972jh,
     author    = "Goldrich, F. and Wigner, Eugene P.",
     title     = "{ON THE OBSERVABILITY OF THE COLLISION MATRIX. (TALK)}",
     note     = "In *J R Klauder, Magic Without Magic*, San Francisco 1972,
                  147-160"
}
@Article{Kelkar:2008na,
     author    = "Kelkar, N. G. and Nowakowski, M.",
     title     = "{Analysis of averaged multichannel delay times}",
     journal   = "Phys. Rev.",
     volume    = "A78",
     year      = "2008",
     pages     = "012709",
     doi       = "10.1103/PhysRevA.78.012709"
}
@Article{Smith:1960zza,
     author    = "Smith, Felix T.",
     title     = "{Lifetime Matrix in Collision Theory}",
     journal   = "Phys. Rev.",
     volume    = "118",
     year      = "1960",
     pages     = "349-356",
     doi       = "10.1103/PhysRev.118.349",
     SLACcitation  = "%%CITATION = PHRVA,118,349;%%"
}
@Article{Wigner:1955zz,
     author    = "Wigner, Eugene P.",
     title     = "{Lower Limit for the Energy Derivative of the Scattering
                  Phase Shift}",
     journal   = "Phys. Rev.",
     volume    = "98",
     year      = "1955",
     pages     = "145-147",
     doi       = "10.1103/PhysRev.98.145",
     SLACcitation  = "%%CITATION = PHRVA,98,145;%%"
}
@article{Wigner:1947zz,
      author         = "Wigner, E.P. and Eisenbud, L.",
      title          = "{Higher Angular Momenta and Long Range Interaction in
                        Resonance Reactions}",
      journal        = "Phys.Rev.",
      volume         = "72",
      pages          = "29-41",
      doi            = "10.1103/PhysRev.72.29",
      year           = "1947",
      SLACcitation   = "%%CITATION = PHRVA,72,29;%%",
}
@phdthesis{Eisenbud:1944,
  author =	 "L. Eisenbud",
  title =	 "The Formal Properties of Nuclear Collisions",
  school =	 "Princeton University",
  address =	 "Princeton, New Jersey",
  year =	 1944
}
@Article{Arndt:1985vj,
     author    = "Arndt, Richard A. and Ford, John M. and Roper, L. David",
     title     = "{PION - NUCLEON PARTIAL WAVE ANALYSIS TO 1100-MeV}",
     journal   = "Phys. Rev.",
     volume    = "D32",
     year      = "1985",
     pages     = "1085",
     doi       = "10.1103/PhysRevD.32.1085",
     SLACcitation  = "%%CITATION = PHRVA,D32,1085;%%"
}
@Article{Aaron:1970xk,
     author    = "Aaron, R. and Teplitz, D. C. and Amado, R. D. and Young, J.
                  E.",
     title     = "{Theory of the d-13 pion-nucleon amplitude}",
     journal   = "Phys. Rev.",
     volume    = "187",
     year      = "1969",
     pages     = "2047-2051",
     doi       = "10.1103/PhysRev.187.2047",
     SLACcitation  = "%%CITATION = PHRVA,187,2047;%%"
}
@Article{Aaron:1969my,
     author    = "Aaron, R. and Amado, R. D. and Young, J. E.",
     title     = "{Relativistic three-body theory with applications to pi-
                  minus n scattering}",
     journal   = "Phys. Rev.",
     volume    = "174",
     year      = "1968",
     pages     = "2022-2032",
     doi       = "10.1103/PhysRev.174.2022",
     SLACcitation  = "%%CITATION = PHRVA,174,2022;%%"
}
@Article{PhysRev.174.2022,
  title = {Relativistic Three-Body Theory with Applications to $\pi{}-N$ Scattering},
  author = {Aaron, R.  and Amado, R. D. and Young, J. E.},
  journal = {Phys. Rev.},
  volume = {174},
  number = {5},
  pages = {2022--2032},
  numpages = {10},
  year = {1968},
  month = {Oct},
  doi = {10.1103/PhysRev.174.2022},
  publisher = {American Physical Society}
}
@Article{Bakamjian:1953kh,
     author    = "Bakamjian, B. and Thomas, L. H.",
     title     = "{Relativistic particle dynamics. 2}",
     journal   = "Phys. Rev.",
     volume    = "92",
     year      = "1953",
     pages     = "1300-1310",
     SLACcitation  = "%%CITATION = PHRVA,92,1300;%%"
}
@Article{Heller:1976wd,
     author    = "Heller, L. and Bohannon, G. E. and Tabakin, F.",
     title     = "{Dependence of the Off Energy Shell T Matrix on the Total
                  Three Momentum}",
     journal   = "Phys. Rev.",
     volume    = "C13",
     year      = "1976",
     pages     = "742-748",
     SLACcitation  = "%%CITATION = PHRVA,C13,742;%%"
}
@Article{Adler:1969gk,
     author    = "Adler, Stephen L.",
     title     = "{Axial vector vertex in spinor electrodynamics}",
     journal   = "Phys. Rev.",
     volume    = "177",
     year      = "1969",
     pages     = "2426-2438",
     doi       = "10.1103/PhysRev.177.2426",
     SLACcitation  = "%%CITATION = PHRVA,177,2426;%%"
}
@Article{Heitler:1941a,
     author    = "Heitler, W.",
     title     = "{The influence of radiation damping on the scattering of light and mesons by free particles. I}",
     journal   = "Math.\ Proc.\ Camb.\ Phil.\ Soc.",
     volume    = "37",
     year      = "1941",
     pages     = "291-300",
     doi       = "10.1017/S0305004100021770"
}
@Book{Weinberg:1995mt,
     author    = "Weinberg, Steven",
     title     = "{The Quantum theory of fields. Vol. 1: Foundations}",
     publisher = "{Cambridge, UK: Univ. Pr. 609 pp.}",
     year      = "1995"
}
@Article{Green:1997yia,
     author    = "Green, Anthony M. and Wycech, S.",
     title     = "{The eta nucleon scattering length and effective range}",
     journal   = "Phys. Rev.",
     volume    = "C55",
     year      = "1997",
     pages     = "2167-2170",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.55.R2167",
     SLACcitation  = "%%CITATION = NUCL-TH/9703009;%%"
}
@Article{Green:1999iq,
     author    = "Green, Anthony M. and Wycech, S.",
     title     = "{A coupled K-matrix description of the reactions pi N -->
                  pi N, pi N  --> eta N, gamma N --> pi N and gamma N --> eta
                  N}",
     journal   = "Phys. Rev.",
     volume    = "C60",
     year      = "1999",
     pages     = "035208",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.60.035208",
     SLACcitation  = "%%CITATION = NUCL-TH/9905011;%%"
}
@Article{Arndt:1998nm,
     author    = "Arndt, R. A. and Green, Anthony M. and Workman, R. L. and
                  Wycech, S.",
     title     = "{The energies and residues of the nucleon resonances
                  N(1535) and  N(1650)}",
     journal   = "Phys. Rev.",
     volume    = "C58",
     year      = "1998",
     pages     = "3636-3640",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.58.3636",
     SLACcitation  = "%%CITATION = NUCL-TH/9807009;%%"
}
@Article{Crede:2003ax,
     author    = "Crede, Volker and others",
 collaboration = "CB-ELSA",
     title     = "{Photoproduction of eta mesons off protons for 0.75-GeV <
                  E(gamma) <  3-GeV}",
     journal   = "Phys. Rev. Lett.",
     volume    = "94",
     year      = "2005",
     pages     = "012004",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevLett.94.012004",
     SLACcitation  = "%%CITATION = HEP-EX/0311045;%%"
}
@Article{Nakabayashi:2006ut,
     author    = "Nakabayashi, T. and others",
     title     = "{Photoproduction of eta mesons off protons for Egamma <=
                  1.15-GeV}",
     journal   = "Phys. Rev.",
     volume    = "C74",
     year      = "2006",
     pages     = "035202",
     doi       = "10.1103/PhysRevC.74.035202",
     SLACcitation  = "%%CITATION = PHRVA,C74,035202;%%"
}
@Article{Williams:2009yj,
     author    = "Williams, M. and others",
 collaboration = "CLAS",
     title     = "{Differential cross sections for the reactions gamma p-> p
                  eta and gamma p -> p eta-prime}",
     journal   = "Phys. Rev.",
     volume    = "C80",
     year      = "2009",
     pages     = "045213",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-ex",
     doi       = "10.1103/PhysRevC.80.045213",
     SLACcitation  = "%%CITATION = 0909.0616;%%"
}
@Article{Ajaka:1998zi,
     author    = "Ajaka, J. and others",
     title     = "{New measurement of Sigma beam asymmetry for eta meson
                  photoproduction  on the proton}",
     journal   = "Phys. Rev. Lett.",
     volume    = "81",
     year      = "1998",
     pages     = "1797-1800",
     doi       = "10.1103/PhysRevLett.81.1797",
     SLACcitation  = "%%CITATION = PRLTA,81,1797;%%"
}
@Article{Gutz:2008zz,
     author    = "Gutz, E. and others",
 collaboration = "CBELSA",
     title     = "{Measurement of the beam asymmetry Sigma in pi eta:
                  Production off the proton with the CBELSA/TAPS
                  experiment}",
     journal   = "Eur. Phys. J.",
     volume    = "A35",
     year      = "2008",
     pages     = "291-293",
     doi       = "10.1140/epja/i2008-10566-9",
     SLACcitation  = "%%CITATION = EPHJA,A35,291;%%"
}
@Article{Dugger:2010etaprop,
     author    = "M.\ Dugger and others",
 collaboration = "CLAS",
     title     = "{Measurement of polarization observables in
                  $\eta-$photoproduction with CLAS}",
     year      = "2004",
  url        = {http://www.jlab.org/exp_prog/proposals/05/PR05-012.ps}
}
@Article{Haider:2009yf,
     author    = "Haider, Q. and Liu, L. C.",
     title     = "{Eta-Mesic Nucleus: A New Form of Nuclear Matter}",
     journal   = "Acta Phys. Polon. Supp.",
     volume    = "2",
     year      = "2009",
     pages     = "121-132",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-th",
     SLACcitation  = "%%CITATION = 0902.4248;%%"
}
@Article{PhysRevC.34.1845,
  title = {Signature for the existence of eta-mesic nucleus},
  author = {Liu, L. C. and Haider, Q. },
  journal = {Phys. Rev. C},
  volume = {34},
  number = {5},
  pages = {1845--1854},
  numpages = {9},
  year = {1986},
  month = {Nov},
  doi = {10.1103/PhysRevC.34.1845},
  publisher = {American Physical Society}
}
@Article{Cheng:1987yw,
     author    = "Cheng, W. K. and Kuo, T. T. S. and Li, G. L.",
     title     = "On formation of eta meson-nucleus bound states",
     journal   = "Phys. Lett.",
     volume    = "B195",
     year      = "1987",
     pages     = "515",
     doi       = "10.1016/0370-2693(87)91564-4",
     SLACcitation  = "%%CITATION = PHLTA,B195,515;%%"
}
@Article{Prakhov:2005qb,
     author    = "Prakhov, S. and others",
     title     = "{Measurement of pi- p $\to$ eta n from threshold to p (pi-)
                  = 747-MeV/c}",
     journal   = "Phys. Rev.",
     volume    = "C72",
     year      = "2005",
     pages     = "015203",
     doi       = "10.1103/PhysRevC.72.015203",
     SLACcitation  = "%%CITATION = PHRVA,C72,015203;%%"
}
@Article{Basdevant:1978tx,
     author    = "Basdevant, J. -L. and Berger, Edmond L.",
     title     = "{UNSTABLE PARTICLE SCATTERING AND AN ANALYTIC QUASIUNITARY
                  ISOBAR MODEL}",
     journal   = "Phys. Rev.",
     volume    = "D19",
     year      = "1979",
     pages     = "239",
     doi       = "10.1103/PhysRevD.19.239",
     SLACcitation  = "%%CITATION = PHRVA,D19,239;%%"
}
@Article{Edwards:1980sa,
     author    = "Edwards, Bonnie J. and Thomas, Gerald H.",
     title     = "{INELASTIC THRESHOLDS AND DIBARYON RESONANCES}",
     journal   = "Phys. Rev.",
     volume    = "D22",
     year      = "1980",
     pages     = "2772",
     doi       = "10.1103/PhysRevD.22.2772",
     SLACcitation  = "%%CITATION = PHRVA,D22,2772;%%"
}
@Article{Kaiser:1996js,
     author    = "Kaiser, Norbert and Waas, T. and Weise, W.",
     title     = "{SU(3) chiral dynamics with coupled channels: Eta and kaon
                  photoproduction}",
     journal   = "Nucl. Phys.",
     volume    = "A612",
     year      = "1997",
     pages     = "297-320",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(96)00321-1",
     SLACcitation  = "%%CITATION = HEP-PH/9607459;%%"
}
@Article{Aznauryan:2003zg,
     author    = "Aznauryan, I. G.",
     title     = "{Resonance contributions to eta photoproduction on protons
                  found using  dispersion relations and an isobar model}",
     journal   = "Phys. Rev.",
     volume    = "C68",
     year      = "2003",
     pages     = "065204",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.68.065204",
     SLACcitation  = "%%CITATION = NUCL-TH/0306079;%%"
}
@Article{Knochlein:1995qz,
     author    = "Knochlein, G. and Drechsel, D. and Tiator, L.",
     title     = "{Photoproduction and electroproduction of eta mesons}",
     journal   = "Z. Phys.",
     volume    = "A352",
     year      = "1995",
     pages     = "327-343",
     archivePrefix = "arXiv",
     doi       = "10.1007/BF01289506",
     SLACcitation  = "%%CITATION = NUCL-TH/9506029;%%"
}
@Article{Chiang:2001as,
     author    = "Chiang, Wen-Tai and Yang, Shin-Nan and Tiator, Lothar and
                  Drechsel, Dieter",
     title     = "{An isobar model for eta photo- and electroproduction on
                  the nucleon}",
     journal   = "Nucl. Phys.",
     volume    = "A700",
     year      = "2002",
     pages     = "429-453",
     archivePrefix = "arXiv",
     doi       = "10.1016/S0375-9474(01)01325-2",
     SLACcitation  = "%%CITATION = NUCL-TH/0110034;%%"
}
@Article{Eden:1952aa,
     author    = "R.\ J.\ Eden",
     title     = "{Threshold behavior in quantum field theory}",
     journal   = "Proc. Royal Soc. of London",
     volume    = "210",
     year      = "1952",
     pages     = "388-404"
}
@Article{Zimmerman:1961aa,
     author    = "W.\ Zimmerman",
     title     = "{Analytic behavior of the scattering amplitude at zero
                  energy}",
     journal   = "Nuovo Cim.",
     volume    = "21",
     year      = "1961",
     pages     = "249-273"
}
@Article{Polkinghorne:1962aa,
     author    = "J.\ C.\ Polkinghorne",
     title     = "Analyticity and unitarity",
     journal   = "Nuovo Cim.",
     volume    = "23",
     year      = "1962",
     pages     = "360-367"
}
@Article{Boyling:1964aa,
     author    = "J.\ B.\ Boyling",
     title     = "Hermitian analyticity and extended unitarity in S-matrix
                  theory",
     journal   = "Nuovo Cim.",
     volume    = "33",
     year      = "1964",
     pages     = "1356-1373"
}
@Article{Bjorken:1960zz,
     author    = "Bjorken, J. D.",
     title     = "{Construction of Coupled Scattering and Production
                  Amplitudes Satisfying Analyticity and Unitarity}",
     journal   = "Phys. Rev. Lett.",
     volume    = "4",
     year      = "1960",
     pages     = "473-474",
     doi       = "10.1103/PhysRevLett.4.473",
     SLACcitation  = "%%CITATION = PRLTA,4,473;%%"
}
@Book{Goldberger:1964aa,
     author    = "M.\ L.\ Goldberger and K.\ M.\ Watson",
     title     = "Collision Theory",
     publisher = "John Wiley and Sons, Inc., New York",
     year      = "1964"
}
@Article{Weinberg:1964zz,
     author    = "Weinberg, Steven",
     title     = "{Systematic Solution of Multiparticle Scattering
                  Problems}",
     journal   = "Phys. Rev.",
     volume    = "133",
     year      = "1964",
     pages     = "B232-B256",
     doi       = "10.1103/PhysRev.133.B232",
     SLACcitation  = "%%CITATION = PHRVA,133,B232;%%"
}
@Article{Mandelstam:1958xc,
     author    = "Mandelstam, S.",
     title     = "{Determination of the pion - nucleon scattering amplitude
                  from dispersion relations and unitarity. General theory}",
     journal   = "Phys. Rev.",
     volume    = "112",
     year      = "1958",
     pages     = "1344-1360",
     doi       = "10.1103/PhysRev.112.1344",
     SLACcitation  = "%%CITATION = PHRVA,112,1344;%%"
}
@Article{Frautschi:1960aa,
     author    = "S.\ C.\ Frautschi and J.\ D.\ Walecka",
     title     = "Pion-nucleon scattering in the Mandelstam representation",
     journal   = "Phys. Rev.",
     volume    = "120",
     year      = "1960",
     pages     = "1486-1505"
}
@Article{Chew:1960iv,
     author    = "Chew, Geoffrey F. and Mandelstam, Stanley",
     title     = "{Theory of low-energy pion pion interactions}",
     journal   = "Phys. Rev.",
     volume    = "119",
     year      = "1960",
     pages     = "467-477",
     doi       = "10.1103/PhysRev.119.467",
     SLACcitation  = "%%CITATION = PHRVA,119,467;%%"
}
@Article{Arndt:1968sm,
     author    = "Arndt, R. A.",
     title     = "{Possible existence of a spin-2 Regge recurrence of the
                  $^1S_0$ $p-p$ pole (the unbound diproton)}",
     journal   = "Phys. Rev.",
     volume    = "165",
     year      = "1968",
     pages     = "1834-1838",
     doi       = "10.1103/PhysRev.165.1834",
     SLACcitation  = "%%CITATION = PHRVA,165,1834;%%"
}
@Article{Bjorken:1961nd,
     author    = "J.\ D.\ Bjorken and M.\ Nauenberg",
     title     = "{Symmetry of the $ND^{-1}$ solutions for coupled
                  scattering amplitudes}",
     journal   = "Phys. Rev.",
     volume    = "121",
     year      = "1961",
     pages     = "1250-1250"
}
@Article{Ceci:2006jj,
     author    = "Ceci, S. and Svarc, A. and Zauner, B. and Manley, M. and
                  Capstick, S.",
     title     = "{Model-independent resonance parameter extraction using the
                  trace of K and T matrices}",
     journal   = "Phys. Lett.",
     volume    = "B659",
     year      = "2008",
     pages     = "228-233",
     archivePrefix = "arXiv",
     doi       = "10.1016/j.physletb.2007.11.003",
     SLACcitation  = "%%CITATION = HEP-PH/0611094;%%"
}
@Book{Martin:1970bb,
     author    = "A.\ D. Martin and T.\ D.\ Spearman",
     title     = "Elementary particle theory",
     publisher = "North Holland Publishing Co., Amsterdam",
     year      = "1970"
}
@Article{Davidson:1990yk,
     author    = "Davidson, R. M. and Mukhopadhyay, N. C.",
     title     = "{Model independent determination of K matrix poles and
                  residues in the Delta (1232) region from the multipole data
                  for pion photoproduction}",
     journal   = "Phys. Rev.",
     volume    = "D42",
     year      = "1990",
     pages     = "20-29",
     doi       = "10.1103/PhysRevD.42.20",
     SLACcitation  = "%%CITATION = PHRVA,D42,20;%%"
}
@Article{Arndt:1989ww,
     author    = "Arndt, Richard A. and Workman, Ron L. and Li, Zhujun and
                  Roper, L. David",
     title     = "{PARTIAL WAVE ANALYSIS OF PION PHOTOPRODUCTION}",
     journal   = "Phys. Rev.",
     volume    = "C42",
     year      = "1990",
     pages     = "1853-1863",
     doi       = "10.1103/PhysRevC.42.1853",
     SLACcitation  = "%%CITATION = PHRVA,C42,1853;%%"
}
@Article{Arndt:1990ej,
     author    = "Arndt, R. A. and Workman, R. L. and Li, Z. and Roper, L. D.
                  ",
     title     = "{Pion photoproduction resonance couplings in the second
                  resonance region}",
     journal   = "Phys. Rev.",
     volume    = "C42",
     year      = "1990",
     pages     = "1864-1866",
     doi       = "10.1103/PhysRevC.42.1864",
     SLACcitation  = "%%CITATION = PHRVA,C42,1864;%%"
}
@Article{Arndt:1995bj,
     author    = "Arndt, Richard A. and Strakovsky, Igor I. and Workman, Ron
                  L. and Pavan, Marcello M.",
     title     = "{Updated analysis of pi N elastic scattering data to 2.1-
                  GeV: The Baryon spectrum}",
     journal   = "Phys. Rev.",
     volume    = "C52",
     year      = "1995",
     pages     = "2120-2130",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.52.2120",
     SLACcitation  = "%%CITATION = NUCL-TH/9505040;%%"
}
@Article{Watson:1952ji,
     author    = "Watson, Kenneth M.",
     title     = "{The Effect of final state interactions on reaction cross-
                  sections}",
     journal   = "Phys. Rev.",
     volume    = "88",
     year      = "1952",
     pages     = "1163-1171",
     doi       = "10.1103/PhysRev.88.1163",
     SLACcitation  = "%%CITATION = PHRVA,88,1163;%%"
}
@Article{Workman:2005eu,
     author    = "Workman, Ron L.",
     title     = "{Single-channel fits and K-matrix constraints}",
     journal   = "Phys. Rev.",
     volume    = "C74",
     year      = "2006",
     pages     = "055207",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.74.055207",
     SLACcitation  = "%%CITATION = NUCL-TH/0510025;%%"
}
@Article{Frazer:1960zz,
     author    = "Frazer, William R. and Fulco, Jose R.",
     title     = "{Partial-Wave Dispersion Relations for Pion-Nucleon
                  Scattering}",
     journal   = "Phys. Rev.",
     volume    = "119",
     year      = "1960",
     pages     = "1420-1426",
     doi       = "10.1103/PhysRev.119.1420",
     SLACcitation  = "%%CITATION = PHRVA,119,1420;%%"
}
@Article{Chiang:2002vq,
     author    = "Chiang, Wen-Tai and Yang, Shin Nan and Tiator, L. and
                  Vanderhaeghen, M. and Drechsel, D.",
     title     = "{A reggeized model for eta and eta' photoproduction}",
     journal   = "Phys. Rev.",
     volume    = "C68",
     year      = "2003",
     pages     = "045202",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.68.045202",
     SLACcitation  = "%%CITATION = NUCL-TH/0212106;%%"
}
@misc{Arndt:2009pc,
   author = "R.\ A.\ Arndt",
   year = {2009}, 
   howpublished = "private communication",
}
@misc{Arndt:2007pc,
   author = "R.\ A.\ Arndt",
   year = {2007}, 
   howpublished = "private communication",
}
@Article{Tabakin:1988wi,
     author    = "Tabakin, Frank and Dytman, Steven A. and Rosenthal, A. S.",
     title     = "{PHOTOPRODUCTION OF ETA MESONS}",
     note      = "Presented at Topical Conf. on Excited Baryons Troy, N.Y., Aug 4-6",
     year      = "1988"
}
@Article{HoffmannRothe:1995pk,
     author    = "Hoffmann-Rothe, P. and Saghai, B. and Tabakin, F.",
     title     = "{eta mesons photoproduction on the proton}",
     note      = "Presented at Few Body Problems Conf., Peniscola, Spain, Jun
                  5-9",
     year      = "1995"
}
@Article{Tiator:1999gr,
     author    = "Tiator, L. and Drechsel, D. and Knochlein, G. and Bennhold,
                  C.",
     title     = "{Analysis of resonance multipoles from polarization
                  observables in eta photoproduction}",
     journal   = "Phys. Rev.",
     volume    = "C60",
     year      = "1999",
     pages     = "035210",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.60.035210",
     SLACcitation  = "%%CITATION = NUCL-TH/9902028;%%"
}
@Article{Tiator:1998qp,
     author    = "Tiator, Lothar and Knochlein, Germar and Bennhold,
                  Cornelius",
     title     = "{Eta photoproduction}",
     journal   = "PiN Newslett.",
     volume    = "14",
     year      = "1998",
     pages     = "70-78",
     archivePrefix = "arXiv",
     SLACcitation  = "%%CITATION = NUCL-TH/9802064;%%"
}
@misc{SAID:ssh,
     note      = "{The {\sc said} interactive suite of codes is available
	           by secure shell interface via:
		   {\tt ssh -C -X said@said.phys.gwu.edu}.}"
}
@Article{Arndt:2001si,
     author    = "Arndt, R. A. and Strakovsky, I. I. and Workman, R. L.",
     title     = "{Analysis of pion electroproduction data}",
     journal   = "PiN Newslett.",
     volume    = "16",
     year      = "2002",
     pages     = "150-153",
     archivePrefix = "arXiv",
     SLACcitation  = "%%CITATION = NUCL-TH/0110001;%%"
}
@Article{Koch:1985bp,
     author    = "Koch, R.",
     title     = "{IMPROVED pi N PARTIAL WAVES CONSISTENT WITH ANALYTICITY
                  AND UNITARITY}",
     journal   = "Z. Phys.",
     volume    = "C29",
     year      = "1985",
     pages     = "597",
     doi       = "10.1007/BF01560295",
     SLACcitation  = "%%CITATION = ZEPYA,C29,597;%%"
}
@Article{Arndt:2003if,
     author    = "Arndt, R. A. and Briscoe, W. J. and Strakovsky, I. I. and
                  Workman, R. L. and Pavan, M. M.",
     title     = "{Dispersion Relation Constrained Partial Wave Analysis of
                  piN Elastic and piN\to\etaN Scattering Data: The Baryon
                  Spectrum}",
     journal   = "Phys. Rev.",
     volume    = "C69",
     year      = "2004",
     pages     = "035213",
     archivePrefix = "arXiv",
     doi       = "10.1103/PhysRevC.69.035213",
     SLACcitation  = "%%CITATION = NUCL-TH/0311089;%%"
}
@Article{Drechsel:2007if,
     author    = "Drechsel, D. and Kamalov, S. S. and Tiator, L.",
     title     = "{Unitary Isobar Model - MAID2007}",
     journal   = "Eur. Phys. J.",
     volume    = "A34",
     year      = "2007",
     pages     = "69-97",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-th",
     doi       = "10.1140/epja/i2007-10490-6",
     SLACcitation  = "%%CITATION = 0710.0306;%%"
}
@Article{McGeorge:2007tg,
     author    = "McGeorge, J. C. and others",
     title     = "{Upgrade of the Glasgow photon tagging spectrometer for
                  Mainz MAMI-C}",
     journal   = "Eur. Phys. J.",
     volume    = "A37",
     year      = "2008",
     pages     = "129-137",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-ex",
     doi       = "10.1140/epja/i2007-10606-0",
     SLACcitation  = "%%CITATION = 0711.3443;%%"
}
@Article{Crede:2009zz,
     author    = "Crede, V. and others",
 collaboration = "CBELSA/TAPS",
     title     = "{Photoproduction of eta and eta-prime mesons off protons}",
     journal   = "Phys. Rev.",
     volume    = "C80",
     year      = "2009",
     pages     = "055202",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-ex",
     doi       = "10.1103/PhysRevC.80.055202",
     SLACcitation  = "%%CITATION = 0909.1248;%%"
}
@misc{Green:note,
     note      = "{The $K$ matrix approach of Refs.\cite{Green:1997yia,
                   Arndt:1998nm,
                   Green:1999iq} include contributions to the hadronic $T$ 
		   matrix which represent the $\pi\pi\!N$ channel, though the 
		   three-body cut is not accounted for properly.}"
}
@Article{Workman:2008iv,
     author    = "Workman, R. L. and Arndt, R. A. and Paris, M. W.",
     title     = "{Resonance parameters from K-matrix and T-matrix poles}",
     journal   = "Phys. Rev.",
     volume    = "C79",
     year      = "2009",
     pages     = "038201",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-th",
     doi       = "10.1103/PhysRevC.79.038201",
     SLACcitation  = "%%CITATION = 0808.2176;%%"
}
@Article{Babelon:1976kv,
     author    = "Babelon, O. and Basdevant, J. -L. and Caillerie, D. and
                  Mennessier, G.",
     title     = "{Unitarity and Inelastic Final State Interactions}",
     journal   = "Nucl. Phys.",
     volume    = "B113",
     year      = "1976",
     pages     = "445",
     doi       = "10.1016/0550-3213(76)90137-1",
     SLACcitation  = "%%CITATION = NUPHA,B113,445;%%"
}
@Book{Eden:1966sm,
     author    = "R.\ J.\ Eden and P.\ V.\ Landshoff and D.\ I.\ Olive 
	          and J.\ C.\ Polkinghorne",
     title     = "The Analytic $S$-matrix",
     publisher = "Cambridge University Press, Cambridge",
     year      = "1966",
     note      = "pp.\ 231--232"
}
@Book{Eden:1966sm-1,
     author    = "R.\ J.\ Eden and P.\ V.\ Landshoff and D.\ I.\ Olive 
	          and J.\ C.\ Polkinghorne",
     title     = "The Analytic $S$-matrix",
     publisher = "Cambridge University Press, Cambridge",
     year      = "1966",
     note      = "pp.\ 252--253"
}
@Book{Queen:1974dr,
     author    = "N.\ M.\ Queen and G.\ Violini",
     title     = "Dispersion theory in high-energy physics",
     publisher = "John Wiley \& Sons, Inc., New York",
     year      = "1974",
     note      = "pp.\ 13--14"
}
@Article{Adler:1964um,
     author    = "Adler, Stephen L.",
     title     = "{Consistency conditions on the strong interactions implied
                  by a partially conserved axial vector current}",
     journal   = "Phys. Rev.",
     volume    = "137",
     year      = "1965",
     pages     = "B1022-B1033",
     doi       = "10.1103/PhysRev.137.B1022",
     SLACcitation  = "%%CITATION = PHRVA,137,B1022;%%"
}
@misc{Adler:1964zero,
     note      = "{We note that the current parameterization neglects
                   the constraints of chiral symmetry near threshold and
                   in the unphysical region. Therefore the Adler 
		   zero\cite{Adler:1964um} is, too, neglected.}"
}
@Article{Elsner:2007hm,
     author    = "Elsner, D. and others",
 collaboration = "CBELSA",
     title     = "{Measurement of the beam asymmetry in eta photoproduction
                  off the proton}",
     journal   = "Eur. Phys. J.",
     volume    = "A33",
     year      = "2007",
     pages     = "147-155",
     archivePrefix = "arXiv",
     doi       = "10.1140/epja/i2007-10447-9",
     SLACcitation  = "%%CITATION = NUCL-EX/0702032;%%"
}
@misc{Tablenote,
     note      = "{The $\chi^2$ per datum analysis presented in Table 
	           \eqref{tab:chi2} includes results for groups that
		   have provided amplitudes in a manner allowing
		   the reconstruction of observables at arbitary angle and
		   energy.}"
}
@Book{Hatfield:1992rz,
     author    = "Hatfield, B.",
     title     = "{Quantum field theory of point particles and strings}",
     publisher = "{Addison-Wesley, Redwood City, USA (Frontiers
                  in physics, 75)}",
     year      = "1992",
     note      = "See \S 19.2 \textit{Particles and Strings} p.\ 487."
}
@Book{Barut:1967ao,
     author    = "A.\ O.\ Barut",
     title     = "The theory of the scattering matrix",
     publisher = "The Macmillan Company, New York",
     year      = "1967",
     note      = "pp.\ 211--222"
}
@Article{Veltman:1963th,
     author    = "Veltman, M. J. G.",
     title     = "{Unitarity and causality in a renormalizable field theory
                  with unstable particles}",
     journal   = "Physica",
     volume    = "29",
     year      = "1963",
     pages     = "186-207",
     SLACcitation  = "%%CITATION = PHYSA,29,186;%%"
}
@Book{Musk:2008si,
     author    = "{N. I. Muskhelishvili}",
     title     = "Singular integral equations: boundary value problems
	          of function theory and their application to mathematical
		  physics",
     publisher = "Dover Publications",
     year      = "2008"
}
@Article{Blankenbecler:1961zz,
     author    = "Blankenbecler, R.",
     title     = "{Construction of Unitary Scattering Amplitudes}",
     journal   = "Phys. Rev.",
     volume    = "122",
     year      = "1961",
     pages     = "983-992",
     doi       = "10.1103/PhysRev.122.983",
     SLACcitation  = "%%CITATION = PHRVA,122,983;%%"
}
@Article{Blankenbecler:1965gx,
     author    = "Blankenbecler, R. and Sugar, R.",
     title     = "{Linear integral equations for relativistic multichannel
                  scattering}",
     journal   = "Phys. Rev.",
     volume    = "142",
     year      = "1966",
     pages     = "1051-1059",
     doi       = "10.1103/PhysRev.142.1051",
     SLACcitation  = "%%CITATION = PHRVA,142,1051;%%"
}
@Article{Cooper:1988ap,
     author    = "Cooper, E. D. and Jennings, B. K.",
     title     = "{OBTAINING THE ONE-BODY LIMIT FROM THE RELATIVISTIC TWO-
                  BODY EQUATION}",
     journal   = "Nucl. Phys.",
     volume    = "A500",
     year      = "1989",
     pages     = "553",
     doi       = "10.1016/0375-9474(89)90225-X",
     SLACcitation  = "%%CITATION = NUPHA,A500,553;%%"
}
@Article{Paris:2010tz,
     author    = "Paris, Mark W. and Workman, Ron L.",
     title     = "{Toward a unified description of hadro- and
                  photoproduction: S-wave pi- and eta-photoproduction
                  amplitudes}",
     journal   = "Phys. Rev.",
     volume    = "C82",
     year      = "2010",
     pages     = "035202",
     archivePrefix = "arXiv",
     primaryClass  =  "nucl-th",
     doi       = "10.1103/PhysRevC.82.035202",
     SLACcitation  = "%%CITATION = 1004.0455;%%"
}
@Article{Dugger:2009pn,
     author    = "Dugger, M. and others",
 collaboration = "CLAS",
     title     = "{$\pi^+$ photoproduction on the proton for photon energies
                  from 0.725 to 2.875 GeV}",
     journal   = "Phys. Rev.",
     volume    = "C79",
     year      = "2009",
     pages     = "065206",
     archivePrefix = "arXiv",
     primaryClass  =  "hep-ex",
     doi       = "10.1103/PhysRevC.79.065206",
     SLACcitation  = "%%CITATION = 0903.1110;%%"
}
@article{Paris:2008ig,
      author         = "Paris, Mark W.",
      title          = "{Dynamical coupled channel calculation of pion and omega
                        meson production}",
      journal        = "Phys.Rev.",
      volume         = "C79",
      pages          = "025208",
      doi            = "10.1103/PhysRevC.79.025208",
      year           = "2009"
}
@article{Suzuki:2009nj,
      author         = "Suzuki, N. and Julia-Diaz, B. and Kamano, H. and Lee,
                        T.-S.H. and Matsuyama, A. and others",
      title          = "{Disentangling the Dynamical Origin of P-11 Nucleon
                        Resonances}",
      journal        = "Phys.Rev.Lett.",
      volume         = "104",
      pages          = "042302",
      doi            = "10.1103/PhysRevLett.104.042302",
      year           = "2010"
}
@article{Gegelia:2009py,
      author         = "Gegelia, J. and Scherer, S.",
      title          = "{How to define physical properties of unstable
                        particles}",
      journal        = "Eur.Phys.J.",
      volume         = "A44",
      pages          = "425-430",
      doi            = "10.1140/epja/i2010-10955-5",
      year           = "2010"
}
@misc{Svarc:2008pc,
   author = "A.\ Svarc",
   year = {2008}, 
   howpublished = "private communication",
}
@misc{Workman:2010ip,
   author = "Ron L.\ Workman and Mark W.\ Paris",
   year = {2010}, 
   howpublished = "in preparation",
}
@misc{Paris:2010is,
   author = "Ron L.\ Workman and Mark W.\ Paris",
   year = {2010}, 
   howpublished = "Submitted to \textit{Phys.\ Rev.\ C}",
}
@article{Paris:2003at,
      author         = "Paris, M.W.",
      title          = "{Electromagnetic response of confined Dirac particles}",
      journal        = "Phys.Rev.",
      volume         = "C68",
      pages          = "025201",
      doi            = "10.1103/PhysRevC.68.025201",
      year           = "2003"
}
@article{Doring:2009bi,
      author         = "Doring, M. and Hanhart, C. and Huang, F. and Krewald, S.
                        and Meissner, U.-G.",
      title          = "{The Role of the background in the extraction of
                        resonance contributions from meson-baryon scattering}",
      journal        = "Phys.Lett.",
      volume         = "B681",
      pages          = "26-31",
      doi            = "10.1016/j.physletb.2009.09.052",
      year           = "2009"
}
@article{Page:2000ij,
      author         = "Page, Philip R. and Goldman, J.Terrance and Ginocchio,
                        Joseph N.",
      title          = "{Relativistic symmetry suppresses quark spin orbit
                        splitting}",
      journal        = "Phys.Rev.Lett.",
      volume         = "86",
      pages          = "204-207",
      doi            = "10.1103/PhysRevLett.86.204",
      year           = "2001"
}
@article{Ginocchio:1996zp,
      author         = "Ginocchio, Joseph N.",
      title          = "{Pseudospin as a relativistic symmetry}",
      journal        = "Phys.Rev.Lett.",
      volume         = "78",
      pages          = "436-439",
      doi            = "10.1103/PhysRevLett.78.436",
      year           = "1997"
}
@Article{March:1953vt,
  title = {The Viral Theorem for Dirac's Equation},
  author = {March, N. H.},
  journal = {Phys. Rev.},
  volume = {92},
  number = {2},
  pages = {481--482},
  numpages = {1},
  year = {1953},
  month = {Oct},
  doi = {10.1103/PhysRev.92.481},
  publisher = {American Physical Society}
}
@INPROCEEDINGS{Shabaev:2003vd,
   author = {{Shabaev}, V.~M.},
    title = "{Virial Relations for the Dirac Equation and Their Applications to Calculations of Hydrogen-Like Atoms}",
booktitle = {Precision Physics of Simple Atomic Systems},
     year = 2003,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 627,
   editor = "{S.~G.~Karshenboim \& V.~B.~Smirnov}",
    pages = {97-113},
      doi = {10.1007/b13865},
   adsurl = {http://adsabs.harvard.edu/abs/2003LNP...627...97S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Epstein:1962hv,
   author = {{Epstein}, J.~H. and {Epstein}, S.~T.},
    title = "{Some Applications of Hypervirial Theorems to the Calculation of Average Values}",
  journal = {American Journal of Physics},
     year = 1962,
    month = apr,
   volume = 30,
    pages = {266-268},
      doi = {10.1119/1.1941987},
   adsurl = {http://adsabs.harvard.edu/abs/1962AmJPh..30..266E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Gasparyan:2003fp,
      author         = "Gasparyan, A.M. and Haidenbauer, J. and Hanhart, C. and
                        Speth, J.",
      title          = "{Pion nucleon scattering in a meson exchange model}",
      journal        = "Phys.Rev.",
      volume         = "C68",
      pages          = "045207",
      doi            = "10.1103/PhysRevC.68.045207",
      year           = "2003"
}
@Article{Schutz:1994cp,
  title = {Role of correlated two-pion exchange in \pi{}N scattering},
  author = {Sch\"utz, C.  and Durso, J. W. and Holinde, K.  and Speth, J. },
  journal = {Phys. Rev. C},
  volume = {49},
  number = {5},
  pages = {2671--2687},
  numpages = {16},
  year = {1994},
  month = {May},
  doi = {10.1103/PhysRevC.49.2671},
  publisher = {American Physical Society}
}
@book{Weinberg:1972gc,
  author = {Steven Weinberg},
  publisher = {John Wiley \& Sons},
  title = {{Gravitation and Cosmology}},
  type = {Book},
  year = 1972
}
@book{CnHv1,
    address = {New York, NY},
    author = {Courant, R. and Hilbert, D.},
    citeulike-article-id = {4487965},
    keywords = {file-import-09-05-07},
    posted-at = {2009-05-07 19:39:56},
    priority = {2},
    publisher = {Interscience Publishers},
    title = {{Methods of Mathematical Physics}},
    volume = {1},
    year = {1953},
    note = {{First English edition, page 112}}
}
@ARTICLE{Low:1955PhRv,
   author = {{Low}, F.~E.},
    title = "{Boson-Fermion Scattering in the Heisenberg Representation}",
  journal = {Phys. Rev.},
     year = 1955,
    month = mar,
   volume = 97,
    pages = {1392-1398},
      doi = {10.1103/PhysRev.97.1392},
   adsurl = {http://adsabs.harvard.edu/abs/1955PhRv...97.1392L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Dyson:1949bp,
      author         = "Dyson, F.J.",
      title          = "{The Radiation theories of Tomonaga, Schwinger, and
                        Feynman}",
      journal        = "Phys.Rev.",
      volume         = "75",
      pages          = "486-502",
      doi            = "10.1103/PhysRev.75.486",
      year           = "1949",
}
@article{Dyson:1949ha,
      author         = "Dyson, F.J.",
      title          = "{The S matrix in quantum electrodynamics}",
      journal        = "Phys.Rev.",
      volume         = "75",
      pages          = "1736-1755",
      doi            = "10.1103/PhysRev.75.1736",
      year           = "1949",
}
@book{Sakurai:1967aqm,
  author = {J.\ J.\ Sakurai},
  publisher = {Addison Wesley},
  title = {{Advanced Quantum Mechanics}},
  type = {Book},
  year = 1967
}
@article{Ceci:2011ae,
      author         = "Ceci, S. and Doring, M. and Hanhart, C. and Krewald, S.
                        and Meissner, U.-G. and others",
      title          = "{Relevance of complex branch points for partial wave
                        analysis}",
      year           = "2011",
      eprint         = "1104.3490",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}
@article{Roper:1964zz,
      author         = "Roper, L.David",
      title          = "{Evidence for a P-11 Pion-Nucleon Resonance at 556 MeV}",
      journal        = "Phys.Rev.Lett.",
      volume         = "12",
      pages          = "340-342",
      doi            = "10.1103/PhysRevLett.12.340",
      year           = "1964",
}
@article{Lehmann:1957zz,
      author         = "Lehmann, H. and Symanzik, K. and Zimmermann, W.",
      title          = "{On the formulation of quantized field theories. II}",
      journal        = "Nuovo Cim.",
      volume         = "6",
      pages          = "319-333",
      doi            = "10.1007/BF02832508",
      year           = "1957",
}
@article{Feynman:1951gn,
      author         = "Feynman, Richard P.",
      title          = "{An Operator calculus having applications in quantum
                        electrodynamics}",
      journal        = "Phys.Rev.",
      volume         = "84",
      pages          = "108-128",
      doi            = "10.1103/PhysRev.84.108",
      year           = "1951",
}
@article{GellMann:1951rw,
      author         = "Gell-Mann, Murray and Low, Francis",
      title          = "{Bound states in quantum field theory}",
      journal        = "Phys.Rev.",
      volume         = "84",
      pages          = "350-354",
      doi            = "10.1103/PhysRev.84.350",
      year           = "1951",
}
@article{Schwinger:1951ex,
      author         = "Schwinger, Julian S.",
      title          = "{On the Green's functions of quantized fields.\ 1.}",
      journal        = "Proc.Nat.Acad.Sci.",
      volume         = "37",
      pages          = "452-455",
      year           = "1951",
}
@article{Schwinger:1951hq,
      author         = "Schwinger, Julian S.",
      title          = "{On the Green's functions of quantized fields.\ 2.}",
      journal        = "Proc.Nat.Acad.Sci.",
      volume         = "37",
      pages          = "455-459",
      year           = "1951"
}
@article{Haag:1957rs,
   author = {Haag, R.},
   affiliation = {Max-Planck-Institut für Physik Göttingen},
   title = {On the physical significance of the redundant solutions                         of the low equation},
   journal = {Nuovo Cimento (1955-1965)},
   publisher = {Italian Physical Society},
   keyword = {Journals},
   pages = {203-215},
   volume = {5},
   issue = {1},
   year = {1957}
}
@Unpublished{Paris:2011ip,
     author    = "Paris, Mark W.",
     title     = "Functional methods in canonical quantum field theory",
     year      = "2011",
     note      = "in preparation"
}
@article{Schweber:1955yf,
   author = {Schweber, S.},
   affiliation = {Brandeis University Waltham Massachusetts},
   title = {On the Yang-Feldman formalism},
   journal = {Nuovo Cimento (1955-1965)},
   publisher = {Italian Physical Society},
   keyword = {Journals},
   pages = {397-412},
   volume = {2},
   issue = {3},
   year = {1955}
}
@article{Rzewuski:1970ef,
   author = "Rzewuski, J.",
   title  = "On entire functionals in quantum field theory",
   journal = "Rep.\ Math.\ Phys.",
   volume = "1",
   pages = "1-27",
   year = "1970"
}
@article{Garbaczewski:1974gf,
   author = "Garbaczewski, Piotr and Rzewuski, Jan",
   title  = "On generating functionals for antisymmetric functions and
             their application in quantum field theory",
   journal = "Rep.\ Math.\ Phys.",
   volume = "6",
   pages = "431-444",
   year = "1974"
}
@article{Efimov:1975sm,
   author = "{G.V.\ Efimov}",
   title  = "On the proof that the S matrix is unitary",
   journal = "Teoret. Mat. Fiz.",
   volume = "25",
   pages = "20-29",
   year = "1975"
}
@book{Akhiezer:1965qe,
  title={Quantum electrodynamics},
  author={Akhiezer, A.I. and Berestetski{\u\i}, V.B.},
  year={1965},
  publisher={Interscience Publishers},
  note = "{C}{h. III, \S 24.4}"
}
@misc{Rgnote,
   note = "{a}nd references therein"
}
@article{Arndt:2002xv,
      author         = "Arndt, R.A. and Briscoe, W.J. and Strakovsky, I.I. and
                        Workman, R.L.",
      title          = "{Analysis of pion photoproduction data}",
      journal        = "Phys.Rev.",
      volume         = "C66",
      pages          = "055213",
      year           = "2002"
}
@article{Workman:2011vb,
      author         = "Workman, Ron L. and Briscoe, William J. and Paris, Mark
                        W. and Strakovsky, Igor I.",
      title          = "{Updated SAID analysis of pion photoproduction data}",
      year           = "2011",
      eprint         = "1109.0722",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
}
@article{Pennington:2011bq,
      author         = "Pennington, M.R.",
      title          = "{Exciting Baryons: now and in the future}",
      year           = "2011",
      eprint         = "1109.3690",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
}
@article{Barker:1975bp,
      author         = "Barker, I.S. and Donnachie, A. and Storrow, J.K.",
      title          = "{Complete Experiments in Pseudoscalar Photoproduction}",
      journal        = "Nucl.Phys.",
      volume         = "B95",
      pages          = "347",
      doi            = "10.1016/0550-3213(75)90049-8",
      year           = "1975",
}
@article{Ivanovich1968441,
   title = "Elastic scattering of several hydrogen and helium isotopes from tritium",
   journal = "Nuclear Physics A",
   volume = "110",
   number = "2",
   pages = "441 - 462",
   year = "1968",
   note = "",
   issn = "0375-9474",
   doi = "10.1016/0375-9474(68)90552-6",
   url = "http://www.sciencedirect.com/science/article/pii/0375947468905526",
   author = "M. Ivanovich and P.G. Young and G.G. Ohlsen",
   keywords = "Nuclear Reactions"
}
@article{LaneThomas:1958rmp,
  volume = {30},
  journal = {Rev. Mod. Phys.},
  author = {Lane, A. M. and Thomas, R. G.},
  month = {Apr},
  doi = {10.1103/RevModPhys.30.257},
  year = {1958},
  title = {R-Matrix Theory of Nuclear Reactions},
  issue = {2},
  publisher = {American Physical Society},
  pages = {257--353}
}
@article{LaneRobson:1966pr,
  volume = {151},
  journal = {Phys. Rev.},
  author = {Lane, A. M. and Robson, D.},
  month = {Nov},
  url = {http://link.aps.org/doi/10.1103/PhysRev.151.774},
  doi = {10.1103/PhysRev.151.774},
  year = {1966},
  title = {Comprehensive Formalism for Nuclear Reaction Problems. I. Derivation of Existing Reaction Theories},
  issue = {3},
  publisher = {American Physical Society},
  pages = {774--787}
}
@unpublished{HaleDodder:1979fus,
   title="R-matrix analysis of light-element reactions for fusion applications",
   author="G.\ M.\ Hale and D.\ C.\ Dodder",
   note="{{\em R-matrix analysis of light-element reactions for fusion applications}}",
   year="1979"
}
@article{Descouvemont:2010cx,
      author         = "Descouvemont, P. and Baye, D.",
      title          = "{The R-matrix theory}",
      journal        = "Rept.\ Prog.\ Phys.",
      volume         = "73",
      pages          = "036301",
      doi            = "10.1088/0034-4885/73/3/036301",
      year           = "2010",
      eprint         = "1001.0678",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = ARXIV:1001.0678;%%",
}
@article{PhysRev.100.25,
  volume = {100},
  journal = {Phys. Rev.},
  author = {Thomas, R. G.},
  month = {Oct},
  url = {http://link.aps.org/doi/10.1103/PhysRev.100.25},
  doi = {10.1103/PhysRev.100.25},
  year = {1955},
  title = {Collision Matrix for ($n,~d$) and ($p,~d$) Reactions},
  issue = {1},
  publisher = {American Physical Society},
  pages = {25--32}
}
@article{PhysRev.160.719,
  volume = {160},
  journal = {Phys. Rev.},
  author = {Buttle, P. J. A.},
  month = {Aug},
  url = {http://link.aps.org/doi/10.1103/PhysRev.160.719},
  doi = {10.1103/PhysRev.160.719},
  year = {1967},
  title = {Solution of Coupled Equations by $R$-Matrix Techniques},
  issue = {4},
  publisher = {American Physical Society},
  pages = {719--729}
}
@article{PhysRevA.31.2698,
  volume = {31},
  journal = {Phys. Rev. A},
  author = {Winter, Thomas G. and Lane, Neal F.},
  month = {Apr},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.31.2698},
  doi = {10.1103/PhysRevA.31.2698},
  year = {1985},
  title = {"$R$-matrix" approach to electron transfer in $$\alpha${}$-H collisions},
  issue = {4},
  publisher = {American Physical Society},
  pages = {2698--2701}
}
@article{PhysRev.97.224,
  volume = {97},
  journal = {Phys. Rev.},
  author = {Thomas, R. G.},
  month = {Jan},
  url = {http://link.aps.org/doi/10.1103/PhysRev.97.224},
  doi = {10.1103/PhysRev.97.224},
  year = {1955},
  title = {Collision Matrices for the Compound Nucleus},
  issue = {1},
  publisher = {American Physical Society},
  pages = {224--237}
}
@article{RevModPhys.34.723,
  volume = {34},
  journal = {Rev. Mod. Phys.},
  author = {Vogt, Erich},
  month = {Oct},
  url = {http://link.aps.org/doi/10.1103/RevModPhys.34.723},
  doi = {10.1103/RevModPhys.34.723},
  year = {1962},
  title = {Theory of Low Energy Nuclear Reactions},
  issue = {4},
  publisher = {American Physical Society},
  pages = {723--747}
}
@article{PhysRev.178.1715,
  volume = {178},
  journal = {Phys. Rev.},
  author = {LANE, A. M. and ROBSON, D.},
  month = {Feb},
  url = {http://link.aps.org/doi/10.1103/PhysRev.178.1715},
  doi = {10.1103/PhysRev.178.1715},
  year = {1969},
  title = {Optimization of Nuclear Resonance Reaction Calculations},
  issue = {4},
  publisher = {American Physical Society},
  pages = {1715--1724}
}
@misc{GMH-Watt:2012pc,
   author = "G.\ M.\ Hale",
   year = {2012}, 
   howpublished = "private communication",
}
@article{Watt:PR87.1037.52,
  title = {Energy Spectrum of Neutrons from Thermal Fission of ${\mathrm{U}}^{235}$},
  author = {Watt, B. E.},
  journal = {Phys. Rev.},
  volume = {87},
  issue = {6},
  pages = {1037--1041},
  year = {1952},
  month = {Sep},
  doi = {10.1103/PhysRev.87.1037},
  url = {http://link.aps.org/doi/10.1103/PhysRev.87.1037},
  publisher = {American Physical Society}
}
@book{Atzeni:2004if,
  author =	 "Stefano Atzeni and {J\"{u}rgen Meyer-ter-Vehn}",
  title =	 "The Physics of Inertial Fusion",
  publisher =	 "Oxford University Press",
  series =       "International Series of Monographs on Physics",
  volume =	 125,
  edition =	 "1st",
  year =	 2004
}
@book{Rolfs:1988cc,
  author =	 "C. Rolfs and W.\ W.\ Rodney",
  title =	 "Cauldrons in the Cosmos",
  publisher =	 "University of Chicago Press",
  edition =	 "1st",
  year =	 1988
}
@article{Workman:2012cm,
  title = {Unified Chew-Mandelstam SAID analysis of pion photoproduction data},
  author = {Workman, Ron L. and Paris, Mark W. and Briscoe, William J. and Strakovsky, Igor I.},
  journal = {Phys. Rev. C},
  volume = {86},
  issue = {1},
  pages = {015202},
  numpages = {10},
  year = {2012},
  month = {Jul},
  doi = {10.1103/PhysRevC.86.015202},
  publisher = {American Physical Society}
}
@article{Workman:2012up,
  title = {Updated SAID analysis of pion photoproduction data},
  author = {Workman, Ron L. and Briscoe, William J. and Paris, Mark W. and Strakovsky, Igor I.},
  journal = {Phys. Rev. C},
  volume = {85},
  issue = {2},
  pages = {025201},
  numpages = {8},
  year = {2012},
  month = {Feb},
  doi = {10.1103/PhysRevC.85.025201},
  publisher = {American Physical Society}
}
@article{Wolf:1956tf,
   author = {Wolfenstein, L},
   title = {Polarization of Fast Nucleons},
   journal = {Annual Review of Nuclear Science},
   volume = {6},
   number = {1},
   pages = {43-76},
   year = {1956},
   doi = {10.1146/annurev.ns.06.120156.000355},
}
@article{Schwinger:1972ert,
  title = {Minutes of the Meeting at Stanford University, California July 11-12, 1947},
  journal = {Phys. Rev.},
  volume = {72},
  issue = {8},
  pages = {738--748},
  year = {1947},
  month = {Oct},
  doi = {10.1103/PhysRev.72.738},
  url = {http://link.aps.org/doi/10.1103/PhysRev.72.738},
  publisher = {American Physical Society}
}
@article{BlattJacksonERT,
  title = {On the Interpretation of Neutron-Proton Scattering Data by the Schwinger Variational Method},
  author = {Blatt, John M. and Jackson, J. David},
  journal = {Phys. Rev.},
  volume = {76},
  issue = {1},
  pages = {18--37},
  year = {1949},
  month = {Jul},
  doi = {10.1103/PhysRev.76.18},
  url = {http://link.aps.org/doi/10.1103/PhysRev.76.18},
  publisher = {American Physical Society}
}
@ARTICLE{Barker:1972bc,
   author = {{Barker}, F.~C.},
    title = "{The boundary condition parameter in R-matrix theory}",
  journal = {Australian Journal of Physics},
     year = 1972,
    month = aug,
   volume = 25,
    pages = {341},
   adsurl = {http://adsabs.harvard.edu/abs/1972AuJPh..25..341B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Cyburt:2009cf,
      author         = "Cyburt, Richard H. and Pospelov, Maxim",
      title          = "{Resonant enhancement of nuclear reactions as a possible
                        solution to the cosmological lithium problem}",
      journal        = "Int.J.Mod.Phys.",
      volume         = "E21",
      pages          = "1250004",
      doi            = "10.1142/S0218301312500048",
      year           = "2012",
      eprint         = "0906.4373",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:0906.4373;%%",
}
@article{Cyburt:2009cfpo,
      author         = "Cyburt and Pospelov",
      journal        = "Int.J.Mod.Phys.",
      volume         = "E21",
      pages          = "1250004",
      year           = "2012",
}
@article{Chakraborty:2010zj,
      author         = "Chakraborty, Nachiketa and Fields, Brian D. and Olive,
                        Keith A.",
      title          = "{Resonant Destruction as a Possible Solution to the
                        Cosmological Lithium Problem}",
      journal        = "Phys.Rev.",
      volume         = "D83",
      pages          = "063006",
      doi            = "10.1103/PhysRevD.83.063006",
      year           = "2011",
      eprint         = "1011.0722",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      reportNumber   = "UMN-TH-2924-10, FTPI-MINN-10-31",
      SLACcitation   = "%%CITATION = ARXIV:1011.0722;%%",
}
@article{Chakraborty:2010zjpo,
      author         = "Chakraborty and Fields and Olive",
      journal        = "Phys.Rev.",
      volume         = "D83",
      pages          = "063006",
      year           = "2011",
}
@article{Wigner:1946zz,
      author         = "Wigner, Eugene P.",
      title          = "{Resonance Reactions and Anomalous Scattering}",
      journal        = "Phys.Rev.",
      volume         = "70",
      pages          = "15-33",
      doi            = "10.1103/PhysRev.70.15",
      year           = "1946",
      SLACcitation   = "%%CITATION = PHRVA,70,15;%%",
}
@article{Wigner:1946zzpo,
      author         = "Wigner",
      journal        = "Phys.Rev.",
      volume         = "70",
      pages          = "15",
      year           = "1946",
}
@article{Hale:2008nd,
title = "Covariances from Light-Element R-Matrix Analyses ",
journal = "Nuclear Data Sheets ",
volume = "109",
number = "12",
pages = "2812 - 2816",
year = "2008",
note = "<ce:title>Special Issue on Workshop on Neutron Cross Section Covariances June 24-28, 2008, Port Jefferson, New York, USA</ce:title> ",
issn = "0090-3752",
doi = "10.1016/j.nds.2008.11.015",
url = "http://www.sciencedirect.com/science/article/pii/S0090375208001038",
author = "G.M. Hale"
}
@article{Hale:2008ndpo,
author = "Hale",
journal = "Nucl.\ Data Sh.",
volume = "109",
pages = "2812",
year = "2008"
}
@article{Hale:1987zz,
      author         = "Hale, G.M. and Brown, Ronald E. and Jarmie, Nelson",
      title          = "{Pole structure of the Jpi=3/2+ resonance in He-5}",
      journal        = "Phys.Rev.Lett.",
      volume         = "59",
      pages          = "763-766",
      doi            = "10.1103/PhysRevLett.59.763",
      year           = "1987",
      SLACcitation   = "%%CITATION = PRLTA,59,763;%%",
}
@article{Hale:1987zzpo,
      author         = "Hale and Brown and Jarmie",
      journal        = "Phys.Rev.Lett.",
      volume         = "59",
      pages          = "763",
      year           = "1987",
}
@article{O'Malley:2011zza,
      author         = "O'Malley, P.D. and Bardayan, D.W. and Adekola, A.S. and
                        Ahn, S. and Chae, K.Y. and others",
      title          = "{Search for a resonant enhancement of the Be-7 + d
                        reaction and primordial Li-7 abundances}",
      journal        = "Phys.Rev.",
      volume         = "C84",
      pages          = "042801",
      doi            = "10.1103/PhysRevC.84.042801",
      year           = "2011",
      SLACcitation   = "%%CITATION = PHRVA,C84,042801;%%",
}
@article{O'Malley:2011zzapo,
      author         = "O'Malley and others",
      journal        = "Phys.\ Rev.",
      volume         = "C84",
      pages          = "042801",
      year           = "2011",
}
@book{BLOT:1990,
      author         = "N.N.\ Bogolubov and A.A.\ Logunov and A.I.\ Oksak
         and I.T.\ Todorov",
      title          = "General Principles of Quantum Field Theory",
      publisher      = "Kluwer Academic Publishers",
      year           = "1988",
      note           = "{C}{h. 14}"
}
@article{Bogoljubov:1958dr,
      author         = "N.N.\ Bogoljubov and B.V.\ Medvedev and M.K.\
                        Polivanov",
      journal        = "Fortschritte der Physik",
      volume         = "6",
      pages          = "169--245",
      year           = "1958"
}
@article{Tilley:2004A9,
      author         = "Tilley, D. R. and {\em et.\ al.}",
      journal        = "Nucl.\ Phys.\ A",
      volume         = "745",
      pages          = "155",
      year           = "2004"
}
@book{Varshalovich:1988qq,
      author         = "D.A.\ Varshalovich and A.N.\ Moskalev and
      V.K.\ Khersonskii",
      title          = "Quantum Theory of Angular Momentum",
      year           = "1988",
      publisher      = "World Scientific",
      note           = "p.\ 144, Eq.(11)"
}
@book{Burke:2011bo,
  author =	 "Philip George Burke",
  title =	 "R-Matrix Theory of Atomic Collisions: Application
     to Atomic, Molecular and Optical Processes",
  publisher =	 "Springer Berlin Heidelberg",
  series =       "Springer Series on Atomic, Optical and Plasma Physics",
  volume =	 61,
  year =	 2011
}
@article{Hale:2014rm,
      author         = "Gerald M.\ Hale and Lowell S.\ Brown and Mark W.\ Paris",
      journal        = "Phys.\ Rev.\ C",
      volume         = "89",
      pages          = "014623",
      year           = "2014"
}
@article{Brown:2014ef,
  title = {Field theory of the <span class="aps-inline-formula"><math><mrow><mi>d</mi><mo>+</mo><mi>t</mi><mo>→</mo><mi>n</mi><mo>+</mo><mi>α</mi></mrow></math></span> reaction dominated by a <span class="aps-inline-formula"><math><msup><mrow></mrow><mn>5</mn></msup></math></span>He<span class="aps-inline-formula"><math><msup><mrow></mrow><mo>*</mo></msup></math></span> unstable particle},
  author = {Brown, Lowell S. and Hale, Gerald M.},
  journal = {Phys. Rev. C},
  volume = {89},
  issue = {1},
  pages = {014622},
  numpages = {15},
  year = {2014},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevC.89.014622}
}
@article{Thomas:1958ta,
      author         = "R.\ G.\ Thomas",
      journal        = "Phys.\ Rev.",
      volume         = "89",
      pages          = "014623",
      year           = "2014"
}
@article{Thomas:1950ta,
  title = {On the Determination of Reduced Widths from the One-Level Dispersion Formula},
  author = {Thomas, R. G.},
  journal = {Phys. Rev.},
  volume = {81},
  issue = {1},
  pages = {148--149},
  numpages = {0},
  year = {1951},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.81.148}
}
@article{Barker:1999wt,
      author         = "F.\ C.\ Barker",
      journal        = "Phys.\ Rev. C",
      volume         = "59",
      pages          = "535",
      year           = "1999"
}
@article{Brune:2002ap,
      author         = "C.\ R.\ Brune",
      journal        = "Phys.\ Rev.\ C",
      volume         = "66",
      pages          = "044611",
      year           = "2002"
}
@article{Azuma:2010az,
      author         = "R.\ E.\ Azuma and E.\ Uberseder and E.\ C.\ Simpson and C.\ R.\ Brune and H.\ Constantini and R.\ J.\ de Boer and J.\ G{\"o}rres and M.\ Heil and P.\ J.\ LeBlanc and C.\ Ugalde and M. Wiescher",
      journal        = "Phys.\ Rev. C",
      volume         = "81",
      pages          = "045805",
      year           = "2010"
}
@unpublished{Larson:2008sa,
   title="Updated User's Guide for SAMMY: Multilevel R-matrix Fits to Neutron Data Using Bayes' Equations",
   author="N.\ M.\ Larson",
   note="{{\em Updated User's Guide for SAMMY: Multilevel R-matrix Fits to Neutron Data Using Bayes' Equations}}",
   eprint="ORNL/TM-9179/R8",
   year="2008"
}
@article{Bloch:1957fu,
      author         = "Claude Bloch",
      journal        = "Nucl.\ Phys.",
      volume         = "4",
      pages          = "503",
      year           = "1957"
}
@book{Thompson:2009nr,
  title={Nuclear Reactions for Astrophysics: Principles, Calculation and Applications of Low-Energy Reactions},
  author={Thompson, I.J. and Nunes, F.M.},
  year={2009},
  publisher={Cambridge University Press}
}
@article{Prosser:1958sf,
  title = {Some Properties of the Shift and Penetration Factors in Nuclear Reactions},
  author = {Prosser, F. W. and Biedenharn, L. C.},
  journal = {Phys. Rev.},
  volume = {109},
  issue = {2},
  pages = {413--417},
  year = {1958},
  month = {Jan},
  publisher = {American Physical Society},
}
@ARTICLE{Pettini:2012yd,
   author = {{Pettini}, M. and {Cooke}, R.},
    title = "{A new, precise measurement of the primordial abundance of deuterium}",
  journal = {\mnras},
 keywords = {quasars: absorption lines, quasars: individual: J1419+0829, cosmology: observations},
     year = 2012,
    month = oct,
   volume = 425,
    pages = {2477-2486},
      doi = {10.1111/j.1365-2966.2012.21665.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425.2477P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Cooke:2014do,
        Author = {Ryan J. Cooke and Max Pettini and Regina A. Jorgenson and Michael T. Murphy and Charles C. Steidel},
        Journal = {The Astrophysical Journal},
        Number = {1},
        Pages = {31},
        Title = {Precision Measures of the Primordial Abundance of Deuterium},
        Volume = {781},
        Year = {2014}
}
@ARTICLE{Olive:2004xx,
   author = {{Olive}, K.~A. and {Skillman}, E.~D.},
    title = "{A Realistic Determination of the Error on the Primordial Helium Abundance: Steps toward Nonparametric Nebular Helium Abundances}",
  journal = {The Astrophysical Journal},
   eprint = {astro-ph/0405588},
 keywords = {Cosmology: Early Universe, Galaxies: Abundances, ISM: H II Regions, ISM: Abundances},
     year = 2004,
    month = dec,
   volume = 617,
    pages = {29-49},
      doi = {10.1086/425170},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...617...29O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Asplund:2006Ap,
   author = {{Asplund}, M. and {Lambert}, D.~L. and {Nissen}, P.~E. and {Primas}, F. and 
        {Smith}, V.~V.},
    title = "{Lithium Isotopic Abundances in Metal-poor Halo Stars}",
  journal = {The Astrophysical Journal},
   eprint = {astro-ph/0510636},
 keywords = {Cosmology: Early Universe, Galaxy: Evolution, Stars: Abundances, Stars: Atmospheres, Stars: Population II},
     year = 2006,
    month = jun,
   volume = 644,
    pages = {229-259},
      doi = {10.1086/503538},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...644..229A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Fields:2011zzb,
      author         = "Fields, Brian D.",
      title          = "{The primordial lithium problem}",
      journal        = "Ann.Rev.Nucl.Part.Sci.",
      volume         = "61",
      pages          = "47-68",
      doi            = "10.1146/annurev-nucl-102010-130445",
      year           = "2011",
      eprint         = "1203.3551",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
      SLACcitation   = "%%CITATION = ARXIV:1203.3551;%%",
}
@article{Sarkar:2012zz,
      author         = "S.\ Sarkar and B.\ Fields",
      title          = "{Review of Particle Physics}",
      collaboration  = "Particle Data Group",
      journal        = "Phys.Rev.",
      volume         = "D86",
      pages          = "010001",
      doi            = "10.1103/PhysRevD.86.010001",
      year           = "2012",
      SLACcitation   = "%%CITATION = PHRVA,D86,010001;%%",
}
@article{Alpher:1948ve,
      author         = "Alpher, R.A. and Bethe, H. and Gamow, G.",
      title          = "{The origin of chemical elements}",
      journal        = "Phys.Rev.",
      volume         = "73",
      pages          = "803-804",
      doi            = "10.1103/PhysRev.73.803",
      year           = "1948",
      SLACcitation   = "%%CITATION = PHRVA,73,803;%%",
}
@unpublished{Fermi:1950up,
      author         = "E.\ Fermi and A.\ Turkevich",
      year="1950"
}
@ARTICLE{Peebles:1966prl,
   author = {{Peebles}, P.~J.},
    title = "{Primeval Helium Abundance and the Primeval Fireball}",
  journal = {Physical Review Letters},
     year = 1966,
    month = mar,
   volume = 16,
    pages = {410-413},
      doi = {10.1103/PhysRevLett.16.410},
   adsurl = {http://adsabs.harvard.edu/abs/1966PhRvL..16..410P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{WFH:1967,
      author         = "Wagoner, Robert V. and Fowler, William A. and Hoyle,
                        Fred",
      title          = "{On the Synthesis of elements at very high temperatures}",
      journal        = "Astrophys.J.",
      volume         = "148",
      pages          = "3-49",
      doi            = "10.1086/149126",
      year           = "1967",
      SLACcitation   = "%%CITATION = ASJOA,148,3;%%",
}
@ARTICLE{Wagoner:1969sy,
   author = {{Wagoner}, R.~V.},
    title = "{Synthesis of the Elements Within Objects Exploding from Very High Temperatures}",
  journal = {\apjs},
     year = 1969,
    month = jun,
   volume = 18,
    pages = {247},
      doi = {10.1086/190191},
   adsurl = {http://adsabs.harvard.edu/abs/1969ApJS...18..247W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Pospelov:2010hj,
      author         = "Pospelov, Maxim and Pradler, Josef",
      title          = "{Big Bang Nucleosynthesis as a Probe of New Physics}",
      journal        = "Ann.Rev.Nucl.Part.Sci.",
      volume         = "60",
      pages          = "539-568",
      doi            = "10.1146/annurev.nucl.012809.104521",
      year           = "2010",
      eprint         = "1011.1054",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      SLACcitation   = "%%CITATION = ARXIV:1011.1054;%%",
}
@article{Serpico:2004gx,
      author         = "Serpico, P. and Esposito, S. and Iocco, F.
                        and Mangano, G. and Miele, G. and others",
      title          = "{Nuclear reaction network for primordial nucleosynthesis:
                        A Detailed analysis of rates, uncertainties and light
                        nuclei yields}",
      journal        = "JCAP",
      volume         = "0412",
      pages          = "010",
      doi            = "10.1088/1475-7516/2004/12/010",
      year           = "2004",
      eprint         = "astro-ph/0408076",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph",
      reportNumber   = "MPP-2004-82, DSP-19-2004",
      SLACcitation   = "%%CITATION = ASTRO-PH/0408076;%%",
}
@article{Descouvement:2004xx,
      author         = "P.\ Descouvement and others",
      journal        = "Nucl.\ Data Tabl.",
      volume         = "88",
      pages          = "203--236",
      year           = "2004"
}
@article{Paris:2014nd,
      author         = "M.\ Paris and G.\ Hale and A.\ Hayes and G.\ Jungman",
      journal        = "Nucl.\ Data Sheets",
      note           = "{\em to appear}",
      year           = "2014"
}
@article{Bosch:1992bh,
   author = {{Bosch}, H.-S. and {Hale}, G.~M.},
    title = "{Improved formulas for fusion cross-sections and thermal reactivities}",
  journal = {Nuclear Fusion},
     year = 1992,
    month = apr,
   volume = 32,
    pages = {611-631},
      doi = {10.1088/0029-5515/32/4/I07},
   adsurl = {http://adsabs.harvard.edu/abs/1992NucFu..32..611B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@unpublished{STEEPM,
   author       = "G.\ Hale and T.\ Talley",
   title        = "Maxwellian-Averaged Data for Thermonuclear Reactions",
   year         = "2009"
}
@unpublished{SPECT,
   author       = "G.\ Hale",
   title        = "{SPECT code}",
   year         = "2000"
}
@article{Nollett:2007su,
      author         = "Nollett, Kenneth M. and Pieper, Steven C. and Wiringa,
                        Robert B. and Carlson, J. and Hale, G.M.",
      title          = "{Quantum Monte Carlo calculations of neutron-alpha
                        scattering}",
      journal        = "Phys.Rev.Lett.",
      volume         = "99",
      pages          = "022502",
      doi            = "10.1103/PhysRevLett.99.022502",
      year           = "2007",
      eprint         = "nucl-th/0612035",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      SLACcitation   = "%%CITATION = NUCL-TH/0612035;%%",
}
@article{Alford:2004pf,
      author         = "Alford, Mark and Braby, Matt and Paris, M.W. and Reddy,
                        Sanjay",
      title          = "{Hybrid stars that masquerade as neutron stars}",
      journal        = "Astrophys.J.",
      volume         = "629",
      pages          = "969-978",
      doi            = "10.1086/430902",
      year           = "2005",
      eprint         = "nucl-th/0411016",
      archivePrefix  = "arXiv",
      primaryClass   = "nucl-th",
      reportNumber   = "JLAB-05-04-294",
      SLACcitation   = "%%CITATION = NUCL-TH/0411016;%%",
}
@article{OMalley:2011xx,
  title = "{Search for a resonant enhancement of the $^7$Be + d reaction and primordial $^7$Li abundances}",
  author = {O'Malley and others},
  journal = {Phys. Rev. C},
  volume = {84},
  issue = {4},
  pages = {042801},
  numpages = {3},
  year = {2011},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevC.84.042801},
  url = {http://link.aps.org/doi/10.1103/PhysRevC.84.042801}
}
@article{Davies:1996pv,
   title = "The mathematics of principal value integrals and
      applications to nuclear physics, transport theory, and condensed
      matter physics",
   author = "K.T.R.\ Davies and M.L.\ Glasser and V.\ Protopopescu and
      Frank Tabakin",
   journal = "Math.\ Mods.\ Meths.\ in Appl.\ Sci.",
   volume = "6",
   pages = "833-885",
   year = "1996"
}
@book{Dodelson:2003mc,
  title={Modern Cosmology},
  author={Dodelson, S.},
  isbn={9780122191411},
  lccn={2002117793},
  series={Academic Press},
  url={http://books.google.com/books?id=3oPRxdXJexcC},
  year={2003},
  publisher={Academic Press}
}
@article{AM66,
   title="Nucleon-nucleon phase shift analyses by chi-square
      minimization",
   author="Richard A.\ Arndt and Malcolm H.\ MacGregor",
   journal="Methods in Computational Physics",
   volume="6",
   year="1966",
   pages="253"
}
@Book{Martin:SfP,
     author    = "B.R.\ Martin",
     title     = "Statistics for Physicists",
     publisher = "Academic Press",
     year      = "1971"
}
@BOOK{Tolman:1938ps,
   author = {{Tolman}, R.~C.},
    title = "{The Principles of Statistical Mechanics}",
     year = 1938,
   adsurl = {http://adsabs.harvard.edu/abs/1938psm..book.....T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Avni:1976cl,
   author = {{Avni}, Y.},
    title = "{Energy spectra of X-ray clusters of galaxies}",
  journal = {\apj},
 keywords = {Energy Spectra, Galactic Clusters, Statistical Analysis, X Ray Sources, X Ray Spectra, Computerized Simulation, Monte Carlo Method, Range (Extremes), Spectral Energy Distribution, Spectrum Analysis},
     year = 1976,
    month = dec,
   volume = 210,
    pages = {642-646},
      doi = {10.1086/154870},
   adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...210..642A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@book{Bondi:1950co,
        Author = {Bondi, H.},
        Isbn = {9780521141185},
        Publisher = {Cambridge University Press},
        Series = {Cambridge Monographs on Physics},
        Title = {Cosmology},
        Url = {http://books.google.com/books?id=xGsFQHK9shAC},
        Year = {2011},
        Bdsk-Url-1 = {http://books.google.com/books?id=xGsFQHK9shAC}
}
@misc{wiki:2010reco,
        author = "{\tt Wikipedia}",
        title = "Recombination (cosmology)",
        howpublished = "\url{http://en.wikipedia.org/wiki/Recombination_(cosmology)\#cite_note-1}",
        year = {2010}, 
        note = "[Online; accessed 01 July 2014]"
}
@article{Detweiler:2005sf,
        Author = {Steven Detweiler},
        Journal = {Classical and Quantum Gravity},
        Number = {15},
        Pages = {S681},
        Title = {Perspective on gravitational self-force analyses},
        Url = {http://stacks.iop.org/0264-9381/22/i=15/a=006},
        Volume = {22},
        Year = {2005},
        Bdsk-Url-1 = {http://stacks.iop.org/0264-9381/22/i=15/a=006}
}
@misc{BICEP2:cosmohist,
   author = "Yinweichen",
   year = {2014}, 
   howpublished =
      "\url{http://commons.wikimedia.org/wiki/File:History_of_the_Universe.svg}"
}
@ARTICLE{Baumann:2009cl,
   author = {{Baumann}, D.},
    title = "{TASI Lectures on Inflation}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {0907.5424},
 primaryClass = "hep-th",
 keywords = {High Energy Physics - Theory, Astrophysics - Cosmology and Extragalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology},
     year = 2009,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2009arXiv0907.5424B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{PlanckXVI:2014,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and et al.},
    title = "{Planck 2013 results. XVI. Cosmological parameters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1303.5076},
 keywords = {cosmic background radiation, cosmological parameters, early Universe, inflation, primordial nucleosynthesis},
     year = 2014,
    month = nov,
   volume = 571,
      eid = {A16},
    pages = {A16},
      doi = {10.1051/0004-6361/201321591},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...571A..16P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@book{Huang:1987sm,
  title={Statistical mechanics},
  author={Huang, K.},
  isbn={9780471815181},
  lccn={86032466},
  url={http://books.google.com/books?id=M8PvAAAAMAAJ},
  year={1987},
  publisher={Wiley}
}
@book{Brown:1994qf,
        Author = {Brown, L.S.},
        Publisher = {Cambridge University Press},
        Title = {Quantum Field Theory},
        Url = {http://books.google.com/books?id=\_qt\_nQEACAAJ},
        Year = {1994},
        Bdsk-Url-1 = {http://books.google.com/books?id=%5C_qt%5C_nQEACAAJ}
}
@book{Peskin:1995in,
        Author = {Peskin, M.E. and Schroeder, D.V.},
        Publisher = {Addison-Wesley Publishing Company},
        Series = {Advanced book classics},
        Title = {An Introduction to Quantum Field Theory},
        Year = {1995}
}
@book{LL:1981pk,
  title={Physical Kinetics},
  author={Lifshitz, E.M. and Pitaevski{\u\i}, L.P.},
  number={v. 10},
  isbn={9780750626354},
  lccn={80042162},
  series={Course of theoretical physics},
  url={http://books.google.com/books?id=h7LgAAAAMAAJ},
  year={1981},
  publisher={Butterworth-Heinemann}
}
@book{LL:1982cm,
  title={Mechanics},
  author={Landau, L.D. and Lifshitz, E.M.},
  number={v. 1},
  isbn={9780080503479},
  url={http://books.google.com/books?id=bE-9tUH2J2wC},
  year={1982},
  publisher={Elsevier Science}
}

@article{BICEP2:2014,
        Author = {Ade, {P.A.R.} and others},
        Journal = {Phys. Rev. Lett.},
        Month = {Jun},
        Pages = {241101},
        Title = {Detection of B-Mode Polarization at Degree Angular Scales by BICEP2},
        Volume = {112},
        Year = {2014}
}
@ARTICLE{Hamann:2008bc,
   author = {{Hamann}, J. and {Lesgourgues}, J. and {Mangano}, G.},
    title = "{Using big bang nucleosynthesis in cosmological parameter extraction from the cosmic microwave background: a forecast for PLANCK}",
  journal = {\jcap},
     year = 2008,
    month = mar,
   volume = 3,
      eid = {004},
    pages = {4},
      doi = {10.1088/1475-7516/2008/03/004},
   adsurl = {http://adsabs.harvard.edu/abs/2008JCAP...03..004H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Nollett:2011ho,
   author = {{Nollett}, K.~M. and {Holder}, G.~P.},
    title = "{An analysis of constraints on relativistic species from primordial nucleosynthesis and the cosmic microwave background}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1112.2683},
 primaryClass = "astro-ph.CO",
 keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics, Nuclear Theory},
     year = 2011,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2011arXiv1112.2683N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Hou:2013da,
   author = {{Hou}, Z. and {Keisler}, R. and {Knox}, L. and {Millea}, M. and 
	{Reichardt}, C.},
    title = "{How massless neutrinos affect the cosmic microwave background damping tail}",
  journal = {\prd},
 keywords = {Background radiations, Non-standard-model neutrinos right-handed neutrinos etc.},
     year = 2013,
    month = apr,
   volume = 87,
   number = 8,
      eid = {083008},
    pages = {083008},
      doi = {10.1103/PhysRevD.87.083008},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvD..87h3008H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{SMK:1993bb,
   author = {{Smith}, M.~S. and {Kawano}, L.~H. and {Malaney}, R.~A.},
    title = "{Experimental, computational, and observational analysis of primordial nucleosynthesis}",
  journal = {\apjs},
 keywords = {Abundance, Light Elements, Monte Carlo Method, Nuclear Fusion, Nuclear Reactions, Baryons, Chemical Reactions, Lithium, Neutrons, Numerical Analysis, Protons, Star Distribution},
     year = 1993,
    month = apr,
   volume = 85,
    pages = {219-247},
      doi = {10.1086/191763},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJS...85..219S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Fuller:2010nn,
   author = {{Boyd}, R.~N. and {Brune}, C.~R. and {Fuller}, G.~M. and {Smith}, C.~J.
	},
    title = "{New nuclear physics for big bang nucleosynthesis}",
  journal = {\prd},
 keywords = {Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Big Bang nucleosynthesis, Fundamental aspects of astrophysics},
     year = 2010,
    month = nov,
   volume = 82,
   number = 10,
      eid = {105005},
    pages = {105005},
      doi = {10.1103/PhysRevD.82.105005},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvD..82j5005B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Weinberg:1971eg,
   author = {{Weinberg}, S.},
    title = "{Entropy Generation and the Survival of Protogalaxies in an Expanding Universe}",
  journal = {\apj},
     year = 1971,
    month = sep,
   volume = 168,
    pages = {175},
      doi = {10.1086/151073},
   adsurl = {http://adsabs.harvard.edu/abs/1971ApJ...168..175W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Shimon:2010cb,
   author = {{Shimon}, M. and {Miller}, N.~J. and {Kishimoto}, C.~T. and 
        {Smith}, C.~J. and {Fuller}, G.~M. and {Keating}, B.~G.},
    title = "{Using Big Bang Nucleosynthesis to extend CMB probes of neutrino physics}",
  journal = {\jcap},
     year = 2010,
    month = may,
   volume = 5,
      eid = {037},
    pages = {37},
      doi = {10.1088/1475-7516/2010/05/037},
   adsurl = {http://adsabs.harvard.edu/abs/2010JCAP...05..037S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{PlanckI:2013ov,
   author = {{Planck Collaboration}},
    title = "{Planck 2013 results. I. Overview of products and scientific results}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1303.5062},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2013,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1303.5062P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ACT:2013cp,
   author = {{ACT Collaboration}},
    title = "{The Atacama Cosmology Telescope: cosmological parameters from three seasons of data}",
  journal = {\jcap},
     year = 2013,
    month = oct,
   volume = 10,
      eid = {060},
    pages = {60},
      doi = {10.1088/1475-7516/2013/10/060},
   adsurl = {http://adsabs.harvard.edu/abs/2013JCAP...10..060S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BICEP2:2014bm,
   author = {{BICEP2 Collaboration} and {Ade}, P.~A.~R and others},
    title = "{BICEP2 II: Experiment and Three-Year Data Set}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1403.4302},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2014,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1403.4302B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SPT:2011hl,
   author = {{SPT Collaboration}},
    title = "{A Measurement of the Damping Tail of the Cosmic Microwave Background Power Spectrum with the South Pole Telescope}",
  journal = {\apj},
 keywords = {cosmic background radiation, cosmological parameters, cosmology: observations},
     year = 2011,
    month = dec,
   volume = 743,
      eid = {28},
    pages = {28},
      doi = {10.1088/0004-637X/743/1/28},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...743...28K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{WMAP:2013ny,
   author = {{WMAP Collaboration}},
    title = "{Nine-year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Parameter Results}",
  journal = {\apjs},
 keywords = {cosmic background radiation, cosmology: observations, dark matter, early universe, instrumentation: detectors, space vehicles, space vehicles: instruments, telescopes },
     year = 2013,
    month = oct,
   volume = 208,
      eid = {19},
    pages = {19},
      doi = {10.1088/0067-0049/208/2/19},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..208...19H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Aver:2013ue,
   author = {{Aver}, E. and {Olive}, K.~A. and {Porter}, R.~L. and {Skillman}, E.~D.
        },
    title = "{The primordial helium abundance from updated emissivities}",
  journal = {\jcap},
     year = 2013,
    month = nov,
   volume = 11,
      eid = {017},
    pages = {17},
      doi = {10.1088/1475-7516/2013/11/017},
   adsurl = {http://adsabs.harvard.edu/abs/2013JCAP...11..017A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Izotov:2010ns,
   author = {{Izotov}, Y.~I. and {Thuan}, T.~X.},
    title = "{The Primordial Abundance of $^{4}$He: Evidence for Non-Standard Big Bang Nucleosynthesis}",
  journal = {\apjl},
 keywords = {galaxies: abundances, galaxies: irregular, galaxies: ISM, ISM: abundances},
     year = 2010,
    month = feb,
   volume = 710,
    pages = {L67-L71},
      doi = {10.1088/2041-8205/710/1/L67},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710L..67I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{AOS:2009yp,
   author = {{Aver}, E. and {Olive}, K.~A. and {Skillman}, E.~D.},
    title = "{A new approach to systematic uncertainties and self-consistency in helium abundance determinations}",
  journal = {\jcap},
     year = 2010,
    month = may,
   volume = 5,
      eid = {003},
    pages = {3},
      doi = {10.1088/1475-7516/2010/05/003},
   adsurl = {http://adsabs.harvard.edu/abs/2010JCAP...05..003A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Izotov:2014yp,
   author = {{Izotov}, Y.~I. and {Thuan}, T.~X. and {Guseva}, N.~G.},
    title = "{A new determination of the primordial He abundance using the He I {$\lambda$}10830 {\AA} emission line: cosmological implications}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1408.6953},
 keywords = {galaxies: abundances, galaxies: irregular, galaxies: ISM, cosmological parameters},
     year = 2014,
    month = nov,
   volume = 445,
    pages = {778-793},
      doi = {10.1093/mnras/stu1771},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.445..778I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GFP-PRL:2014mn,
     author    = "Evan Grohs and George M.\ Fuller and Chad T.\ Kishimoto and Mark W.\ Paris",
    title = "{Effects of $N_\textrm{eff}$ and neutrino rest mass on ionization equilibrium freeze-out}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1412.6875},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2014,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1412.6875G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GFP-PRL:2014mnelse,
   author = {{Grohs}, E. and {Fuller}, G.~M. and {Kishimoto}, C.~T. and {Paris}, M.~W.
	},
    title = "{Effects of neutrino rest mass on \$N\_$\backslash$text$\{$eff$\}$\$ and ionization equilibrium freeze-out}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1412.6875},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2014,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1412.6875G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dolgov:1997ne,
   author = {{Dolgov}, A.~D. and {Hansen}, S.~H. and {Semikoz}, D.~V.},
    title = "{Non-equilibrium corrections to the spectra of massless neutrinos in the early universe}",
  journal = {Nuclear Physics B},
   eprint = {hep-ph/9703315},
     year = 1997,
    month = feb,
   volume = 503,
    pages = {426-444},
      doi = {10.1016/S0550-3213(97)00479-3},
   adsurl = {http://adsabs.harvard.edu/abs/1997NuPhB.503..426D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Gnedin:1998ne,
   author = {{Gnedin}, N.~Y. and {Gnedin}, O.~Y.},
    title = "{Cosmological Neutrino Background Revisited}",
  journal = {\apj},
   eprint = {astro-ph/9712199},
 keywords = {COSMOLOGY: EARLY UNIVERSE, ELEMENTARY PARTICLES, COSMOLOGY: COSMIC MICROWAVE BACKGROUND, NUCLEAR REACTIONS, NUCLEOSYNTHESIS, ABUNDANCES, Cosmology: Early Universe, Elementary Particles, Cosmology: Cosmic Microwave Background, Nuclear Reactions, Nucleosynthesis, Abundances},
     year = 1998,
    month = dec,
   volume = 509,
    pages = {11-15},
      doi = {10.1086/306469},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...509...11G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{FKK:2011di,
   author = {{Fuller}, G.~M. and {Kishimoto}, C.~T. and {Kusenko}, A.},
    title = "{Heavy sterile neutrinos, entropy and relativistic energy production, and the relic neutrino background}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1110.6479},
 primaryClass = "astro-ph.CO",
 keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics, High Energy Physics - Phenomenology},
     year = 2011,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2011arXiv1110.6479F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{AliHamoud:2011hr,
   author = {{Ali-Ha{\"i}moud}, Y. and {Hirata}, C.~M.},
    title = "{HyRec: A fast and highly accurate primordial hydrogen and helium recombination code}",
  journal = {\prd},
 keywords = {Cosmology, Radiative transfer, scattering, Multiphoton ionization and excitation to highly excited states, Background radiations},
     year = 2011,
    month = feb,
   volume = 83,
   number = 4,
      eid = {043513},
    pages = {043513},
      doi = {10.1103/PhysRevD.83.043513},
   adsurl = {http://adsabs.harvard.edu/abs/2011PhRvD..83d3513A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Chluba:2011cr,
   author = {{Chluba}, J. and {Thomas}, R.~M.},
    title = "{Towards a complete treatment of the cosmological recombination problem}",
  journal = {\mnras},
 keywords = {cosmic background radiation, cosmological parameters, cosmology: observations, cosmology: theory},
     year = 2011,
    month = apr,
   volume = 412,
    pages = {748-764},
      doi = {10.1111/j.1365-2966.2010.17940.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.412..748C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{SSS:2000rc,
   author = {{Seager}, S. and {Sasselov}, D.~D. and {Scott}, D.},
    title = "{How Exactly Did the Universe Become Neutral?}",
  journal = {\apjs},
 keywords = {Atomic Processes, Cosmology: Cosmic Microwave Background, Cosmology: Theory, Cosmology: Early Universe},
     year = 2000,
    month = jun,
   volume = 128,
    pages = {407-430},
      doi = {10.1086/313388},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJS..128..407S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{SSS:1999nc,
   author = {{Seager}, S. and {Sasselov}, D.~D. and {Scott}, D.},
    title = "{A New Calculation of the Recombination Epoch}",
  journal = {\apjl},
 keywords = {ATOMIC PROCESSES, COSMOLOGY: COSMIC MICROWAVE BACKGROUND, COSMOLOGY: THEORY, COSMOLOGY: EARLY UNIVERSE, Atomic Processes, Cosmology: Cosmic Microwave Background, Cosmology: Theory, Cosmology: Early Universe},
     year = 1999,
    month = sep,
   volume = 523,
    pages = {L1-L5},
      doi = {10.1086/312250},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...523L...1S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Silk:1968dd,
   author = {{Silk}, J.},
    title = "{Cosmic Black-Body Radiation and Galaxy Formation}",
  journal = {\apj},
     year = 1968,
    month = feb,
   volume = 151,
    pages = {459},
      doi = {10.1086/149449},
   adsurl = {http://adsabs.harvard.edu/abs/1968ApJ...151..459S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Zaldarriaga:1995dd,
   author = {{Zaldarriaga}, M. and {Harari}, D.~D.},
    title = "{Analytic approach to the polarization of the cosmic microwave background in flat and open universes}",
  journal = {\prd},
 keywords = {Background radiations, Observational cosmology},
     year = 1995,
    month = sep,
   volume = 52,
    pages = {3276-3287},
      doi = {10.1103/PhysRevD.52.3276},
   adsurl = {http://adsabs.harvard.edu/abs/1995PhRvD..52.3276Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Hu:1997dd,
   author = {{Hu}, W. and {White}, M.},
    title = "{CMB anisotropies: Total angular momentum method}",
  journal = {\prd},
 keywords = {Background radiations, Observational cosmology},
     year = 1997,
    month = jul,
   volume = 56,
    pages = {596-615},
      doi = {10.1103/PhysRevD.56.596},
   adsurl = {http://adsabs.harvard.edu/abs/1997PhRvD..56..596H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Trotta:2004bc,
   author = {{Trotta}, R. and {Hansen}, S.~H.},
    title = "{Constraining the helium abundance with CMB data}",
  journal = {\prd},
 keywords = {Cosmology, Gravity in more than four dimensions Kaluza-Klein theory unified field theories, alternative theories of gravity, Dark matter, Background radiations},
     year = 2004,
    month = jan,
   volume = 69,
   number = 2,
      eid = {023509},
    pages = {023509},
      doi = {10.1103/PhysRevD.69.023509},
   adsurl = {http://adsabs.harvard.edu/abs/2004PhRvD..69b3509T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Ichikawa:2006bc,
  title = {Primordial helium abundance from CMB: A constraint from recent observations and a forecast},
  author = {Ichikawa, Kazuhide and Sekiguchi, Toyokazu and Takahashi, Tomo},
  journal = {Phys. Rev. D},
  volume = {78},
  issue = {4},
  pages = {043509},
  numpages = {10},
  year = {2008},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.78.043509},
  url = {http://link.aps.org/doi/10.1103/PhysRevD.78.043509}
}

@ARTICLE{1968ApJ...153....1P,
   author = {{Peebles}, P.~J.~E.},
    title = "{Recombination of the Primeval Plasma}",
  journal = {\apj},
     year = 1968,
    month = jul,
   volume = 153,
    pages = {1},
      doi = {10.1086/149628},
   adsurl = {http://adsabs.harvard.edu/abs/1968ApJ...153....1P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1968ZhETF..55..278Z,
   author = {{Zeldovich}, Y.~B. and {Kurt}, V.~G. and {Syunyaev}, R.~A.},
    title = "{Recombination of Hydrogen in the Hot Model of the Universe}",
  journal = {Zhurnal Eksperimentalnoi i Teoreticheskoi Fiziki},
 keywords = {Cosmology, Cosmic Microwave Background Radiation, Intergalactic Gas},
     year = 1968,
    month = jul,
   volume = 55,
    pages = {278-286},
   adsurl = {http://adsabs.harvard.edu/abs/1968ZhETF..55..278Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991A&A...251..680P,
   author = {{Pequignot}, D. and {Petitjean}, P. and {Boisson}, C.},
    title = "{Total and effective radiative recombination coefficients}",
  journal = {\aap},
 keywords = {Hydrogen, Interstellar Gas, Ionized Gases, Radiative Recombination, Recombination Coefficient, Ultraviolet Spectra, Carbon, Cold Plasmas, Forbidden Bands, Nitrogen, Oxygen, Planetary Nebulae},
     year = 1991,
    month = nov,
   volume = 251,
    pages = {680-688},
   adsurl = {http://adsabs.harvard.edu/abs/1991A%26A...251..680P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998MNRAS.297.1073H,
   author = {{Hummer}, D.~G. and {Storey}, P.~J.},
    title = "{Recombination of helium-like ions - I. Photoionization cross-sections and total recombination and cooling coefficients for atomic helium}",
  journal = {\mnras},
 keywords = {ATOMIC DATA, ATOMIC PROCESSES, LINE: FORMATION},
     year = 1998,
    month = jul,
   volume = 297,
    pages = {1073-1078},
      doi = {10.1046/j.1365-8711.1998.2970041073.x},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.297.1073H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2000ApJ...530L..57R,
   author = {{Ryan}, S.~G. and {Beers}, T.~C. and {Olive}, K.~A. and {Fields}, B.~D. and 
	{Norris}, J.~E.},
    title = "{Primordial Lithium and Big Bang Nucleosynthesis}",
  journal = {\apjl},
   eprint = {astro-ph/9905211},
 keywords = {COSMOLOGY: THEORY, GALAXY: HALO, NUCLEAR REACTIONS, NUCLEOSYNTHESIS, ABUNDANCES, STARS: POPULATION II},
     year = 2000,
    month = feb,
   volume = 530,
    pages = {L57-L60},
      doi = {10.1086/312492},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...530L..57R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Lewis:2002mc,
   author = {{Lewis}, A. and {Bridle}, S.},
    title = "{Cosmological parameters from CMB and other data: A Monte Carlo approach}",
  journal = {\prd},
   eprint = {astro-ph/0205436},
 keywords = {Observational cosmology, Applications of Monte Carlo methods, Neutrino mass and mixing},
     year = 2002,
    month = nov,
   volume = 66,
   number = 10,
      eid = {103511},
    pages = {103511},
      doi = {10.1103/PhysRevD.66.103511},
   adsurl = {http://adsabs.harvard.edu/abs/2002PhRvD..66j3511L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Unpublished{GFG:2015,
     author    = "Lauren A.\ Gilbert and George M.\ Fuller and Evan Grohs",
     note      = "in preparation",
     year      = "2015",
}

@Unpublished{AFG:2015,
     author    = "Jeremy N.\ Ariche and George M.\ Fuller and Evan Grohs",
     note      = "in preparation",
     year      = "2015",
}
@ARTICLE{KF:2008PRD,
   author = {{Kishimoto}, C.~T. and {Fuller}, G.~M.},
    title = "{Lepton-number-driven sterile neutrino production in the early universe}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0802.3377},
 keywords = {Dark matter, Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc.},
     year = 2008,
    month = jul,
   volume = 78,
   number = 2,
      eid = {023524},
    pages = {023524},
      doi = {10.1103/PhysRevD.78.023524},
   adsurl = {http://adsabs.harvard.edu/abs/2008PhRvD..78b3524K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{KF:2008PRL,
   author = {{Fuller}, G.~M. and {Kishimoto}, C.~T.},
    title = "{Quantum Coherence of Relic Neutrinos}",
  journal = {Physical Review Letters},
archivePrefix = "arXiv",
   eprint = {0811.4370},
 keywords = {Neutrino mass and mixing, Decoherence, open systems, quantum statistical methods, Particle-theory and field-theory models of the early Universe},
     year = 2009,
    month = may,
   volume = 102,
   number = 20,
      eid = {201303},
    pages = {201303},
      doi = {10.1103/PhysRevLett.102.201303},
   adsurl = {http://adsabs.harvard.edu/abs/2009PhRvL.102t1303F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2014SPIE.9153E..1PB,
   author = {{SPT Collaboration}},
    title = "{SPT-3G: a next-generation cosmic microwave background polarization experiment on the South Pole telescope}",
booktitle = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
     year = 2014,
   series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
   volume = 9153,
archivePrefix = "arXiv",
   eprint = {1407.2973},
 primaryClass = "astro-ph.IM",
    month = jul,
      eid = {91531P},
    pages = {1},
      doi = {10.1117/12.2057305},
   adsurl = {http://adsabs.harvard.edu/abs/2014SPIE.9153E..1PB},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...794..171T,
   author = {{The Polarbear Collaboration}},
    title = "{A Measurement of the Cosmic Microwave Background B-mode Polarization Power Spectrum at Sub-degree Scales with POLARBEAR}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1403.2369},
 keywords = {cosmic background radiation, cosmology: observations, large-scale structure of universe },
     year = 2014,
    month = oct,
   volume = 794,
      eid = {171},
    pages = {171},
      doi = {10.1088/0004-637X/794/2/171},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...794..171T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004NJPh....6..117K,
   author = {{Kneller}, J.~P. and {Steigman}, G.},
    title = "{BBN for pedestrians}",
  journal = {New Journal of Physics},
   eprint = {astro-ph/0406320},
     year = 2004,
    month = sep,
   volume = 6,
    pages = {117},
      doi = {10.1088/1367-2630/6/1/117},
   adsurl = {http://adsabs.harvard.edu/abs/2004NJPh....6..117K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mangano:3.040,
   author = {{Mangano}, G. and {Miele}, G. and {Pastor}, S. and {Peloso}, M.
	},
    title = "{A precision calculation of the effective number of cosmological neutrinos}",
  journal = {Physics Letters B},
   eprint = {astro-ph/0111408},
     year = 2002,
    month = may,
   volume = 534,
    pages = {8-16},
      doi = {10.1016/S0370-2693(02)01622-2},
   adsurl = {http://adsabs.harvard.edu/abs/2002PhLB..534....8M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DarkRadScherrer:2012,
   author = {{Menestrina}, J.~L. and {Scherrer}, R.~J.},
    title = "{Dark radiation from particle decays during big bang nucleosynthesis}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1111.0605},
 primaryClass = "astro-ph.CO",
 keywords = {Particle-theory and field-theory models of the early Universe},
     year = 2012,
    month = feb,
   volume = 85,
   number = 4,
      eid = {047301},
    pages = {047301},
      doi = {10.1103/PhysRevD.85.047301},
   adsurl = {http://adsabs.harvard.edu/abs/2012PhRvD..85d7301M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{VFC:QKE,
   author = {{Vlasenko}, A. and {Fuller}, G.~M. and {Cirigliano}, V.},
    title = "{Neutrino quantum kinetics}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1309.2628},
 primaryClass = "hep-ph",
 keywords = {Neutrino mass and mixing, Supernovae, Nuclear physics aspects of novae supernovae and other explosive environments, Neutrino interactions},
     year = 2014,
    month = may,
   volume = 89,
   number = 10,
      eid = {105004},
    pages = {105004},
      doi = {10.1103/PhysRevD.89.105004},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..89j5004V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014arXiv1410.7684M,
   author = {{Mertens}, S. and {Dolde}, K. and {Korzeczek}, M. and {Glueck}, F. and 
	{Groh}, S. and {Martin}, R.~D. and {Poon}, A.~W.~P. and {Steidl}, M.
	},
    title = "{Wavelet Approach to Search for Sterile Neutrinos in Tritium \$$\backslash$beta\$-Decay Spectra}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1410.7684},
 primaryClass = "hep-ph",
 keywords = {High Energy Physics - Phenomenology, Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Experiment},
     year = 2014,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1410.7684M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ABFW_2005_PRD,
   author = {{Abazajian}, K. and {Bell}, N.~F. and {Fuller}, G.~M. and {Wong}, Y.~Y.~Y.
	},
    title = "{Cosmological lepton asymmetry, primordial nucleosynthesis and sterile neutrinos}",
  journal = {\prd},
  eprint = {astro-ph/0410175},
 keywords = {Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Big Bang nucleosynthesis, Fundamental aspects of astrophysics},
     year = 2005,
    month = sep,
   volume = 72,
   number = 6,
      eid = {063004},
    pages = {063004},
      doi = {10.1103/PhysRevD.72.063004},
   adsurl = {http://adsabs.harvard.edu/abs/2005PhRvD..72f3004A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006PhRvD..74h5008S,
   author = {{Smith}, C.~J. and {Fuller}, G.~M. and {Kishimoto}, C.~T. and 
	{Abazajian}, K.~N.},
    title = "{Light element signatures of sterile neutrinos and cosmological lepton numbers}",
  journal = {\prd},
   eprint = {astro-ph/0608377},
 keywords = {Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Big Bang nucleosynthesis, Fundamental aspects of astrophysics},
     year = 2006,
    month = oct,
   volume = 74,
   number = 8,
      eid = {085008},
    pages = {085008},
      doi = {10.1103/PhysRevD.74.085008},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhRvD..74h5008S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@techreport{TMT,
   author = "David Silva and Paul Hickson and Charles Steidel and
      Michael Bolte",
   title  = "{TMT Detailed Science Case: 2007}",
     year = "2007",
     note = "http://www.tmt.org"
}

@ARTICLE{LSND:1997,
   author = {{Athanassopoulos}, C. and others},
    title = "{The liquid scintillator neutrino detector and LAMPF neutrino source}",
  journal = {Nuclear Instruments and Methods in Physics Research A},
   eprint = {nucl-ex/9605002},
     year = 1997,
    month = feb,
   volume = 388,
    pages = {149-172},
      doi = {10.1016/S0168-9002(96)01155-2},
   adsurl = {http://adsabs.harvard.edu/abs/1997NIMPA.388..149A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MiniBooNE:2010,
   author = {{Aguilar-Arevalo}, A.~A. and others},
    title = "{Measurement of the neutrino neutral-current elastic differential cross section}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1007.4730},
 primaryClass = "hep-ex",
 keywords = {Neutrino interactions, Neutral currents, Elastic scattering, Protons and neutrons},
     year = 2010,
    month = nov,
   volume = 82,
   number = 9,
      eid = {092005},
    pages = {092005},
      doi = {10.1103/PhysRevD.82.092005},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvD..82i2005A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DoubleChooz:2012,
   author = {{Abe}, Y. and others},
    title = "{Reactor $\bar{\nu_e}$ disappearance in the 
              Double Chooz experiment}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1207.6632},
 primaryClass = "hep-ex",
 keywords = {Neutrino mass and mixing},
     year = 2012,
    month = sep,
   volume = 86,
   number = 5,
      eid = {052008},
    pages = {052008},
      doi = {10.1103/PhysRevD.86.052008},
   adsurl = {http://adsabs.harvard.edu/abs/2012PhRvD..86e2008A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@INPROCEEDINGS{GMT,
   author = {{McCarthy}, P. and {Bernstein}, R.~A.},
    title = "{Giant Magellan Telescope: Status and Opportunities for Scientific Synergy}",
booktitle = {Thirty Meter Telescope Science Forum},
     year = 2014,
    month = jul,
      eid = {61},
    pages = {61},
   adsurl = {http://adsabs.harvard.edu/abs/2014tmt..confE..61M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@BOOK{EELT,
   author = {{Hook (ed.)}, I.},
     year = 2005,
   title = "{The science case for the European Extremely Large Telescope : the next step in mankind's quest for the Universe.}",
 keywords = {Extremely Large Telescope (ELT), VERY LARGE TELESCOPES, TELESCOPE INSTRUMENTATION},
   publisher = {Cambridge, UK: OPTICON and Garching bei Muenchen, Germany: European Southern Observatory (ESO)},
   adsurl = {http://adsabs.harvard.edu/abs/2005scee.book.....H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002NuPhB.632..363D,
   author = {{Dolgov}, A.~D. and {Hansen}, S.~H. and {Pastor}, S. and {Petcov}, S.~T. and 
	{Raffelt}, G.~G. and {Semikoz}, D.~V.},
    title = "{Cosmological bounds on neutrino degeneracy improved by flavor oscillations}",
  journal = {Nucl. Phys. B},
   eprint = {hep-ph/0201287},
     year = 2002,
    month = jun,
   volume = 632,
    pages = {363-382},
      doi = {10.1016/S0550-3213(02)00274-2},
   adsurl = {http://adsabs.harvard.edu/abs/2002NuPhB.632..363D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008RPPh...71h6201O,
   author = {{Otten}, E.~W. and {Weinheimer}, C.},
    title = "{Neutrino mass limit from tritium {$\beta$} decay}",
  journal = {Reports on Progress in Physics},
archivePrefix = "arXiv",
   eprint = {0909.2104},
 primaryClass = "hep-ex",
     year = 2008,
    month = aug,
   volume = 71,
   number = 8,
      eid = {086201},
    pages = {086201},
      doi = {10.1088/0034-4885/71/8/086201},
   adsurl = {http://adsabs.harvard.edu/abs/2008RPPh...71h6201O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008JPhCS.136b2031D,
   author = {{Drexlin}, G.},
    title = "{Direct neutrino mass measurements}",
  journal = {Journal of Physics Conference Series},
     year = 2008,
    month = nov,
   volume = 136,
   number = 2,
      eid = {022031},
    pages = {022031},
      doi = {10.1088/1742-6596/136/2/022031},
   adsurl = {http://adsabs.harvard.edu/abs/2008JPhCS.136b2031D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005JHEP...11..028K,
   author = {{Kusenko}, A. and {Pascoli}, S. and {Semikoz}, D.},
    title = "{Bounds on heavy sterile neutrinos revisited}",
  journal = {Journal of High Energy Physics},
   eprint = {hep-ph/0405198},
     year = 2005,
    month = nov,
   volume = 11,
      eid = {028},
    pages = {28},
      doi = {10.1088/1126-6708/2005/11/028},
   adsurl = {http://adsabs.harvard.edu/abs/2005JHEP...11..028K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983PhLB..128..361B,
   author = {{Bergsma}, F. and others},
    title = "{A search for decays of heavy neutrinos}",
  journal = {Physics Letters B},
     year = 1983,
    month = sep,
   volume = 128,
    pages = {361-366},
      doi = {10.1016/0370-2693(83)90275-7},
   adsurl = {http://adsabs.harvard.edu/abs/1983PhLB..128..361B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986PhLB..166..479B,
   author = {{Bernardi}, G. and {Carugno}, G. and {Chauveau}, J. and {Dicarlo}, F. and 
	{Dris}, M. and {Dumarchez}, J. and {Ferro-Luzzi}, M. and {Levy}, J.-M. and 
	{Lukas}, D. and {Perreau}, J.-M. and {Pons}, Y. and {Touchard}, A.-M. and 
	{Vannucci}, F.},
    title = "{Search for neutrino decay}",
  journal = {Physics Letters B},
     year = 1986,
    month = jan,
   volume = 166,
    pages = {479-483},
      doi = {10.1016/0370-2693(86)91602-3},
   adsurl = {http://adsabs.harvard.edu/abs/1986PhLB..166..479B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1988PhLB..203..332B,
   author = {{Bernardi}, G. and {Carugno}, G. and {Chauveau}, J. and {Dicarlo}, F. and 
	{Dris}, M. and {Dumarchez}, J. and {Ferro-Luzzi}, M. and {Levy}, J.-M. and 
	{Lukas}, D. and {Perreau}, J.-M. and {Pons}, Y. and {Touchard}, A.-M. and 
	{Vannucci}, F.},
    title = "{Further limits on heavy neutrino couplings}",
  journal = {Physics Letters B},
     year = 1988,
    month = mar,
   volume = 203,
    pages = {332-334},
      doi = {10.1016/0370-2693(88)90563-1},
   adsurl = {http://adsabs.harvard.edu/abs/1988PhLB..203..332B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993PhLB..302..336B,
   author = {{Baranov}, S. and {Batusov}, Y. and {Bunyatov}, S. and {Klimov}, O. and 
	{Lyukov}, V. and {Nefedov}, Y. and {Popov}, B. and {Valuev}, V. and 
	{Borisov}, A. and {Goryachev}, V. and {Kirsanov}, M. and {Kozhin}, A. and 
	{Kravtsov}, V. and {Spiridonov}, A. and {Tumakov}, V. and {Vovenko}, A. and 
	{Kiss}, D.},
    title = "{Search for heavy neutrinos at the IHEP-JINR Neutrino Detector}",
  journal = {Physics Letters B},
     year = 1993,
    month = mar,
   volume = 302,
    pages = {336-340},
      doi = {10.1016/0370-2693(93)90405-7},
   adsurl = {http://adsabs.harvard.edu/abs/1993PhLB..302..336B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001NuPhS..98...37N,
   author = {{N{\'e}d{\'e}lec}, P.},
    title = "{Tau-sterile neutrino mixing in NOMAD}",
  journal = {Nuclear Physics B Proceedings Supplements},
     year = 2001,
    month = apr,
   volume = 98,
    pages = {37-42},
      doi = {10.1016/S0920-5632(01)01192-6},
   adsurl = {http://adsabs.harvard.edu/abs/2001NuPhS..98...37N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003PhRvL..91x1301K,
   author = {{Kaplinghat}, M. and {Knox}, L. and {Song}, Y.-S.},
    title = "{Determining Neutrino Mass from the Cosmic Microwave Background Alone}",
  journal = {Physical Review Letters},
   eprint = {astro-ph/0303344},
 keywords = {Background radiations, Neutrino mass and mixing, Gravitational lenses and luminous arcs},
     year = 2003,
    month = dec,
   volume = 91,
   number = 24,
      eid = {241301},
    pages = {241301},
      doi = {10.1103/PhysRevLett.91.241301},
   adsurl = {http://adsabs.harvard.edu/abs/2003PhRvL..91x1301K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004JCAP...04..008H,
   author = {{Hannestad}, S. and {Raffelt}, G.},
    title = "{Cosmological mass limits on neutrinos, axions, and other light particles}",
  journal = {\jcap},
   eprint = {hep-ph/0312154},
     year = 2004,
    month = apr,
   volume = 4,
      eid = {008},
    pages = {8},
      doi = {10.1088/1475-7516/2004/04/008},
   adsurl = {http://adsabs.harvard.edu/abs/2004JCAP...04..008H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009PhRvD..80l3509D,
   author = {{de Bernardis}, F. and {Kitching}, T.~D. and {Heavens}, A. and 
	{Melchiorri}, A.},
    title = "{Determining the neutrino mass hierarchy with cosmology}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0907.1917},
 primaryClass = "astro-ph.CO",
 keywords = {Observational cosmology, Neutrino mass and mixing},
     year = 2009,
    month = dec,
   volume = 80,
   number = 12,
      eid = {123509},
    pages = {123509},
      doi = {10.1103/PhysRevD.80.123509},
   adsurl = {http://adsabs.harvard.edu/abs/2009PhRvD..80l3509D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010JCAP...08..001H,
   author = {{Hannestad}, S. and {Mirizzi}, A. and {Raffelt}, G.~G. and {Wong}, Y.~Y.~Y.
	},
    title = "{Neutrino and axion hot dark matter bounds after WMAP-7}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1004.0695},
     year = 2010,
    month = aug,
   volume = 8,
      eid = {001},
    pages = {1},
      doi = {10.1088/1475-7516/2010/08/001},
   adsurl = {http://adsabs.harvard.edu/abs/2010JCAP...08..001H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010PhRvD..82h7302A,
   author = {{Archidiacono}, M. and {Cooray}, A. and {Melchiorri}, A. and 
	{Pandolfi}, S.},
    title = "{CMB neutrino mass bounds and reionization}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1010.5757},
 primaryClass = "astro-ph.CO",
 keywords = {Cosmology, Gravitational radiation magnetic fields and other observations, Background radiations, Particle-theory and field-theory models of the early Universe},
     year = 2010,
    month = oct,
   volume = 82,
   number = 8,
      eid = {087302},
    pages = {087302},
      doi = {10.1103/PhysRevD.82.087302},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvD..82h7302A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011PhRvD..83k5023G,
   author = {{Giusarma}, E. and {Corsi}, M. and {Archidiacono}, M. and {de Putter}, R. and 
	{Melchiorri}, A. and {Mena}, O. and {Pandolfi}, S.},
    title = "{Constraints on massive sterile neutrino species from current and future cosmological data}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1102.4774},
 primaryClass = "astro-ph.CO",
 keywords = {Cosmology, Gravitational radiation magnetic fields and other observations, Background radiations, Particle-theory and field-theory models of the early Universe},
     year = 2011,
    month = jun,
   volume = 83,
   number = 11,
      eid = {115023},
    pages = {115023},
      doi = {10.1103/PhysRevD.83.115023},
   adsurl = {http://adsabs.harvard.edu/abs/2011PhRvD..83k5023G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013PhRvD..87k3010V,
   author = {{Volpe}, C. and {V{\"a}{\"a}n{\"a}nen}, D. and {Espinoza}, C.
	},
    title = "{Extended evolution equations for neutrino propagation in astrophysical and cosmological environments}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1302.2374},
 primaryClass = "hep-ph",
 keywords = {Neutrino mass and mixing, Supernovae, Neutrino interactions, Many-body theory},
     year = 2013,
    month = jun,
   volume = 87,
   number = 11,
      eid = {113010},
    pages = {113010},
      doi = {10.1103/PhysRevD.87.113010},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvD..87k3010V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhRvD..90l5040S,
   author = {{Serreau}, J. and {Volpe}, C.},
    title = "{Neutrino-antineutrino correlations in dense anisotropic media}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1409.3591},
 primaryClass = "hep-ph",
 keywords = {Neutrino mass and mixing, Neutrino interactions, Supernovae},
     year = 2014,
    month = dec,
   volume = 90,
   number = 12,
      eid = {125040},
    pages = {125040},
      doi = {10.1103/PhysRevD.90.125040},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..90l5040S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010PhRvD..82l5017F,
   author = {{Fuller}, G.~M. and {Smith}, C.~J.},
    title = "{Nuclear weak interaction rates in primordial nucleosynthesis}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1009.0277},
 primaryClass = "astro-ph.CO",
 keywords = {Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Big Bang nucleosynthesis, Fundamental aspects of astrophysics},
     year = 2010,
    month = dec,
   volume = 82,
   number = 12,
      eid = {125017},
    pages = {125017},
      doi = {10.1103/PhysRevD.82.125017},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvD..82l5017F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991ApJ...368....1S,
   author = {{Savage}, M.~J. and {Malaney}, R.~A. and {Fuller}, G.~M.},
    title = "{Neutrino oscillations and the leptonic charge of the universe}",
  journal = {\apj},
 keywords = {Cosmology, Neutrinos, Nuclear Astrophysics, Universe, Adiabatic Conditions, Degenerate Matter, Leptons, Nuclear Fusion, Oscillations},
     year = 1991,
    month = feb,
   volume = 368,
    pages = {1-11},
      doi = {10.1086/169665},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...368....1S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002PhRvD..66a3008A,
   author = {{Abazajian}, K.~N. and {Beacom}, J.~F. and {Bell}, N.~F.},
    title = "{Stringent constraints on cosmological neutrino-antineutrino asymmetries from synchronized flavor transformation}",
  journal = {\prd},
   eprint = {astro-ph/0203442},
 keywords = {Neutrino mass and mixing, Big Bang nucleosynthesis},
     year = 2002,
    month = jul,
   volume = 66,
   number = 1,
      eid = {013008},
    pages = {013008},
      doi = {10.1103/PhysRevD.66.013008},
   adsurl = {http://adsabs.harvard.edu/abs/2002PhRvD..66a3008A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002PhRvD..66b5015W,
   author = {{Wong}, Y.~Y.},
    title = "{Analytical treatment of neutrino asymmetry equilibration from flavor oscillations in the early universe}",
  journal = {\prd},
   eprint = {hep-ph/0203180},
 keywords = {Neutrino mass and mixing, Neutrino interactions, Background radiations},
     year = 2002,
    month = jul,
   volume = 66,
   number = 2,
      eid = {025015},
    pages = {025015},
      doi = {10.1103/PhysRevD.66.025015},
   adsurl = {http://adsabs.harvard.edu/abs/2002PhRvD..66b5015W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Abazajian201566,
   author = {{Abazajian}, K.~N. and et al.},
    title = "{Neutrino physics from the cosmic microwave background and large scale structure}",
  journal = {Astroparticle Physics},
     year = 2015,
    month = mar,
   volume = 63,
    pages = {66-80},
      doi = {10.1016/j.astropartphys.2014.05.014},
   adsurl = {http://adsabs.harvard.edu/abs/2015APh....63...66A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{Kaplinghat,
   author = "Manoj Kaplinghat",
   year = {2013}, 
   howpublished = "private communication",
}
@Article{Lewis:1999bs,
     author    = "Lewis, Antony and Challinor, Anthony and Lasenby, Anthony",
     title     = "Efficient Computation of {CMB} anisotropies in closed {FRW}
                  models",
     journal   = "Astrophys. J.",
     volume    = "538",
     year      = "2000",
     pages     = "473-476",
     eprint    = "astro-ph/9911177",

     SLACcitation  = "%%CITATION = ASTRO-PH 9911177;%%"
}

@ARTICLE{2000NuPhB.590..562D,
   author = {{Dolgov}, A.~D. and {Hansen}, S.~H. and {Raffelt}, G. and {Semikoz}, D.~V.
	},
    title = "{Heavy sterile neutrinos: bounds from big-bang nucleosynthesis and SN 1987A}",
  journal = {Nuclear Physics B},
   eprint = {hep-ph/0008138},
     year = 2000,
    month = dec,
   volume = 590,
    pages = {562-574},
      doi = {10.1016/S0550-3213(00)00566-6},
   adsurl = {http://adsabs.harvard.edu/abs/2000NuPhB.590..562D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...600...26H,
   author = {{Hansen}, S.~H. and {Haiman}, Z.},
    title = "{Do We Need Stars to Reionize the Universe at High Redshifts? Early Reionization by Decaying Heavy Sterile Neutrinos}",
  journal = {\apj},
   eprint = {astro-ph/0305126},
 keywords = {Cosmology: Theory, Galaxies: Intergalactic Medium, Neutrinos},
     year = 2004,
    month = jan,
   volume = 600,
    pages = {26-31},
      doi = {10.1086/379636},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...600...26H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1990eaun.book.....K,
   author = {{Kolb}, E.~W. and {Turner}, M.~S.},
    title = "{The Early Universe.}",
publisher = "Addison-Wesley Publishing Co.",
 keywords = {Elementary Particles: Early Universe, Elementary Particles: Cosmology},
     year = 1990,
   adsurl = {http://adsabs.harvard.edu/abs/1990eaun.book.....K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009PhR...472....1I,
   author = {{Iocco}, F. and {Mangano}, G. and {Miele}, G. and {Pisanti}, O. and 
	{Serpico}, P.~D.},
    title = "{Primordial nucleosynthesis: From precision cosmology to fundamental physics}",
  journal = {\physrep},
archivePrefix = "arXiv",
   eprint = {0809.0631},
     year = 2009,
    month = mar,
   volume = 472,
    pages = {1-76},
      doi = {10.1016/j.physrep.2009.02.002},
   adsurl = {http://adsabs.harvard.edu/abs/2009PhR...472....1I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009NuPhS.188...15M,
   author = {{Miele}, G. and {Pisanti}, O.},
    title = "{Primordial Nucleosynthesis: an updated comparison of observational light nuclei abundances with theoretical predictions}",
  journal = {Nuclear Physics B Proceedings Supplements},
archivePrefix = "arXiv",
   eprint = {0811.4479},
     year = 2009,
    month = mar,
   volume = 188,
    pages = {15-19},
      doi = {10.1016/j.nuclphysbps.2009.02.002},
   adsurl = {http://adsabs.harvard.edu/abs/2009NuPhS.188...15M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010JPhCS.259a2007M,
   author = {{Miele}, G. and {Pisanti}, O. and {Sarikas}, S.},
    title = "{Primordial Nucleosynthesis and Neutrino Physics Beyond the Standard Model}",
  journal = {Journal of Physics Conference Series},
     year = 2010,
    month = nov,
   volume = 259,
   number = 1,
      eid = {012007},
    pages = {012007},
      doi = {10.1088/1742-6596/259/1/012007},
   adsurl = {http://adsabs.harvard.edu/abs/2010JPhCS.259a2007M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008CoPhC.178..956P,
   author = {{Pisanti}, O. and {Cirillo}, A. and {Esposito}, S. and {Iocco}, F. and 
	{Mangano}, G. and {Miele}, G. and {Serpico}, P.~D.},
    title = "{PArthENoPE: Public algorithm evaluating the nucleosynthesis of primordial elements}",
  journal = {Computer Physics Communications},
archivePrefix = "arXiv",
   eprint = {0705.0290},
 keywords = {Big Bang nucleosynthesis},
     year = 2008,
    month = jun,
   volume = 178,
    pages = {956-971},
      doi = {10.1016/j.cpc.2008.02.015},
   adsurl = {http://adsabs.harvard.edu/abs/2008CoPhC.178..956P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012CoPhC.183.1822A,
   author = {{Arbey}, A.},
    title = "{AlterBBN: A program for calculating the BBN abundances of the elements in alternative cosmologies}",
  journal = {Computer Physics Communications},
archivePrefix = "arXiv",
   eprint = {1106.1363},
 primaryClass = "astro-ph.CO",
 keywords = {Big-Bang Nucleosynthesis, Early Universe, Alternative cosmologies},
     year = 2012,
    month = aug,
   volume = 183,
    pages = {1822-1831},
      doi = {10.1016/j.cpc.2012.03.018},
   adsurl = {http://adsabs.harvard.edu/abs/2012CoPhC.183.1822A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FFN:IV,
   author = {{Fuller}, G.~M. and {Fowler}, W.~A. and {Newman}, M.~J.},
    title = "{Stellar weak interaction rates for intermediate-mass nuclei. IV - Interpolation procedures for rapidly varying lepton capture rates using effective log (ft)-values}",
  journal = {\apj},
 keywords = {Leptons, Neutrinos, Nuclear Capture, Stellar Cores, Weak Interactions (Field Theory), Computational Astrophysics, Computerized Simulation, Electron Capture},
     year = 1985,
    month = jun,
   volume = 293,
    pages = {1-16},
      doi = {10.1086/163208},
   adsurl = {http://adsabs.harvard.edu/abs/1985ApJ...293....1F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Book{mABR70a,
  author =	 {M. Abramowitz and I. A. Stegun},
  title = 	 {Handbook of Mathematical Functions with Formulas, Graphs, and Mathematical Tables (Partially Mathcad-enabled)},
  publisher = 	 {U. S. Department of Commerce, NIST},
  year = 	 {1972},
  address = 	 {New York},
  note = {Online version available at: http://app.knovel.com/hotlink/toc/id:kpHMFFGMT1/handbook-mathematical/handbook-mathematical}
}

@ARTICLE{letsgoeu2,
   author = {{Kawano}, L.},
    title = "{Let's go: Early universe 2. Primordial nucleosynthesis the computer way}",
  journal = {NASA STI/Recon Technical Report},
 keywords = {Nuclear Fusion, Runge-Kutta Method, Universe, User Manuals (Computer Programs), Algorithms, Computation, Fortran},
     year = 1992,
    month = jan,
   volume = 92,
    pages = {25163},
   adsurl = {http://adsabs.harvard.edu/abs/1992STIN...9225163K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{opac-b1131978,
   title = "An introduction to quantum field theory",
   author = "Peskin, Michael Edward and Schroeder, Daniel V.",
   series = "Advanced book program",
   publisher = "Westview Press Reading (Mass.)",
   address = "Boulder (Colo.)",
   url = "http://opac.inria.fr/record=b1131978",
   isbn = "0-201-50934-2",
   note = "Autre tirage : 1997",
   year = 1995
}

@book{Press:1993:NRF:563041,
 author = {Press, William H. and Teukolsky, Saul A. and Vetterling, William T. and Flannery, Brian P.},
 title = {Numerical Recipes in FORTRAN; The Art of Scientific Computing},
 year = {1993},
 isbn = {0521437164},
 edition = {2nd},
 publisher = {Cambridge University Press},
 address = {New York, NY, USA},
} 

@ARTICLE{1995PhRvD..52.1764H,
   author = {{Hannestad}, S. and {Madsen}, J.},
    title = "{Neutrino decoupling in the early Universe}",
  journal = {\prd},
   eprint = {astro-ph/9506015},
 keywords = {Elementary particle processes, Neutrino interactions, Neutrino mass and mixing, Origin formation and abundances of the elements},
     year = 1995,
    month = aug,
   volume = 52,
    pages = {1764-1769},
      doi = {10.1103/PhysRevD.52.1764},
   adsurl = {http://adsabs.harvard.edu/abs/1995PhRvD..52.1764H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1988kteu.book.....B,
   author = {{Bernstein}, J.},
     year = 1988,
    title = "{Kinetic theory in the expanding universe}",
 keywords = {Astronomical Models, Computational Astrophysics, Cosmology, Kinetic Theory, Black Body Radiation, Canonical Forms, Elementary Particles, Neutrinos, Relativistic Theory},
    publisher = {Cambridge and New York, Cambridge University Press, 157 p.},
   adsurl = {http://adsabs.harvard.edu/abs/1988kteu.book.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015NuPhB.890..481B,
   author = {{Birrell}, J. and {Yang}, C.~T. and {Rafelski}, J.},
    title = "{Relic neutrino freeze-out: Dependence on natural constants}",
  journal = {Nuclear Physics B},
archivePrefix = "arXiv",
   eprint = {1406.1759},
 primaryClass = "nucl-th",
     year = 2015,
    month = jan,
   volume = 890,
    pages = {481-517},
      doi = {10.1016/j.nuclphysb.2014.11.020},
   adsurl = {http://adsabs.harvard.edu/abs/2015NuPhB.890..481B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{Pathria_stat_mech,
 author = {Press, Raj K.},
 title = {Statistical Mechanics},
 year = {1996},
 isbn = {0750624698},
 edition = {2nd},
 publisher = {Butterworth-Heinemann},
 address = {Woburn, MA, USA},
} 

@ARTICLE{1999NuPhB.543..269D,
   author = {{Dolgov}, A.~D. and {Hansen}, S.~H. and {Semikoz}, D.~V.},
    title = "{Non-equilibrium corrections to the spectra of massless neutrinos in the early universe}",
  journal = {Nuclear Physics B},
   eprint = {hep-ph/9805467},
 keywords = {NEUTRINO, EARLY UNIVERSE, NON-EQUILIBRIUM KINETICS, CMB ANISOTROPIES},
     year = 1999,
    month = mar,
   volume = 543,
    pages = {269-274},
      doi = {10.1016/S0550-3213(98)00818-9},
   adsurl = {http://adsabs.harvard.edu/abs/1999NuPhB.543..269D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000NuPhB.590..539E,
   author = {{Esposito}, S. and {Miele}, G. and {Pastor}, S. and {Peloso}, M. and 
	{Pisanti}, O.},
    title = "{Non equilibrium spectra of degenerate relic neutrinos}",
  journal = {Nuclear Physics B},
   eprint = {astro-ph/0005573},
     year = 2000,
    month = dec,
   volume = 590,
    pages = {539-561},
      doi = {10.1016/S0550-3213(00)00554-X},
   adsurl = {http://adsabs.harvard.edu/abs/2000NuPhB.590..539E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{neff:3.046,
   author = {{Mangano}, G. and {Miele}, G. and {Pastor}, S. and {Pinto}, T. and 
	{Pisanti}, O. and {Serpico}, P.~D.},
    title = "{Relic neutrino decoupling including flavour oscillations}",
  journal = {Nuclear Physics B},
   eprint = {hep-ph/0506164},
     year = 2005,
    month = nov,
   volume = 729,
    pages = {221-234},
      doi = {10.1016/j.nuclphysb.2005.09.041},
   adsurl = {http://adsabs.harvard.edu/abs/2005NuPhB.729..221M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1982PhRvD..26.2694D,
   author = {{Dicus}, D.~A. and {Kolb}, E.~W. and {Gleeson}, A.~M. and {Sudarshan}, E.~C.~G. and 
	{Teplitz}, V.~L. and {Turner}, M.~S.},
    title = "{Primordial nucleosynthesis including radiative, Coulomb, and finite-temperature corrections to weak rates}",
  journal = {\prd},
     year = 1982,
    month = nov,
   volume = 26,
    pages = {2694-2706},
      doi = {10.1103/PhysRevD.26.2694},
   adsurl = {http://adsabs.harvard.edu/abs/1982PhRvD..26.2694D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989ApJ...336..539H,
   author = {{Herrera}, M.~A. and {Hacyan}, S.},
    title = "{Relaxation time of neutrinos in the early universe}",
  journal = {\apj},
 keywords = {Neutrinos, Relaxation Time, Universe, Nuclear Fusion, Particle Interactions, Relativistic Theory},
     year = 1989,
    month = jan,
   volume = 336,
    pages = {539-543},
      doi = {10.1086/167032},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...336..539H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991PhRvD..44..393R,
   author = {{Rana}, N.~C. and {Mitra}, B.},
    title = "{Effect of neutrino heating in the early Universe on neutrino decoupling temperatures and nucleosynthesis}",
  journal = {\prd},
     year = 1991,
    month = jul,
   volume = 44,
    pages = {393-397},
      doi = {10.1103/PhysRevD.44.393},
   adsurl = {http://adsabs.harvard.edu/abs/1991PhRvD..44..393R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992PhRvD..46.3372D,
   author = {{Dodelson}, S. and {Turner}, M.~S.},
    title = "{Nonequilibrium neutrino statistical mechanics in the expanding Universe}",
  journal = {\prd},
 keywords = {Origin formation and abundances of the elements},
     year = 1992,
    month = oct,
   volume = 46,
    pages = {3372-3387},
      doi = {10.1103/PhysRevD.46.3372},
   adsurl = {http://adsabs.harvard.edu/abs/1992PhRvD..46.3372D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992PhRvD..46.5378D,
   author = {{Dolgov}, A.~D. and {Fukugita}, M.},
    title = "{Nonequilibrium effect of the neutrino distribution on primordial helium synthesis}",
  journal = {\prd},
 keywords = {Origin formation and abundances of the elements},
     year = 1992,
    month = dec,
   volume = 46,
    pages = {5378-5382},
      doi = {10.1103/PhysRevD.46.5378},
   adsurl = {http://adsabs.harvard.edu/abs/1992PhRvD..46.5378D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{1999PhRvD..59j3502L,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/1999PhRvD..59j3502L},
	Author = {{Lopez}, R.~E. and {Turner}, M.~S.},
	Date-Added = {2014-09-11 17:03:44 +0000},
	Date-Modified = {2014-09-11 17:03:44 +0000},
	Doi = {10.1103/PhysRevD.59.103502},
	Eid = {103502},
	Eprint = {astro-ph/9807279},
	Journal = {\prd},
	Keywords = {Origin formation and abundances of the elements, Finite-temperature field theory, Specific calculations, Big Bang nucleosynthesis},
	Month = may,
	Number = 10,
	Pages = {103502},
	Title = {{Precision prediction for the big-bang abundance of primordial $^{4}$He}},
	Volume = 59,
	Year = 1999,
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevD.59.103502}}

@ARTICLE{1982NuPhB.209..372C,
   author = {{Cambier}, J.-L. and {Primack}, J.~R. and {Sher}, M.},
    title = "{Finite temperature radiative corrections to neutron decay and related processes}",
  journal = {Nucl. Phys. B},
     year = 1982,
    month = dec,
   volume = 209,
    pages = {372-388},
      doi = {10.1016/0550-3213(82)90262-0},
   adsurl = {http://adsabs.harvard.edu/abs/1982NuPhB.209..372C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{2014PhRvL.112p1303A,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {http://adsabs.harvard.edu/abs/2014PhRvL.112p1303A},
	Archiveprefix = {arXiv},
	Author = {{Abazajian}, K.~N.},
	Date-Added = {2014-09-11 15:11:10 +0000},
	Date-Modified = {2014-09-11 15:11:10 +0000},
	Doi = {10.1103/PhysRevLett.112.161303},
	Eid = {161303},
	Eprint = {1403.0954},
	OPTJournal = {Physical Review Letters},
	Journal = {Phys.~Rev.~Lett.},
	Keywords = {Dark matter, Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Galaxy groups clusters and superclusters, large scale structure of the Universe},
	Month = apr,
	Number = 16,
	Pages = {161303},
	Title = {{Resonantly Produced 7{\^A} keV Sterile Neutrino Dark Matter Models and the Properties of Milky Way Satellites}},
	Volume = 112,
	Year = 2014,
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevLett.112.161303}}

@BOOK{1990bmc..book.....D,
   author = {{Dolgov}, A.~D. and {Sazhin}, M.~V. and {Zeldovich}, Y.~B.},
    title = "{Basics of modern cosmology}",
 keywords = {Astronomical Models, Cosmology, Hubble Constant, Universe, Vacuum Effects, Background Radiation, Baryons, Gravitation Theory, Gravitational Waves, Relativistic Effects, Relic Radiation, Space Plasmas, String Theory, Weak Interactions (Field Theory)},
booktitle = {Gif-sur-Yvette, France, Editions Frontieres, 1990, 251 p.~Translation.},
     year = 1990,
   adsurl = {http://adsabs.harvard.edu/abs/1990bmc..book.....D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006PhRvL..97n1301K,
   author = {{Kishimoto}, C.~T. and {Fuller}, G.~M. and {Smith}, C.~J.},
    title = "{Coherent Active-Sterile Neutrino Flavor Transformation in the Early Universe}",
  OPTjournal = {Physical Review Letters},
  journal = {Phys.~Rev.~Lett.},
   eprint = {astro-ph/0607403},
 keywords = {Big Bang nucleosynthesis, Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Particle-theory and field-theory models of the early Universe},
     year = 2006,
    month = oct,
   volume = 97,
   number = 14,
      eid = {141301},
    pages = {141301},
      doi = {10.1103/PhysRevLett.97.141301},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhRvL..97n1301K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hou.2013PhRvD..87h3008H,
   author = {{Hou}, Z. and {Keisler}, R. and {Knox}, L. and {Millea}, M. and 
	{Reichardt}, C.},
    title = "{How massless neutrinos affect the cosmic microwave background damping tail}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1104.2333},
 primaryClass = "astro-ph.CO",
 keywords = {Background radiations, Non-standard-model neutrinos right-handed neutrinos etc.},
     year = 2013,
    month = apr,
   volume = 87,
   number = 8,
      eid = {083008},
    pages = {083008},
      doi = {10.1103/PhysRevD.87.083008},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvD..87h3008H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Birrell.PhysRevD.89.023008,
  title = {Relic neutrinos: Physically consistent treatment of effective number of neutrinos and neutrino mass},
  author = {Birrell, Jeremiah and Yang, Cheng-Tao and Chen, Pisin and Rafelski, Johann},
  journal = {Phys. Rev. D},
  volume = {89},
  issue = {2},
  pages = {023008},
  numpages = {10},
  year = {2014},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.89.023008}
}

@ARTICLE{Lopez.1999PhRvL..82.3952L,
   author = {{Lopez}, R.~E. and {Dodelson}, S. and {Heckler}, A. and {Turner}, M.~S.
        },
    title = "{Precision Detection of the Cosmic Neutrino Background}",
  OPTjournal = {Physical Review Letters},
  journal = {Phys.~Rev.~Lett.},
   eprint = {astro-ph/9803095},
     year = 1999,
    month = may,
   volume = 82,
    pages = {3952-3955},
      doi = {10.1103/PhysRevLett.82.3952},
   adsurl = {http://adsabs.harvard.edu/abs/1999PhRvL..82.3952L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Zahn.PhysRevD.67.063002,
  title = {Probing the Friedmann equation during recombination with future cosmic microwave background experiments},
  author = {Zahn, Oliver and Zaldarriaga, Matias},
  journal = {Phys. Rev. D},
  volume = {67},
  issue = {6},
  pages = {063002},
  numpages = {11},
  year = {2003},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.67.063002}
}

@ARTICLE{Hu.1996ApJ.471.542H,
   author = {{Hu}, W. and {Sugiyama}, N.},
    title = "{Small-Scale Cosmological Perturbations: an Analytic Approach}",
  journal = {\apj},
   eprint = {astro-ph/9510117},
 keywords = {COSMOLOGY: COSMIC MICROWAVE BACKGROUND, COSMOLOGY: LARGE-SCALE STRUCTURE OF UNIVERSE, COSMOLOGY: THEORY, COSMOLOGY: DARK MATTER, ELEMENTARY PARTICLES},
     year = 1996,
    month = nov,
   volume = 471,
    pages = {542},
      doi = {10.1086/177989},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...471..542H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010PhRvL.105r1301H,
   author = {{Hamann}, J. and {Hannestad}, S. and {Raffelt}, G.~G. and {Tamborra},
I. and 
        {Wong}, Y.~Y.~Y.},
    title = "{Cosmology Favoring Extra Radiation and Sub-eV Mass Sterile Neutrinos
as an Option}",
  OPTjournal = {Physical Review Letters},
  journal = {Phys.~Rev.~Lett.},
archivePrefix = "arXiv",
   eprint = {1006.5276},
 primaryClass = "hep-ph",
 keywords = {Observational cosmology, Neutrino mass and mixing, Non-standard-model
neutrinos right-handed neutrinos etc., Particle-theory and field-theory models of
the early Universe},
     year = 2010,
    month = oct,
   volume = 105,
   number = 18,
      eid = {181301},
    pages = {181301},
      doi = {10.1103/PhysRevLett.105.181301},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvL.105r1301H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011JCAP...09..034H,
   author = {{Hamann}, J. and {Hannestad}, S. and {Raffelt}, G.~G. and {Wong}, Y.~Y.~Y.
        },
    title = "{Sterile neutrinos with eV masses in cosmology - How disfavoured
exactly?}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1108.4136},
 primaryClass = "astro-ph.CO",
     year = 2011,
    month = sep,
   volume = 9,
      eid = {034},
    pages = {34},
      doi = {10.1088/1475-7516/2011/09/034},
   adsurl = {http://adsabs.harvard.edu/abs/2011JCAP...09..034H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhRvD..90h3503D,
   author = {{Dvorkin}, C. and {Wyman}, M. and {Rudd}, D.~H. and {Hu}, W.
        },
    title = "{Neutrinos help reconcile Planck measurements with both the early and
local Universe}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1403.8049},
 keywords = {Cosmology, Neutrino muon pion and other elementary particles, cosmic
rays, Background radiations, Observational cosmology},
     year = 2014,
    month = oct,
   volume = 90,
   number = 8,
      eid = {083503},
    pages = {083503},
      doi = {10.1103/PhysRevD.90.083503},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..90h3503D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...782...74H,
   author = {{Hou}, Z. and {Reichardt}, C.~L. and {Story}, K.~T. and {Follin}, B. and 
	{Keisler}, R. and {Aird}, K.~A. and {Benson}, B.~A. and {Bleem}, L.~E. and 
	{Carlstrom}, J.~E. and {Chang}, C.~L. and {Cho}, H.-M. and {Crawford}, T.~M. and 
	{Crites}, A.~T. and {de Haan}, T. and {de Putter}, R. and {Dobbs}, M.~A. and 
	{Dodelson}, S. and {Dudley}, J. and {George}, E.~M. and {Halverson}, N.~W. and 
	{Holder}, G.~P. and {Holzapfel}, W.~L. and {Hoover}, S. and 
	{Hrubes}, J.~D. and {Joy}, M. and {Knox}, L. and {Lee}, A.~T. and 
	{Leitch}, E.~M. and {Lueker}, M. and {Luong-Van}, D. and {McMahon}, J.~J. and 
	{Mehl}, J. and {Meyer}, S.~S. and {Millea}, M. and {Mohr}, J.~J. and 
	{Montroy}, T.~E. and {Padin}, S. and {Plagge}, T. and {Pryke}, C. and 
	{Ruhl}, J.~E. and {Sayre}, J.~T. and {Schaffer}, K.~K. and {Shaw}, L. and 
	{Shirokoff}, E. and {Spieler}, H.~G. and {Staniszewski}, Z. and 
	{Stark}, A.~A. and {van Engelen}, A. and {Vanderlinde}, K. and 
	{Vieira}, J.~D. and {Williamson}, R. and {Zahn}, O.},
    title = "{Constraints on Cosmology from the Cosmic Microwave Background Power Spectrum of the 2500 deg$^{2}$ SPT-SZ Survey}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1212.6267},
 primaryClass = "astro-ph.CO",
 keywords = {cosmic background radiation, cosmological parameters, early universe, inflation},
     year = 2014,
    month = feb,
   volume = 782,
      eid = {74},
    pages = {74},
      doi = {10.1088/0004-637X/782/2/74},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...782...74H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005NuPhB.708..215C,
   author = {{Cirelli}, M. and {Marandella}, G. and {Strumia}, A. and {Vissani}, F.
	},
    title = "{Probing oscillations into sterile neutrinos with cosmology, astrophysics and experiments}",
  journal = {Nuclear Physics B},
   eprint = {hep-ph/0403158},
 keywords = {14.60.Pq, 14.60.St, 26.35.+c, 97.60.Bw},
     year = 2005,
    month = feb,
   volume = 708,
    pages = {215-267},
      doi = {10.1016/j.nuclphysb.2004.11.056},
   adsurl = {http://adsabs.harvard.edu/abs/2005NuPhB.708..215C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Howlett:2012mh,
      author         = "Howlett, Cullan and Lewis, Antony and Hall, Alex and
                        Challinor, Anthony",
      title          = "{CMB power spectrum parameter degeneracies in the era of
                        precision cosmology}",
      journal        = "JCAP",
      volume         = "1204",
      pages          = "027",
      year           = "2012",
      eprint         = "1201.3654",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.CO",
}

@ARTICLE{SPT:2003IA,
   author = {{Carlstrom}, J.~E. and {Spt Collaboration}},
    title = "{The 8m South Pole Telescope}",
  journal = {IAU Special Session},
     year = 2003,
   volume = 2,
    pages = {34},
}

@ARTICLE{GFKP-5pts:2014mn,
   author = {{Grohs}, E. and {Fuller}, G.~M. and {Kishimoto}, C.~T. and {Paris}, M.~W.
	},
    title = "{Probing neutrino physics with a self-consistent treatment of the weak decoupling, nucleosynthesis, and photon decoupling epochs}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1502.02718},
     year = 2015,
    month = may,
   volume = 5,
      eid = {017},
    pages = {017},
      doi = {10.1088/1475-7516/2015/05/017},
   adsurl = {http://adsabs.harvard.edu/abs/2015JCAP...05..017G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{2008cosm.book.....W,
   author = {{Weinberg}, S.},
    title = "{Cosmology}",
booktitle = {Cosmology, by Steven Weinberg.~ISBN 978-0-19-852682-7.~Published by Oxford University Press, Oxford, UK, 2008.},
     year = 2008,
publisher = {Oxford University Press},
   adsurl = {http://adsabs.harvard.edu/abs/2008cosm.book.....W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhRvD..89g3013B,
   author = {{Balantekin}, A.~B. and {Vassh}, N.},
    title = "{Magnetic moments of active and sterile neutrinos}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1312.6858},
 primaryClass = "hep-ph",
 keywords = {Neutrino mass and mixing, Ordinary neutrinos (nuW bosons, Non-standard-model neutrinos right-handed neutrinos etc.},
     year = 2014,
    month = apr,
   volume = 89,
   number = 7,
      eid = {073013},
    pages = {073013},
      doi = {10.1103/PhysRevD.89.073013},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..89g3013B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013JCAP...04..041B,
   author = {{Bae}, K.~J. and {Baer}, H. and {Lessa}, A.},
    title = "{Dark radiation constraints on mixed Axion/Neutralino dark matter}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1301.7428},
 primaryClass = "hep-ph",
     year = 2013,
    month = apr,
   volume = 4,
      eid = {041},
    pages = {41},
      doi = {10.1088/1475-7516/2013/04/041},
   adsurl = {http://adsabs.harvard.edu/abs/2013JCAP...04..041B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{adams2008,
   author = {{Adams}, F.~C.},
    title = "{Stars in other universes: stellar structure with different fundamental constants}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {0807.3697},
     year = 2008,
    month = aug,
   volume = 8,
      eid = {010},
    pages = {10},
      doi = {10.1088/1475-7516/2008/08/010},
   adsurl = {http://adsabs.harvard.edu/abs/2008JCAP...08..010A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{coppess,
   author = {{Adams}, F.~C. and {Coppess}, K.~R. and {Bloch}, A.~M.},
    title = "{Planets in other universes: habitability constraints on density fluctuations and galactic structure}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1505.06158},
     year = 2015,
    month = sep,
   volume = 9,
      eid = {030},
    pages = {030},
      doi = {10.1088/1475-7516/2015/09/030},
   adsurl = {http://adsabs.harvard.edu/abs/2015JCAP...09..030A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Elhay:1987:AIF:35078.214351,
 author = {Elhay, Sylvan and Kautsky, Jaroslav},
 title = {Algorithm 655: IQPACK: FORTRAN Subroutines for the Weights of Interpolatory Quadratures},
 journal = {ACM Trans. Math. Softw.},
 issue_date = {Dec. 1987},
 volume = {13},
 number = {4},
 month = dec,
 year = {1987},
 issn = {0098-3500},
 pages = {399--415},
 numpages = {17},
 url = {http://doi.acm.org/10.1145/35078.214351},
 doi = {10.1145/35078.214351},
 acmid = {214351},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {approximate integration, interpolatory quadrature, multiple knot quadratures, quadrature coefficients, simple Gaussian quadrature},
} 

@ARTICLE{1994PhRvD..49..611H,
   author = {{Heckler}, A.~F.},
    title = "{Astrophysical applications of quantum corrections to the equation of state of a plasma}",
  journal = {\prd},
 keywords = {Elementary particle processes, Origin formation and abundances of the elements},
     year = 1994,
    month = jan,
   volume = 49,
    pages = {611-617},
      doi = {10.1103/PhysRevD.49.611},
   adsurl = {http://adsabs.harvard.edu/abs/1994PhRvD..49..611H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997PhRvD..56.5123F,
   author = {{Fornengo}, N. and {Kim}, C.~W. and {Song}, J.},
    title = "{Finite temperature effects on the neutrino decoupling in the early Universe}",
  journal = {\prd},
   eprint = {hep-ph/9702324},
 keywords = {Finite-temperature field theory, Elementary particle processes, Thermodynamic processes conduction convection equations of state},
     year = 1997,
    month = oct,
   volume = 56,
    pages = {5123-5134},
      doi = {10.1103/PhysRevD.56.5123},
   adsurl = {http://adsabs.harvard.edu/abs/1997PhRvD..56.5123F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975ApJ...201..467T,
   author = {{Tubbs}, D.~L. and {Schramm}, D.~N.},
    title = "{Neutrino Opacities at High Temperatures and Densities}",
  journal = {\apj},
     year = 1975,
    month = oct,
   volume = 201,
    pages = {467-488},
      doi = {10.1086/153909},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...201..467T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1976ApJ...208L..19F,
   author = {{Flowers}, E.~G. and {Sutherland}, P.~G.},
    title = "{Neutrino-neutrino scattering and supernovae}",
  journal = {\apjl},
 keywords = {Gravitational Collapse, Neutrinos, Scattering Cross Sections, Supernovae, Inelastic Scattering, Particle Collisions},
     year = 1976,
    month = aug,
   volume = 208,
    pages = {L19-L21},
      doi = {10.1086/182223},
   adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...208L..19F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJS..149....1K,
   author = {{Kirkman}, D. and {Tytler}, D. and {Suzuki}, N. and {O'Meara}, J.~M. and 
	{Lubin}, D.},
    title = "{The Cosmological Baryon Density from the Deuterium-to-Hydrogen Ratio in QSO Absorption Systems: D/H toward Q1243+3047}",
  journal = {\apjs},
   eprint = {astro-ph/0302006},
 keywords = {Cosmology: Observations, Nuclear Reactions, Nucleosynthesis, Abundances, Galaxies: Quasars: Absorption Lines, Galaxies: Quasars: Individual: Alphanumeric: Q1243+3047},
     year = 2003,
    month = nov,
   volume = 149,
    pages = {1-28},
      doi = {10.1086/378152},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJS..149....1K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000PhR...333..409T,
   author = {{Tytler}, D. and {O'Meara}, J.~M. and {Suzuki}, N. and {Lubin}, D.
	},
    title = "{Deuterium and the baryonic density of the universe}",
  journal = {\physrep},
     year = 2000,
    month = aug,
   volume = 333,
    pages = {409-432},
      doi = {10.1016/S0370-1573(00)00032-6},
   adsurl = {http://adsabs.harvard.edu/abs/2000PhR...333..409T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010PhRvD..81f5027S,
   author = {{Smith}, C.~J. and {Fuller}, G.~M.},
    title = "{Weak interaction rate Coulomb corrections in big bang nucleosynthesis}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0905.2781},
 primaryClass = "astro-ph.CO",
 keywords = {Big Bang nucleosynthesis, Neutrino mass and mixing, Fundamental aspects of astrophysics},
     year = 2010,
    month = mar,
   volume = 81,
   number = 6,
      eid = {065027},
    pages = {065027},
      doi = {10.1103/PhysRevD.81.065027},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvD..81f5027S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FFN:I,
   author = {{Fuller}, G.~M. and {Fowler}, W.~A. and {Newman}, M.~J.},
    title = "{Stellar weak-interaction rates for sd-shell nuclei. I - Nuclear matrix element systematics with application to Al-26 and selected nuclei of importance to the supernova problem}",
  journal = {\apjs},
 keywords = {Neutrinos, Nuclear Astrophysics, Nuclear Reactions, Supernovae, Weak Interactions (Field Theory), Aluminum 26, Electron Capture, Electron Transitions, Energy Dissipation, Positrons, Reaction Kinetics},
     year = 1980,
    month = mar,
   volume = 42,
    pages = {447-473},
      doi = {10.1086/190657},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJS...42..447F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Adelberger:2011bp,
   author = {{Adelberger}, E.~G. and others},
    title = "{Solar fusion cross sections. II. The pp chain and CNO cycles}",
  journal = {Reviews of Modern Physics},
archivePrefix = "arXiv",
   eprint = {1004.2318},
 primaryClass = "nucl-ex",
 keywords = {Stellar hydrogen burning, Solar neutrinos, Solar interior, Nuclear reactions involving few-nucleon systems},
     year = 2011,
    month = jan,
   volume = 83,
    pages = {195-246},
      doi = {10.1103/RevModPhys.83.195},
   adsurl = {http://adsabs.harvard.edu/abs/2011RvMP...83..195A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{cmbs4uofc,
  title = {Cosmology with {CMB S4} workshop},
  howpublished = {\url{https://cosmo.uchicago.edu/CMB-S4workshops/index.php/UMICH-2015:Neutrino_and_Light_Relativisic_Species_Summary}},
  author = {Dan Green},
  note = {{Accessed}: 2015-11-11}
}
@ARTICLE{Nollett:2014bb,
   author = {{Nollett}, K.~M. and {Steigman}, G.},
    title = "{BBN and the CMB constrain light, electromagnetically coupled WIMPs}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1312.5725},
 keywords = {Big Bang nucleosynthesis, Dark matter, Particle-theory and field-theory models of the early Universe, Non-standard-model neutrinos right-handed neutrinos etc.},
     year = 2014,
    month = apr,
   volume = 89,
   number = 8,
   note   = {and Private Communication},
      eid = {083508},
    pages = {083508},
      doi = {10.1103/PhysRevD.89.083508},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..89h3508N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Marcucci:2015dp,
   author = {{Marcucci}, L.~E. and {Mangano}, G. and {Kievsky}, A. and {Viviani}, M.
        },
    title = "{Implication of the proton-deuteron radiative capture for Big Bang Nucleosynthesis}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1510.07877},
 primaryClass = "nucl-th",
 keywords = {Nuclear Theory, Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2015,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2015arXiv151007877M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vassh_tdecoup,
   author = {{Vassh}, N. and {Grohs}, E. and {Balantekin}, A.~B. and {Fuller}, G.~M.
	},
    title = "{Majorana neutrino magnetic moment and neutrino decoupling in big bang nucleosynthesis}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1510.00428},
 keywords = {Neutrino interactions, Big Bang nucleosynthesis, Non-standard-model neutrinos right-handed neutrinos etc., Ordinary neutrinos (nuW bosons)},
     year = 2015,
    month = dec,
   volume = 92,
   number = 12,
      eid = {125020},
    pages = {125020},
      doi = {10.1103/PhysRevD.92.125020},
   adsurl = {http://adsabs.harvard.edu/abs/2015PhRvD..92l5020V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015PhRvD..91h3505N,
   author = {{Nollett}, K.~M. and {Steigman}, G.},
    title = "{BBN and the CMB constrain neutrino coupled light WIMPs}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1411.6005},
 keywords = {Big Bang nucleosynthesis, Non-standard-model neutrinos right-handed neutrinos etc., Dark matter, Particle-theory and field-theory models of the early Universe},
     year = 2015,
    month = apr,
   volume = 91,
   number = 8,
      eid = {083505},
    pages = {083505},
      doi = {10.1103/PhysRevD.91.083505},
   adsurl = {http://adsabs.harvard.edu/abs/2015PhRvD..91h3505N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009PhRvD..79j5001S,
   author = {{Smith}, C.~J. and {Fuller}, G.~M. and {Smith}, M.~S.},
    title = "{Big bang nucleosynthesis with independent neutrino distribution functions}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0812.1253},
 keywords = {Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Big Bang nucleosynthesis, Fundamental aspects of astrophysics},
     year = 2009,
    month = may,
   volume = 79,
   number = 10,
      eid = {105001},
    pages = {105001},
      doi = {10.1103/PhysRevD.79.105001},
   adsurl = {http://adsabs.harvard.edu/abs/2009PhRvD..79j5001S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...423...50J,
   author = {{Jedamzik}, K. and {Fuller}, G.~M. and {Mathews}, G.~J.},
    title = "{Inhomogeneous primordial nucleosynthesis: Coupled nuclear reactions and hydrodynamic dissipation processes}",
  journal = {\apj},
   eprint = {astro-ph/9312065},
 keywords = {Big Bang Cosmology, Coupled Modes, Dissipation, Hydrodynamic Equations, Inhomogeneity, Nuclear Fusion, Abundance, Baryons, Heat Transmission, Neutrinos, Photons},
     year = 1994,
    month = mar,
   volume = 423,
    pages = {50-67},
      doi = {10.1086/173789},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...423...50J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013arXiv1310.4340D,
   author = {{de Gouvea}, A. and et al.},
    title = "{Neutrinos}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1310.4340},
 primaryClass = "hep-ex",
 keywords = {High Energy Physics - Experiment, High Energy Physics - Phenomenology},
     year = 2013,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1310.4340D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991NuPhB.349..743B,
   author = {{Barbieri}, R. and {Dolgov}, A.},
    title = "{Neutrino oscillations in the early universe}",
  journal = {Nuclear Physics B},
     year = 1991,
    month = feb,
   volume = 349,
    pages = {743-753},
      doi = {10.1016/0550-3213(91)90396-F},
   adsurl = {http://adsabs.harvard.edu/abs/1991NuPhB.349..743B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AkhmedovBerezhiani,
   author = {{Akhmedov}, E.~K. and {Berezhiani}, Z.~G.},
    title = "{Implications of Majorana neutrino transition magnetic moments for neutrino signals from supernovae}",
  journal = {Nuclear Physics B},
     year = 1992,
    month = apr,
   volume = 373,
    pages = {479-497},
      doi = {10.1016/0550-3213(92)90441-D},
   adsurl = {http://adsabs.harvard.edu/abs/1992NuPhB.373..479A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gouvea,
   author = {{de Gouv{\^e}a}, A. and {Shalgar}, S.},
    title = "{Transition magnetic moments and collective neutrino oscillations: three-flavor effects and detectability}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1301.5637},
 primaryClass = "astro-ph.HE",
     year = 2013,
    month = apr,
   volume = 4,
      eid = {018},
    pages = {18},
      doi = {10.1088/1475-7516/2013/04/018},
   adsurl = {http://adsabs.harvard.edu/abs/2013JCAP...04..018D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993APh.....1..165R,
   author = {{Raffelt}, G. and {Sigl}, G.},
    title = "{Neutrino flavor conversion in a supernova core}",
  journal = {Astroparticle Physics},
   eprint = {astro-ph/9209005},
     year = 1993,
    month = mar,
   volume = 1,
    pages = {165-183},
      doi = {10.1016/0927-6505(93)90020-E},
   adsurl = {http://adsabs.harvard.edu/abs/1993APh.....1..165R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005PhRvD..71i3004S,
   author = {{Strack}, P. and {Burrows}, A.},
    title = "{Generalized Boltzmann formalism for oscillating neutrinos}",
  journal = {\prd},
   eprint = {hep-ph/0504035},
 keywords = {Neutrino mass and mixing, Quantum ensemble theory, Classical transport},
     year = 2005,
    month = may,
   volume = 71,
   number = 9,
      eid = {093004},
    pages = {093004},
      doi = {10.1103/PhysRevD.71.093004},
   adsurl = {http://adsabs.harvard.edu/abs/2005PhRvD..71i3004S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007JPhG...34...47B,
   author = {{Balantekin}, A.~B. and {Pehlivan}, Y.},
    title = "{Neutrino neutrino interactions and flavour mixing in dense matter}",
  journal = {Journal of Physics G Nuclear Physics},
   eprint = {astro-ph/0607527},
     year = 2007,
    month = jan,
   volume = 34,
    pages = {47-65},
      doi = {10.1088/0954-3899/34/1/004},
   adsurl = {http://adsabs.harvard.edu/abs/2007JPhG...34...47B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013PrPNP..71..162B,
   author = {{Balantekin}, A.~B. and {Fuller}, G.~M.},
    title = "{Neutrinos in cosmology and astrophysics}",
  journal = {Progress in Particle and Nuclear Physics},
archivePrefix = "arXiv",
   eprint = {1303.3874},
 primaryClass = "nucl-th",
     year = 2013,
    month = jul,
   volume = 71,
    pages = {162-166},
      doi = {10.1016/j.ppnp.2013.03.008},
   adsurl = {http://adsabs.harvard.edu/abs/2013PrPNP..71..162B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015PhLB..747...27C,
   author = {{Cirigliano}, V. and {Fuller}, G.~M. and {Vlasenko}, A.},
    title = "{A new spin on neutrino quantum kinetics}",
  journal = {Physics Letters B},
archivePrefix = "arXiv",
   eprint = {1406.5558},
 primaryClass = "hep-ph",
     year = 2015,
    month = jul,
   volume = 747,
    pages = {27-35},
      doi = {10.1016/j.physletb.2015.04.066},
   adsurl = {http://adsabs.harvard.edu/abs/2015PhLB..747...27C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Trans_BBN,
   author = {{Grohs}, E. and {Fuller}, G.~M. and {Kishimoto}, C.~T. and {Paris}, M.~W. and 
	{Vlasenko}, A.},
    title = "{Neutrino energy transport in weak decoupling and big bang nucleosynthesis}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1512.02205},
     year = 2016,
    month = apr,
   volume = 93,
   number = 8,
      eid = {083522},
    pages = {083522},
      doi = {10.1103/PhysRevD.93.083522},
   adsurl = {http://adsabs.harvard.edu/abs/2016PhRvD..93h3522G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997PhRvD..56.3191L,
   author = {{Lopez}, R.~E. and {Turner}, M.~S. and {Gyuk}, G.},
    title = "{Effect of finite nucleon mass on primordial nucleosynthesis}",
  journal = {\prd},
   eprint = {astro-ph/9703065},
 keywords = {Stellar structure interiors evolution nucleosynthesis ages, Neutrino interactions, Hadronic decays},
     year = 1997,
    month = sep,
   volume = 56,
    pages = {3191-3197},
      doi = {10.1103/PhysRevD.56.3191},
   adsurl = {http://adsabs.harvard.edu/abs/1997PhRvD..56.3191L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012PhRvC..85f5503S,
   author = {{Steyerl}, A. and {Pendlebury}, J.~M. and {Kaufman}, C. and 
	{Malik}, S.~S. and {Desai}, A.~M.},
    title = "{Quasielastic scattering in the interaction of ultracold neutrons with a liquid wall and application in a reanalysis of the Mambo I neutron-lifetime experiment}",
  journal = {\prc},
 keywords = {Neutron physics, Protons and neutrons, Lifetimes, Nuclear reaction models and methods},
     year = 2012,
    month = jun,
   volume = 85,
   number = 6,
      eid = {065503},
    pages = {065503},
      doi = {10.1103/PhysRevC.85.065503},
   adsurl = {http://adsabs.harvard.edu/abs/2012PhRvC..85f5503S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013PhRvL.111v2501Y,
   author = {{Yue}, A.~T. and {Dewey}, M.~S. and {Gilliam}, D.~M. and {Greene}, G.~L. and 
	{Laptev}, A.~B. and {Nico}, J.~S. and {Snow}, W.~M. and {Wietfeldt}, F.~E.
	},
    title = "{Improved Determination of the Neutron Lifetime}",
  journal = {Physical Review Letters},
archivePrefix = "arXiv",
   eprint = {1309.2623},
 primaryClass = "nucl-ex",
 keywords = {Lifetimes, Protons and neutrons, Beta decay, double beta decay, electron and muon capture, Big Bang nucleosynthesis},
     year = 2013,
    month = nov,
   volume = 111,
   number = 22,
      eid = {222501},
    pages = {222501},
      doi = {10.1103/PhysRevLett.111.222501},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvL.111v2501Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002PhR...370..333D,
   author = {{Dolgov}, A.~D.},
    title = "{Neutrinos in cosmology}",
  journal = {\physrep},
   eprint = {hep-ph/0202122},
     year = 2002,
    month = nov,
   volume = 370,
    pages = {333-535},
      doi = {10.1016/S0370-1573(02)00139-4},
   adsurl = {http://adsabs.harvard.edu/abs/2002PhR...370..333D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016MNRAS.455.1512C,
   author = {{Cooke}, R. and {Pettini}, M.},
    title = "{The primordial abundance of deuterium: ionization correction}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1510.03867},
 keywords = {methods: numerical, galaxies: abundances, galaxies: ISM, quasars: absorption lines, cosmological parameters, primordial nucleosynthesis},
     year = 2016,
    month = jan,
   volume = 455,
    pages = {1512-1521},
      doi = {10.1093/mnras/stv2343},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.455.1512C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{B2FH,
   author = {{Burbidge}, E.~M. and {Burbidge}, G.~R. and {Fowler}, W.~A. and 
	{Hoyle}, F.},
    title = "{Synthesis of the Elements in Stars}",
  journal = {Reviews of Modern Physics},
     year = 1957,
   volume = 29,
    pages = {547-650},
      doi = {10.1103/RevModPhys.29.547},
   adsurl = {http://adsabs.harvard.edu/abs/1957RvMP...29..547B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012arXiv1208.0032S,
   author = {{Steigman}, G.},
    title = "{Neutrinos And Big Bang Nucleosynthesis}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1208.0032},
 primaryClass = "hep-ph",
 keywords = {High Energy Physics - Phenomenology, Astrophysics - Cosmology and Extragalactic Astrophysics, Nuclear Experiment, Nuclear Theory},
     year = 2012,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2012arXiv1208.0032S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998RvMP...70..303S,
   author = {{Schramm}, D.~N. and {Turner}, M.~S.},
    title = "{Big-bang nucleosynthesis enters the precision era}",
  journal = {Reviews of Modern Physics},
   eprint = {astro-ph/9706069},
     year = 1998,
    month = jan,
   volume = 70,
    pages = {303-318},
      doi = {10.1103/RevModPhys.70.303},
   adsurl = {http://adsabs.harvard.edu/abs/1998RvMP...70..303S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cyburt:2016RMP,
   author = {{Cyburt}, R.~H. and {Fields}, B.~D. and {Olive}, K.~A. and {Yeh}, T.-H.
	},
    title = "{Big bang nucleosynthesis: Present status}",
  journal = {Reviews of Modern Physics},
archivePrefix = "arXiv",
   eprint = {1505.01076},
     year = 2016,
    month = jan,
   volume = 88,
   number = 1,
      eid = {015004},
    pages = {015004},
      doi = {10.1103/RevModPhys.88.015004},
   adsurl = {http://adsabs.harvard.edu/abs/2016RvMP...88a5004C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016JCAP...07..051D,
   author = {{de Salas}, P.~F. and {Pastor}, S.},
    title = "{Relic neutrino decoupling with flavour oscillations revisited}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1606.06986},
 primaryClass = "hep-ph",
     year = 2016,
    month = jul,
   volume = 7,
      eid = {051},
    pages = {051},
      doi = {10.1088/1475-7516/2016/07/051},
   adsurl = {http://adsabs.harvard.edu/abs/2016JCAP...07..051D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989RvMP...61...25B,
   author = {{Bernstein}, J. and {Brown}, L.~S. and {Feinberg}, G.},
    title = "{Cosmological helium production simplified}",
  journal = {Reviews of Modern Physics},
     year = 1989,
    month = jan,
   volume = 61,
    pages = {25-39},
      doi = {10.1103/RevModPhys.61.25},
   adsurl = {http://adsabs.harvard.edu/abs/1989RvMP...61...25B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993PhRvL..71.1965Q,
   author = {{Qian}, Y.-Z. and {Fuller}, G.~M. and {Mathews}, G.~J. and {Mayle}, R.~W. and 
	{Wilson}, J.~R. and {Woosley}, S.~E.},
    title = "{Connection between flavor mixing of cosmologically significant neutrinos and heavy element nucleosynthesis in supernovae}",
  journal = {Physical Review Letters},
 keywords = {Heavy Elements, Neutrinos, Nuclear Fusion, Supernovae, Flavor (Particle Physics), Stellar Mass Ejection},
     year = 1993,
    month = sep,
   volume = 71,
    pages = {1965-1968},
      doi = {10.1103/PhysRevLett.71.1965},
   adsurl = {http://adsabs.harvard.edu/abs/1993PhRvL..71.1965Q},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhRvD..90h3519I,
   author = {{Ishida}, H. and {Kusakabe}, M. and {Okada}, H.},
    title = "{Effects of long-lived 10 MeV-scale sterile neutrinos on primordial elemental abundances and the effective neutrino number}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1403.5995},
 keywords = {Big Bang nucleosynthesis, Dark matter, Particle-theory and field-theory models of the early Universe, Observational cosmology},
     year = 2014,
    month = oct,
   volume = 90,
   number = 8,
      eid = {083519},
    pages = {083519},
      doi = {10.1103/PhysRevD.90.083519},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..90h3519I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014NuPhB.888..248B,
   author = {{Boyanovsky}, D.},
    title = "{Space-time evolution of heavy sterile neutrinos in cascade decays}",
  journal = {Nuclear Physics B},
archivePrefix = "arXiv",
   eprint = {1406.5739},
 primaryClass = "hep-ph",
     year = 2014,
    month = nov,
   volume = 888,
    pages = {248-270},
      doi = {10.1016/j.nuclphysb.2014.09.018},
   adsurl = {http://adsabs.harvard.edu/abs/2014NuPhB.888..248B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhRvD..90j5024B,
   author = {{Boyanovsky}, D.},
    title = "{Nearly degenerate heavy sterile neutrinos in cascade decay: Mixing and oscillations}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1409.4265},
 primaryClass = "hep-ph",
 keywords = {Field theory, Other nonperturbative techniques, Other topics in general theory of fields and particles},
     year = 2014,
    month = nov,
   volume = 90,
   number = 10,
      eid = {105024},
    pages = {105024},
      doi = {10.1103/PhysRevD.90.105024},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..90j5024B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015PhRvD..91f3502L,
   author = {{Lello}, L. and {Boyanovsky}, D.},
    title = "{Cosmological implications of light sterile neutrinos produced after the QCD phase transition}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1411.2690},
 keywords = {Dark matter, Neutrino interactions, Elementary particle processes},
     year = 2015,
    month = mar,
   volume = 91,
   number = 6,
      eid = {063502},
    pages = {063502},
      doi = {10.1103/PhysRevD.91.063502},
   adsurl = {http://adsabs.harvard.edu/abs/2015PhRvD..91f3502L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cmbs4_science_book,
   author = {{Carlstrom}, J.~E. and et al.},
    title = "{CMB-S4 Science Book, First Edition}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1610.02743},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, General Relativity and Quantum Cosmology, High Energy Physics - Phenomenology, High Energy Physics - Theory},
     year = 2016,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161002743A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016arXiv160801336J,
   author = {{Johns}, L. and {Mina}, M. and {Cirigliano}, V. and {Paris}, M.~W. and 
	{Fuller}, G.~M.},
    title = "{Neutrino flavor transformation in the lepton-asymmetric universe}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1608.01336},
 primaryClass = "hep-ph",
     year = 2016,
    month = oct,
   volume = 94,
   number = 8,
      eid = {083505},
    pages = {083505},
      doi = {10.1103/PhysRevD.94.083505},
   adsurl = {http://adsabs.harvard.edu/abs/2016PhRvD..94h3505J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013PhRvD..87g3006S,
   author = {{Saviano}, N. and {Mirizzi}, A. and {Pisanti}, O. and {Serpico}, P.~D. and 
	{Mangano}, G. and {Miele}, G.},
    title = "{Multimomentum and multiflavor active-sterile neutrino oscillations in the early universe: Role of neutrino asymmetries and effects on nucleosynthesis}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1302.1200},
 primaryClass = "astro-ph.CO",
 keywords = {Non-standard-model neutrinos right-handed neutrinos etc., Neutrino mass and mixing, Big Bang nucleosynthesis, Cosmology},
     year = 2013,
    month = apr,
   volume = 87,
   number = 7,
      eid = {073006},
    pages = {073006},
      doi = {10.1103/PhysRevD.87.073006},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvD..87g3006S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{gradshteyn2007,
  added-at = {2011-05-02T05:41:34.000+0200},
  author = {Gradshteyn, I. S. and Ryzhik, I. M.},
  biburl = {http://www.bibsonomy.org/bibtex/2bae535b4ef6bc86a7a04e6de6fa4d311/peter.ralph},
  description = {MR: Publications results for "MR Number=(2360010)"},
  edition = {Seventh},
  interhash = {1850c3bd20bb756bfc17136ec16a9a7c},
  intrahash = {bae535b4ef6bc86a7a04e6de6fa4d311},
  isbn = {978-0-12-373637-6; 0-12-373637-4},
  keywords = {reference},
  mrclass = {00A22 (33-00 65-00 65A05)},
  mrnumber = {2360010 (2008g:00005)},
  note = {Translated from the Russian, Translation edited and with a preface by Alan Jeffrey and Daniel Zwillinger, With one CD-ROM (Windows, Macintosh and UNIX)},
  pages = {xlviii+1171},
  publisher = {Elsevier/Academic Press, Amsterdam},
  timestamp = {2011-05-02T05:41:34.000+0200},
  title = {Table of integrals, series, and products},
  year = 2007
}

@ARTICLE{WFO_approx,
   author = {{Grohs}, E. and {Fuller}, G.~M.},
    title = "{The surprising influence of late charged current weak interactions on Big Bang Nucleosynthesis}",
  journal = {Nuclear Physics B},
archivePrefix = "arXiv",
   eprint = {1607.02797},
     year = 2016,
    month = oct,
   volume = 911,
    pages = {955-973},
      doi = {10.1016/j.nuclphysb.2016.08.034},
   adsurl = {http://adsabs.harvard.edu/abs/2016NuPhB.911..955G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2014EPJWC..6900003P,
   author = {{Paris}, M.~W. and {Brown}, L.~S. and {Hale}, G.~M. and {Hayes-Sterbenz}, A.~C. and 
	{Jungman}, G. and {Kawano}, T. and {Fuller}, G.~M. and {Grohs}, E. and 
	{Kunieda}, S.},
    title = "{Toward a self-consistent and unitary reaction network for big-bang nucleosynthesis}",
booktitle = {European Physical Journal Web of Conferences},
     year = 2014,
   series = {European Physical Journal Web of Conferences},
   volume = 69,
    month = apr,
      eid = {00003},
    pages = {00003},
      doi = {10.1051/epjconf/20136900003},
   adsurl = {http://adsabs.harvard.edu/abs/2014EPJWC..6900003P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Unpublished{BMW:2017,
     author    = "J. Richard Bond and George M. Fuller and E. Grohs and Joel Meyers and Matthew Wilson",
     note      = "in preparation",
     year      = "2017",
}

@ARTICLE{1996PhRvD..54.2753S,
   author = {{Shi}, X.},
    title = "{Chaotic amplification of neutrino chemical potentials by neutrino oscillations in big bang nucleosynthesis}",
  journal = {\prd},
   eprint = {astro-ph/9602135},
 keywords = {Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Big Bang nucleosynthesis, Dark matter},
     year = 1996,
    month = aug,
   volume = 54,
    pages = {2753-2760},
      doi = {10.1103/PhysRevD.54.2753},
   adsurl = {http://adsabs.harvard.edu/abs/1996PhRvD..54.2753S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002PhRvD..65b3511H,
   author = {{Hansen}, S.~H. and {Mangano}, G. and {Melchiorri}, A. and {Miele}, G. and 
	{Pisanti}, O.},
    title = "{Constraining neutrino physics with big bang nucleosynthesis and cosmic microwave background radiation}",
  journal = {\prd},
   eprint = {astro-ph/0105385},
 keywords = {Particle-theory and field-theory models of the early Universe, Gravity in more than four dimensions Kaluza-Klein theory unified field theories, alternative theories of gravity, Dark matter, Background radiations},
     year = 2001,
    month = dec,
   volume = 65,
   number = 2,
      eid = {023511},
    pages = {023511},
      doi = {10.1103/PhysRevD.65.023511},
   adsurl = {http://adsabs.harvard.edu/abs/2002PhRvD..65b3511H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005PhRvD..71l7301S,
   author = {{Serpico}, P.~D. and {Raffelt}, G.~G.},
    title = "{Lepton asymmetry and primordial nucleosynthesis in the era of precision cosmology}",
  journal = {\prd},
   eprint = {astro-ph/0506162},
 keywords = {Big Bang nucleosynthesis, Ordinary neutrinos (nuW bosons, Observational cosmology},
     year = 2005,
    month = jun,
   volume = 71,
   number = 12,
      eid = {127301},
    pages = {127301},
      doi = {10.1103/PhysRevD.71.127301},
   adsurl = {http://adsabs.harvard.edu/abs/2005PhRvD..71l7301S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009JCAP...07..005S,
   author = {{Shiraishi}, M. and {Ichikawa}, K. and {Ichiki}, K. and {Sugiyama}, N. and 
	{Yamaguchi}, M.},
    title = "{Constraints on neutrino masses from WMAP5 and BBN in the lepton asymmetric universe}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {0904.4396},
 primaryClass = "astro-ph.CO",
     year = 2009,
    month = jul,
   volume = 7,
      eid = {005},
    pages = {005},
      doi = {10.1088/1475-7516/2009/07/005},
   adsurl = {http://adsabs.harvard.edu/abs/2009JCAP...07..005S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012PhRvD..86b3517C,
   author = {{Castorina}, E. and {Fran{\c c}a}, U. and {Lattanzi}, M. and 
	{Lesgourgues}, J. and {Mangano}, G. and {Melchiorri}, A. and 
	{Pastor}, S.},
    title = "{Cosmological lepton asymmetry with a nonzero mixing angle ${\theta}_{13}$}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1204.2510},
 primaryClass = "astro-ph.CO",
 keywords = {Cosmology, Neutrino mass and mixing, Big Bang nucleosynthesis, Background radiations},
     year = 2012,
    month = jul,
   volume = 86,
   number = 2,
      eid = {023517},
    pages = {023517},
      doi = {10.1103/PhysRevD.86.023517},
   adsurl = {http://adsabs.harvard.edu/abs/2012PhRvD..86b3517C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012PhLB..708....1M,
   author = {{Mangano}, G. and {Miele}, G. and {Pastor}, S. and {Pisanti}, O. and 
	{Sarikas}, S.},
    title = "{Updated BBN bounds on the cosmological lepton asymmetry for non-zero {\thetas}$_{}$}",
  journal = {Physics Letters B},
archivePrefix = "arXiv",
   eprint = {1110.4335},
 primaryClass = "hep-ph",
     year = 2012,
    month = feb,
   volume = 708,
    pages = {1-5},
      doi = {10.1016/j.physletb.2012.01.015},
   adsurl = {http://adsabs.harvard.edu/abs/2012PhLB..708....1M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011JCAP...03..035M,
   author = {{Mangano}, G. and {Miele}, G. and {Pastor}, S. and {Pisanti}, O. and 
	{Sarikas}, S.},
    title = "{Constraining the cosmic radiation density due to lepton number with Big Bang Nucleosynthesis}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1011.0916},
     year = 2011,
    month = mar,
   volume = 3,
      eid = {035},
    pages = {035},
      doi = {10.1088/1475-7516/2011/03/035},
   adsurl = {http://adsabs.harvard.edu/abs/2011JCAP...03..035M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006PhRvD..74h5015C,
   author = {{Chu}, Y.-Z. and {Cirelli}, M.},
    title = "{Sterile neutrinos, lepton asymmetries, primordial elements: How much of each?}",
  journal = {\prd},
   eprint = {astro-ph/0608206},
 keywords = {Non-standard-model neutrinos right-handed neutrinos etc., Neutrino mass and mixing, Big Bang nucleosynthesis, Cosmology},
     year = 2006,
    month = oct,
   volume = 74,
   number = 8,
      eid = {085015},
    pages = {085015},
      doi = {10.1103/PhysRevD.74.085015},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhRvD..74h5015C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998NuPhB.534..447K,
   author = {{Kirilova}, D.~P. and {Chizhov}, M.~V.},
    title = "{Neutrino degeneracy effect on neutrino oscillations and primordial helium yield}",
  journal = {Nuclear Physics B},
   eprint = {hep-ph/9806441},
 keywords = {NEUTRINO OSCILLATIONS, LEPTON ASYMMETRY, COSMOLOGICAL NUCLEOSYNTHESIS},
     year = 1998,
    month = nov,
   volume = 534,
    pages = {447-463},
      doi = {10.1016/S0550-3213(98)00641-5},
   adsurl = {http://adsabs.harvard.edu/abs/1998NuPhB.534..447K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016arXiv160903200B,
   author = {{Barenboim}, G. and {Kinney}, W.~H. and {Park}, W.-I.},
    title = "{Flavor versus mass eigenstates in neutrino asymmetries: implications for cosmology}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1609.03200},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology},
     year = 2016,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160903200B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dark_rad:2000,
   author = {{Mukohyama}, S.},
    title = "{Brane-world solutions, standard cosmology, and dark radiation}",
  journal = {Physics Letters B},
   eprint = {hep-th/9911165},
     year = 2000,
    month = feb,
   volume = 473,
    pages = {241-245},
      doi = {10.1016/S0370-2693(99)01505-1},
   adsurl = {http://adsabs.harvard.edu/abs/2000PhLB..473..241M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999PhRvL..82.2832S,
   author = {{Shi}, X. and {Fuller}, G.~M.},
    title = "{New Dark Matter Candidate: Nonthermal Sterile Neutrinos}",
  journal = {Physical Review Letters},
   eprint = {astro-ph/9810076},
     year = 1999,
    month = apr,
   volume = 82,
    pages = {2832-2835},
      doi = {10.1103/PhysRevLett.82.2832},
   adsurl = {http://adsabs.harvard.edu/abs/1999PhRvL..82.2832S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016arXiv160204816A,
   author = {{Adhikari}, R. and et al.},
    title = "{A White Paper on keV Sterile Neutrino Dark Matter}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1602.04816},
 primaryClass = "hep-ph",
 keywords = {High Energy Physics - Phenomenology, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, High Energy Physics - Experiment},
     year = 2016,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv160204816A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977ARNPS..27...37S,
   author = {{Schramm}, D.~N. and {Wagoner}, R.~V.},
    title = "{Element production in the early universe.}",
  journal = {Annual Review of Nuclear and Particle Science},
     year = 1977,
   volume = 27,
    pages = {37-74},
      doi = {10.1146/annurev.ns.27.120177.000345},
   adsurl = {http://adsabs.harvard.edu/abs/1977ARNPS..27...37S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1973ApJ...179..343W,
   author = {{Wagoner}, R.~V.},
    title = "{Big-Bang Nucleosynthesis Revisited}",
  journal = {\apj},
     year = 1973,
    month = jan,
   volume = 179,
    pages = {343-360},
      doi = {10.1086/151873},
   adsurl = {http://adsabs.harvard.edu/abs/1973ApJ...179..343W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001PhRvD..64l3506K,
   author = {{Kneller}, J.~P. and {Scherrer}, R.~J. and {Steigman}, G. and 
	{Walker}, T.~P.},
    title = "{How does the cosmic microwave background plus big bang nucleosynthesis constrain new physics?}",
  journal = {\prd},
   eprint = {astro-ph/0101386},
 keywords = {Observational cosmology, Big Bang nucleosynthesis, Background radiations},
     year = 2001,
    month = dec,
   volume = 64,
   number = 12,
    pages = {123506},
      doi = {10.1103/PhysRevD.64.123506},
   adsurl = {http://adsabs.harvard.edu/abs/2001PhRvD..64l3506K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...830..148C,
   author = {{Cooke}, R.~J. and {Pettini}, M. and {Nollett}, K.~M. and {Jorgenson}, R.
	},
    title = "{The Primordial Deuterium Abundance of the Most Metal-poor Damped Lyman-{$\alpha$} System}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1607.03900},
 keywords = {cosmology: observations, cosmology: theory, primordial nucleosynthesis, quasars: absorption lines, quasars: individual: J1358+0349 },
     year = 2016,
    month = oct,
   volume = 830,
      eid = {148},
    pages = {148},
      doi = {10.3847/0004-637X/830/2/148},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...830..148C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016JCAP...12..019S,
   author = {{Sloth Lundkvist Hansen}, R. and {Smirnov}, A.~Y.},
    title = "{The Liouville equation for flavour evolution of neutrinos and neutrino wave packets}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1610.00910},
 primaryClass = "hep-ph",
     year = 2016,
    month = dec,
   volume = 12,
      eid = {019},
    pages = {019},
      doi = {10.1088/1475-7516/2016/12/019},
   adsurl = {http://adsabs.harvard.edu/abs/2016JCAP...12..019S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016NuPhB.908..366C,
   author = {{Chakraborty}, S. and {Hansen}, R. and {Izaguirre}, I. and {Raffelt}, G.
	},
    title = "{Collective neutrino flavor conversion: Recent developments}",
  journal = {Nuclear Physics B},
archivePrefix = "arXiv",
   eprint = {1602.02766},
 primaryClass = "hep-ph",
     year = 2016,
    month = jul,
   volume = 908,
    pages = {366-381},
      doi = {10.1016/j.nuclphysb.2016.02.012},
   adsurl = {http://adsabs.harvard.edu/abs/2016NuPhB.908..366C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015IJMPE..2441009V,
   author = {{Volpe}, C.},
    title = "{Neutrino quantum kinetic equations}",
  journal = {International Journal of Modern Physics E},
archivePrefix = "arXiv",
   eprint = {1506.06222},
 primaryClass = "astro-ph.SR",
 keywords = {Neutrino masses and mixings, core-collapse supernova neutrinos, flavor conversion phenomena, mean-field, kinetic equations, linearisation, Neutrino mass and mixing, Supernovae, Neutrino interactions, Many-body theory},
     year = 2015,
    month = sep,
   volume = 24,
      eid = {1541009},
    pages = {1541009},
      doi = {10.1142/S0218301315410098},
   adsurl = {http://adsabs.harvard.edu/abs/2015IJMPE..2441009V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015NuPhB.891..128B,
   author = {{Bhupal Dev}, P.~S. and {Millington}, P. and {Pilaftsis}, A. and 
	{Teresi}, D.},
    title = "{Kadanoff-Baym approach to flavour mixing and oscillations in resonant leptogenesis}",
  journal = {Nuclear Physics B},
archivePrefix = "arXiv",
   eprint = {1410.6434},
 primaryClass = "hep-ph",
     year = 2015,
    month = feb,
   volume = 891,
    pages = {128-158},
      doi = {10.1016/j.nuclphysb.2014.12.003},
   adsurl = {http://adsabs.harvard.edu/abs/2015NuPhB.891..128B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Blaschke_Cirigliano_2016,
   author = {{Blaschke}, D.~N. and {Cirigliano}, V.},
    title = "{Neutrino quantum kinetic equations: The collision term}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1605.09383},
 primaryClass = "hep-ph",
     year = 2016,
    month = aug,
   volume = 94,
   number = 3,
      eid = {033009},
    pages = {033009},
      doi = {10.1103/PhysRevD.94.033009},
   adsurl = {http://adsabs.harvard.edu/abs/2016PhRvD..94c3009B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015RAA....15.1945S,
   author = {{Skidmore}, W. and {TMT International Science Development Teams} and 
	{Science Advisory Committee}, T.},
    title = "{Thirty Meter Telescope Detailed Science Case: 2015}",
  journal = {Research in Astronomy and Astrophysics},
archivePrefix = "arXiv",
   eprint = {1505.01195},
 primaryClass = "astro-ph.IM",
     year = 2015,
    month = dec,
   volume = 15,
      eid = {1945},
    pages = {1945},
      doi = {10.1088/1674-4527/15/12/001},
   adsurl = {http://adsabs.harvard.edu/abs/2015RAA....15.1945S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015PhRvD..92j3509P,
   author = {{Patwardhan}, A.~V. and {Fuller}, G.~M. and {Kishimoto}, C.~T. and 
	{Kusenko}, A.},
    title = "{Diluted equilibrium sterile neutrino dark matter}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1507.01977},
 keywords = {Dark matter, Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Elementary particle processes},
     year = 2015,
    month = nov,
   volume = 92,
   number = 10,
      eid = {103509},
    pages = {103509},
      doi = {10.1103/PhysRevD.92.103509},
   adsurl = {http://adsabs.harvard.edu/abs/2015PhRvD..92j3509P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AFP_2001,
   author = {{Abazajian}, K. and {Fuller}, G.~M. and {Patel}, M.},
    title = "{Sterile neutrino hot, warm, and cold dark matter}",
  journal = {\prd},
   eprint = {astro-ph/0101524},
 keywords = {Dark matter, Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Galaxy groups clusters and superclusters, large scale structure of the Universe},
     year = 2001,
    month = jul,
   volume = 64,
   number = 2,
      eid = {023501},
    pages = {023501},
      doi = {10.1103/PhysRevD.64.023501},
   adsurl = {http://adsabs.harvard.edu/abs/2001PhRvD..64b3501A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dod_Wid_1994,
   author = {{Dodelson}, S. and {Widrow}, L.~M.},
    title = "{Sterile neutrinos as dark matter}",
  journal = {Physical Review Letters},
   eprint = {hep-ph/9303287},
 keywords = {Particle-theory and field-theory models of the early Universe, Quark and lepton masses and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Dark matter},
     year = 1994,
    month = jan,
   volume = 72,
    pages = {17-20},
      doi = {10.1103/PhysRevLett.72.17},
   adsurl = {http://adsabs.harvard.edu/abs/1994PhRvL..72...17D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002APh....16..339D,
   author = {{Dolgov}, A.~D. and {Hansen}, S.~H.},
    title = "{Massive sterile neutrinos as warm dark matter}",
  journal = {Astroparticle Physics},
   eprint = {hep-ph/0009083},
     year = 2002,
    month = jan,
   volume = 16,
    pages = {339-344},
      doi = {10.1016/S0927-6505(01)00115-3},
   adsurl = {http://adsabs.harvard.edu/abs/2002APh....16..339D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002PhRvD..66b3526A,
   author = {{Abazajian}, K.~N. and {Fuller}, G.~M.},
    title = "{Bulk QCD thermodynamics and sterile neutrino dark matter}",
  journal = {\prd},
   eprint = {astro-ph/0204293},
 keywords = {Dark matter, Non-standard-model neutrinos right-handed neutrinos etc., Quark-gluon plasma, Relativistic heavy-ion collisions},
     year = 2002,
    month = jul,
   volume = 66,
   number = 2,
      eid = {023526},
    pages = {023526},
      doi = {10.1103/PhysRevD.66.023526},
   adsurl = {http://adsabs.harvard.edu/abs/2002PhRvD..66b3526A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005PhLB..620...17A,
   author = {{Asaka}, T. and {Shaposhnikov}, M.},
    title = "{The @nMSM, dark matter and baryon asymmetry of the universe [rapid communication]}",
  journal = {Physics Letters B},
   eprint = {hep-ph/0505013},
 keywords = {Neutrino mass and mixing, Particle-theory and field-theory models of the early Universe, Dark matter},
     year = 2005,
    month = jul,
   volume = 620,
    pages = {17-26},
      doi = {10.1016/j.physletb.2005.06.020},
   adsurl = {http://adsabs.harvard.edu/abs/2005PhLB..620...17A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005PhLB..631..151A,
   author = {{Asaka}, T. and {Blanchet}, S. and {Shaposhnikov}, M.},
    title = "{The {$\nu$}MSM, dark matter and neutrino masses [rapid communication]}",
  journal = {Physics Letters B},
   eprint = {hep-ph/0503065},
 keywords = {Neutrino mass and mixing, Particle-theory and field-theory models of the early Universe, Dark matter},
     year = 2005,
    month = dec,
   volume = 631,
    pages = {151-156},
      doi = {10.1016/j.physletb.2005.09.070},
   adsurl = {http://adsabs.harvard.edu/abs/2005PhLB..631..151A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006PhLB..638..401A,
   author = {{Asaka}, T. and {Shaposhnikov}, M. and {Kusenko}, A.},
    title = "{Opening a new window for warm dark matter}",
  journal = {Physics Letters B},
   eprint = {hep-ph/0602150},
 keywords = {Non-standard-model neutrinos right-handed neutrinos etc., Dark matter},
     year = 2006,
    month = jul,
   volume = 638,
    pages = {401-406},
      doi = {10.1016/j.physletb.2006.05.067},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhLB..638..401A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006PhLB..639..414S,
   author = {{Shaposhnikov}, M. and {Tkachev}, I.},
    title = "{The {$\nu$}MSM, inflation, and dark matter}",
  journal = {Physics Letters B},
   eprint = {hep-ph/0604236},
 keywords = {Neutrino mass and mixing, Particle-theory and field-theory models of the early Universe, Dark matter},
     year = 2006,
    month = aug,
   volume = 639,
    pages = {414-417},
      doi = {10.1016/j.physletb.2006.06.063},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhLB..639..414S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007JHEP...01..091A,
   author = {{Asaka}, T. and {Shaposhnikov}, M. and {Laine}, M.},
    title = "{Lightest sterile neutrino abundance within the {$\nu$}MSM}",
  journal = {Journal of High Energy Physics},
   eprint = {hep-ph/0612182},
     year = 2007,
    month = jan,
   volume = 1,
      eid = {091},
    pages = {091},
      doi = {10.1088/1126-6708/2007/01/091},
   adsurl = {http://adsabs.harvard.edu/abs/2007JHEP...01..091A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007NuPhB.763...49S,
   author = {{Shaposhnikov}, M.},
    title = "{A possible symmetry of the {$\nu$}MSM}",
  journal = {Nuclear Physics B},
   eprint = {hep-ph/0605047},
 keywords = {Neutrino mass and mixing, Particle-theory and field-theory models of the early Universe, Dark matter},
     year = 2007,
    month = feb,
   volume = 763,
    pages = {49-59},
      doi = {10.1016/j.nuclphysb.2006.11.003},
   adsurl = {http://adsabs.harvard.edu/abs/2007NuPhB.763...49S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007JHEP...07..030B,
   author = {{Boyanovsky}, D. and {Ho}, C.-M.},
    title = "{Sterile neutrino production via active-sterile oscillations: the quantum Zeno effect}",
  journal = {Journal of High Energy Physics},
   eprint = {hep-ph/0612092},
     year = 2007,
    month = jul,
   volume = 7,
      eid = {030},
    pages = {030},
      doi = {10.1088/1126-6708/2007/07/030},
   adsurl = {http://adsabs.harvard.edu/abs/2007JHEP...07..030B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007PhRvD..76j3514B,
   author = {{Boyanovsky}, D.},
    title = "{Production of a sterile species via active-sterile mixing: An exactly solvable model}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0706.3167},
 primaryClass = "hep-ph",
 keywords = {Particle-theory and field-theory models of the early Universe, Finite-temperature field theory, Neutrino mass and mixing},
     year = 2007,
    month = nov,
   volume = 76,
   number = 10,
      eid = {103514},
    pages = {103514},
      doi = {10.1103/PhysRevD.76.103514},
   adsurl = {http://adsabs.harvard.edu/abs/2007PhRvD..76j3514B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010PhRvD..81h5032B,
   author = {{Bezrukov}, F. and {Hettmansperger}, H. and {Lindner}, M.},
    title = "{keV sterile neutrino dark matter in gauge extensions of the standard model}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {0912.4415},
 primaryClass = "hep-ph",
 keywords = {Non-standard-model neutrinos right-handed neutrinos etc., Models beyond the standard model, Neutrino mass and mixing, Dark matter},
     year = 2010,
    month = apr,
   volume = 81,
   number = 8,
      eid = {085032},
    pages = {085032},
      doi = {10.1103/PhysRevD.81.085032},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvD..81h5032B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010PhLB..693..144K,
   author = {{Kusenko}, A. and {Takahashi}, F. and {Yanagida}, T.~T.},
    title = "{Dark matter from split seesaw}",
  journal = {Physics Letters B},
archivePrefix = "arXiv",
   eprint = {1006.1731},
 primaryClass = "hep-ph",
     year = 2010,
    month = sep,
   volume = 693,
    pages = {144-148},
      doi = {10.1016/j.physletb.2010.08.031},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhLB..693..144K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013PhRvL.110f1801C,
   author = {{Canetti}, L. and {Drewes}, M. and {Shaposhnikov}, M.},
    title = "{Sterile Neutrinos as the Origin of Dark and Baryonic Matter}",
  journal = {Physical Review Letters},
archivePrefix = "arXiv",
   eprint = {1204.3902},
 primaryClass = "hep-ph",
 keywords = {Non-standard-model neutrinos right-handed neutrinos etc., Neutrino mass and mixing, Dark matter, Particle-theory and field-theory models of the early Universe},
     year = 2013,
    month = feb,
   volume = 110,
   number = 6,
      eid = {061801},
    pages = {061801},
      doi = {10.1103/PhysRevLett.110.061801},
   adsurl = {http://adsabs.harvard.edu/abs/2013PhRvL.110f1801C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013IJMPD..2230020M,
   author = {{Merle}, A.},
    title = "{keV Neutrino Model Building}",
  journal = {International Journal of Modern Physics D},
archivePrefix = "arXiv",
   eprint = {1302.2625},
 primaryClass = "hep-ph",
 keywords = {Neutrinos, dark matter, model building, Neutrino mass and mixing, Non-standard-model neutrinos right-handed neutrinos etc., Miscellaneous theoretical ideas and models, Dark matter},
     year = 2013,
    month = aug,
   volume = 22,
      eid = {1330020},
    pages = {1330020},
      doi = {10.1142/S0218271813300206},
   adsurl = {http://adsabs.harvard.edu/abs/2013IJMPD..2230020M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013JPhG...40i5202B,
   author = {{Bezrukov}, F. and {Kartavtsev}, A. and {Lindner}, M.},
    title = "{Leptogenesis in models with keV sterile neutrino dark matter}",
  journal = {Journal of Physics G Nuclear Physics},
archivePrefix = "arXiv",
   eprint = {1204.5477},
 primaryClass = "hep-ph",
     year = 2013,
    month = sep,
   volume = 40,
   number = 9,
      eid = {095202},
    pages = {095202},
      doi = {10.1088/0954-3899/40/9/095202},
   adsurl = {http://adsabs.harvard.edu/abs/2013JPhG...40i5202B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014JCAP...03..028M,
   author = {{Merle}, A. and {Niro}, V. and {Schmidt}, D.},
    title = "{New production mechanism for keV sterile neutrino Dark Matter by decays of frozen-in scalars}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1306.3996},
 primaryClass = "hep-ph",
     year = 2014,
    month = mar,
   volume = 3,
      eid = {028},
    pages = {028},
      doi = {10.1088/1475-7516/2014/03/028},
   adsurl = {http://adsabs.harvard.edu/abs/2014JCAP...03..028M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015JHEP...09..064H,
   author = {{Humbert}, P. and {Lindner}, M. and {Patra}, S. and {Smirnov}, J.
	},
    title = "{Lepton number violation within the conformal inverse seesaw}",
  journal = {Journal of High Energy Physics},
archivePrefix = "arXiv",
   eprint = {1505.07453},
 primaryClass = "hep-ph",
 keywords = {Higgs Physics, Beyond Standard Model, Neutrino Physics},
     year = 2015,
    month = sep,
   volume = 9,
      eid = {64},
    pages = {64},
      doi = {10.1007/JHEP09(2015)064},
   adsurl = {http://adsabs.harvard.edu/abs/2015JHEP...09..064H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015PhLB..749..283M,
   author = {{Merle}, A. and {Schneider}, A.},
    title = "{Production of Sterile Neutrino dark matter and the 3.5 keV line}",
  journal = {Physics Letters B},
archivePrefix = "arXiv",
   eprint = {1409.6311},
 primaryClass = "hep-ph",
     year = 2015,
    month = oct,
   volume = 749,
    pages = {283-288},
      doi = {10.1016/j.physletb.2015.07.080},
   adsurl = {http://adsabs.harvard.edu/abs/2015PhLB..749..283M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016RPPh...79l4201A,
   author = {{Alekhin}, S. and et al.},
    title = "{A facility to search for hidden particles at the CERN SPS: the SHiP physics case}",
  journal = {Reports on Progress in Physics},
archivePrefix = "arXiv",
   eprint = {1504.04855},
 primaryClass = "hep-ph",
     year = 2016,
    month = dec,
   volume = 79,
   number = 12,
      eid = {124201},
    pages = {124201},
      doi = {10.1088/0034-4885/79/12/124201},
   adsurl = {http://adsabs.harvard.edu/abs/2016RPPh...79l4201A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2008AIPC.1016..403S,
   author = {{Smith}, M.~S. and {Bruner}, B.~D. and {Kozub}, R.~L. and {Roberts}, L.~F. and 
	{Tytler}, D. and {Fuller}, G.~M. and {Lingerfelt}, E. and {Hix}, W.~R. and 
	{Nesaraja}, C.~D.},
    title = "{Big Bang Nucleosynthesis: Impact of Nuclear Physics Uncertainties on Baryonic Matter Density Constraints}",
 keywords = {Cosmology, Origin formation and abundances of the elements, Fusion reactors},
booktitle = {Origin of Matter and Evolution of Galaxies},
     year = 2008,
   series = {American Institute of Physics Conference Series},
   volume = 1016,
   editor = {{Suda}, T. and {Nozawa}, T. and {Ohnishi}, A. and {Kato}, K. and 
	{Fujimoto}, M.~Y. and {Kajino}, T. and {Kubono}, S.},
    month = may,
    pages = {403-405},
      doi = {10.1063/1.2943606},
   adsurl = {http://adsabs.harvard.edu/abs/2008AIPC.1016..403S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015PhyS...90h8008K,
   author = {{Keister}, B.~D.},
    title = "{Numerical and physical stability of supernova neutrino flavor evolution}",
  journal = {\physscr},
archivePrefix = "arXiv",
   eprint = {1408.4729},
 primaryClass = "astro-ph.HE",
     year = 2015,
    month = aug,
   volume = 90,
   number = 8,
      eid = {088008},
    pages = {088008},
      doi = {10.1088/0031-8949/90/8/088008},
   adsurl = {http://adsabs.harvard.edu/abs/2015PhyS...90h8008K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015PhRvD..91l5020K,
   author = {{Kartavtsev}, A. and {Raffelt}, G. and {Vogel}, H.},
    title = "{Neutrino propagation in media: Flavor, helicity, and pair correlations}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1504.03230},
 primaryClass = "hep-ph",
 keywords = {Neutrino mass and mixing, Neutrino interactions, Supernovae},
     year = 2015,
    month = jun,
   volume = 91,
   number = 12,
      eid = {125020},
    pages = {125020},
      doi = {10.1103/PhysRevD.91.125020},
   adsurl = {http://adsabs.harvard.edu/abs/2015PhRvD..91l5020K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010PhRvD..82i3009G,
   author = {{Gu}, P.-H.},
    title = "{Large lepton asymmetry for small baryon asymmetry and warm dark matter}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1005.1632},
 primaryClass = "hep-ph",
 keywords = {Particle-theory and field-theory models of the early Universe, Extensions of electroweak gauge sector, Neutrino mass and mixing, Dark matter},
     year = 2010,
    month = nov,
   volume = 82,
   number = 9,
      eid = {093009},
    pages = {093009},
      doi = {10.1103/PhysRevD.82.093009},
   adsurl = {http://adsabs.harvard.edu/abs/2010PhRvD..82i3009G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010NuPhB.837...50G,
   author = {{Gava}, J. and {Volpe}, C.},
    title = "{CP violation effects on the neutrino degeneracy parameters in the Early Universe}",
  journal = {Nuclear Physics B},
archivePrefix = "arXiv",
   eprint = {1002.0981},
 primaryClass = "hep-ph",
     year = 2010,
    month = sep,
   volume = 837,
    pages = {50-60},
      doi = {10.1016/j.nuclphysb.2010.04.024},
   adsurl = {http://adsabs.harvard.edu/abs/2010NuPhB.837...50G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008JHEP...08..008S,
   author = {{Shaposhnikov}, M.},
    title = "{The {$\nu$}MSM, leptonic asymmetries, and properties of singlet fermions}",
  journal = {Journal of High Energy Physics},
archivePrefix = "arXiv",
   eprint = {0804.4542},
 primaryClass = "hep-ph",
     year = 2008,
    month = aug,
   volume = 8,
      eid = {008},
    pages = {008},
      doi = {10.1088/1126-6708/2008/08/008},
   adsurl = {http://adsabs.harvard.edu/abs/2008JHEP...08..008S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008JCAP...08..011S,
   author = {{Simha}, V. and {Steigman}, G.},
    title = "{Constraining the universal lepton asymmetry}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {0806.0179},
 primaryClass = "hep-ph",
     year = 2008,
    month = aug,
   volume = 8,
      eid = {011},
    pages = {011},
      doi = {10.1088/1475-7516/2008/08/011},
   adsurl = {http://adsabs.harvard.edu/abs/2008JCAP...08..011S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003PhRvD..68f3507Y,
   author = {{Yamaguchi}, M.},
    title = "{Generation of cosmological large lepton asymmetry from a rolling scalar field}",
  journal = {\prd},
   eprint = {hep-ph/0211163},
 keywords = {Particle-theory and field-theory models of the early Universe},
     year = 2003,
    month = sep,
   volume = 68,
   number = 6,
      eid = {063507},
    pages = {063507},
      doi = {10.1103/PhysRevD.68.063507},
   adsurl = {http://adsabs.harvard.edu/abs/2003PhRvD..68f3507Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002PhRvD..66d3516K,
   author = {{Kawasaki}, M. and {Takahashi}, F. and {Yamaguchi}, M.},
    title = "{Large lepton asymmetry from Q-balls}",
  journal = {\prd},
   eprint = {hep-ph/0205101},
 keywords = {Particle-theory and field-theory models of the early Universe},
     year = 2002,
    month = aug,
   volume = 66,
   number = 4,
      eid = {043516},
    pages = {043516},
      doi = {10.1103/PhysRevD.66.043516},
   adsurl = {http://adsabs.harvard.edu/abs/2002PhRvD..66d3516K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000PhRvL..84.4798M,
   author = {{McDonald}, J.},
    title = "{Naturally Large Cosmological Neutrino Asymmetries in the Minimal Supersymmetric Standard Model}",
  journal = {Physical Review Letters},
   eprint = {hep-ph/9908300},
     year = 2000,
    month = may,
   volume = 84,
    pages = {4798-4801},
      doi = {10.1103/PhysRevLett.84.4798},
   adsurl = {http://adsabs.harvard.edu/abs/2000PhRvL..84.4798M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999JHEP...11..015M,
   author = {{March-Russell}, J. and {Riotto}, A. and {Murayama}, H.},
    title = "{The small observed baryon asymmetry from a large lepton asymmetry}",
  journal = {Journal of High Energy Physics},
   eprint = {hep-ph/9908396},
     year = 1999,
    month = nov,
   volume = 11,
      eid = {015},
    pages = {015},
      doi = {10.1088/1126-6708/1999/11/015},
   adsurl = {http://adsabs.harvard.edu/abs/1999JHEP...11..015M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999PhRvD..59k3001B,
   author = {{Bell}, N.~F. and {Volkas}, R.~R. and {Wong}, Y.~Y.~Y.},
    title = "{Relic neutrino asymmetry evolution from first principles}",
  journal = {\prd},
   eprint = {hep-ph/9809363},
 keywords = {Neutrino mass and mixing, Neutrino interactions, Non-standard-model neutrinos right-handed neutrinos etc., Neutrino muon pion and other elementary particles, cosmic rays},
     year = 1999,
    month = jun,
   volume = 59,
   number = 11,
      eid = {113001},
    pages = {113001},
      doi = {10.1103/PhysRevD.59.113001},
   adsurl = {http://adsabs.harvard.edu/abs/1999PhRvD..59k3001B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999NuPhB.538..297C,
   author = {{Casas}, A. and {Cheng}, W.~Y. and {Gelmini}, G.},
    title = "{Generation of large lepton asymmetries}",
  journal = {Nuclear Physics B},
   eprint = {hep-ph/9709289},
     year = 1999,
    month = jan,
   volume = 538,
    pages = {297-308},
      doi = {10.1016/S0550-3213(98)00606-3},
   adsurl = {http://adsabs.harvard.edu/abs/1999NuPhB.538..297C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996PhRvD..53.5349F,
   author = {{Foot}, R. and {Thomson}, M.~J. and {Volkas}, R.~R.},
    title = "{Large neutrino asymmetries from neutrino oscillations}",
  journal = {\prd},
   eprint = {hep-ph/9509327},
 keywords = {Neutrino mass and mixing, Neutrino muon pion and other elementary particles, cosmic rays},
     year = 1996,
    month = may,
   volume = 53,
    pages = {R5349-R5353},
      doi = {10.1103/PhysRevD.53.R5349},
   adsurl = {http://adsabs.harvard.edu/abs/1996PhRvD..53.5349F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994PhRvD..49.2710M,
   author = {{McKellar}, B.~H.~J. and {Thomson}, M.~J.},
    title = "{Oscillating neutrinos in the early Universe}",
  journal = {\prd},
 keywords = {Particle-theory and field-theory models of the early Universe, Ordinary neutrinos (nuW bosons, Elementary particle processes},
     year = 1994,
    month = mar,
   volume = 49,
    pages = {2710-2728},
      doi = {10.1103/PhysRevD.49.2710},
   adsurl = {http://adsabs.harvard.edu/abs/1994PhRvD..49.2710M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1990PhRvD..42.3344H,
   author = {{Harvey}, J.~A. and {Turner}, M.~S.},
    title = "{Cosmological baryon and lepton number in the presence of electroweak fermion-number violation}",
  journal = {\prd},
     year = 1990,
    month = nov,
   volume = 42,
    pages = {3344-3349},
      doi = {10.1103/PhysRevD.42.3344},
   adsurl = {http://adsabs.harvard.edu/abs/1990PhRvD..42.3344H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981PhRvD..24.2090H,
   author = {{Harvey}, J.~A. and {Kolb}, E.~W.},
    title = "{Grand unified theories and the lepton number of the Universe}",
  journal = {\prd},
     year = 1981,
    month = oct,
   volume = 24,
    pages = {2090-2099},
      doi = {10.1103/PhysRevD.24.2090},
   adsurl = {http://adsabs.harvard.edu/abs/1981PhRvD..24.2090H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{h2_unstable,
   author = {{Adams}, F.~C. and {Grohs}, E.},
    title = "{On the Habitability of Universes without Stable Deuterium}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1612.04741},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2016,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161204741A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{be8_stable,
   author = {{Adams}, F.~C. and {Grohs}, E.},
    title = "{Stellar helium burning in other universes: A solution to the triple alpha fine-tuning problem}",
  journal = {Astroparticle Physics},
archivePrefix = "arXiv",
   eprint = {1608.04690},
 keywords = {Fine-tuning, Multiverse, Stellar nucleosynthesis, Triple alpha},
     year = 2017,
    month = jan,
   volume = 87,
    pages = {40-54},
      doi = {10.1016/j.astropartphys.2016.12.002},
   adsurl = {http://adsabs.harvard.edu/abs/2017APh....87...40A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995PhRvD..52.3184K,
   author = {{Kosteleck{\'y}}, V.~A. and {Samuel}, S.},
    title = "{Neutrino oscillations in the early Universe with nonequilibrium neutrino distributions}",
  journal = {\prd},
   eprint = {hep-ph/9507427},
 keywords = {Elementary particle processes, Quark and lepton masses and mixing, Neutrino mass and mixing},
     year = 1995,
    month = sep,
   volume = 52,
    pages = {3184-3201},
      doi = {10.1103/PhysRevD.52.3184},
   adsurl = {http://adsabs.harvard.edu/abs/1995PhRvD..52.3184K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993NuPhB.406..423S,
   author = {{Sigl}, G. and {Raffelt}, G.},
    title = "{General kinetic description of relativistic mixed neutrinos}",
  journal = {Nuclear Physics B},
     year = 1993,
    month = sep,
   volume = 406,
    pages = {423-451},
      doi = {10.1016/0550-3213(93)90175-O},
   adsurl = {http://adsabs.harvard.edu/abs/1993NuPhB.406..423S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{PlanckXIII:2015,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and 
	{Arnaud}, M. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and 
	{Banday}, A.~J. and {Barreiro}, R.~B. and {Bartlett}, J.~G. and et al.},
    title = "{Planck 2015 results. XIII. Cosmological parameters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1502.01589},
 keywords = {cosmology: observations, cosmology: theory, cosmic background radiation, cosmological parameters},
     year = 2016,
    month = sep,
   volume = 594,
      eid = {A13},
    pages = {A13},
      doi = {10.1051/0004-6361/201525830},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...594A..13P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lep_trans,
   author = {{Grohs}, E. and {Fuller}, G.~M. and {Kishimoto}, C.~T. and {Paris}, M.~W.
	},
    title = "{Lepton asymmetry, neutrino spectral distortions, and big bang nucleosynthesis}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1612.01986},
     year = 2017,
    month = mar,
   volume = 95,
   number = 6,
      eid = {063503},
    pages = {063503},
      doi = {10.1103/PhysRevD.95.063503},
   adsurl = {http://adsabs.harvard.edu/abs/2017PhRvD..95f3503G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FFN:III,
   author = {{Fuller}, G.~M. and {Fowler}, W.~A. and {Newman}, M.~J.},
    title = "{Stellar weak interaction rates for intermediate mass nuclei. III - Rate tables for the free nucleons and nuclei with A = 21 to A = 60}",
  journal = {\apjs},
 keywords = {Astrophysics, Nuclear Astrophysics, Nuclei (Nuclear Physics), Nucleons, Stellar Evolution, Weak Energy Interactions, Electron Capture, Energy Dissipation, Neutrinos, Positrons, Tables (Data)},
     year = 1982,
    month = mar,
   volume = 48,
    pages = {279-319},
      doi = {10.1086/190779},
   adsurl = {http://adsabs.harvard.edu/abs/1982ApJS...48..279F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016JCAP...01..007B,
   author = {{Baumann}, D. and {Green}, D. and {Meyers}, J. and {Wallisch}, B.
	},
    title = "{Phases of new physics in the CMB}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1508.06342},
     year = 2016,
    month = jan,
   volume = 1,
      eid = {007},
    pages = {007},
      doi = {10.1088/1475-7516/2016/01/007},
   adsurl = {http://adsabs.harvard.edu/abs/2016JCAP...01..007B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014arXiv1412.1078S,
   author = {{Shimon}, M.},
    title = "{A Globally Unevolving Universe}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1412.1078},
 primaryClass = "physics.gen-ph",
 keywords = {Physics - General Physics, General Relativity and Quantum Cosmology},
     year = 2014,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1412.1078S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014arXiv1411.1071C,
   author = {{Cherry}, J.~F. and {Friedland}, A. and {Shoemaker}, I.~M.},
    title = "{Neutrino Portal Dark Matter: From Dwarf Galaxies to IceCube}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1411.1071},
 primaryClass = "hep-ph",
 keywords = {High Energy Physics - Phenomenology, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
     year = 2014,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1411.1071C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017arXiv170400626F,
   author = {{Forastieri}, F. and {Lattanzi}, M. and {Mangano}, G. and {Mirizzi}, A. and 
	{Natoli}, P. and {Saviano}, N.},
    title = "{Cosmic microwave background constraints on secret interactions among sterile neutrinos}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1704.00626},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, High Energy Physics - Phenomenology},
     year = 2017,
    month = apr,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170400626F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014PhRvD..90c5022F,
   author = {{Fradette}, A. and {Pospelov}, M. and {Pradler}, J. and {Ritz}, A.
	},
    title = "{Cosmological constraints on very dark photons}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1407.0993},
 primaryClass = "hep-ph",
 keywords = {Extensions of electroweak gauge sector, Models beyond the standard model, Other particles, Dark matter},
     year = 2014,
    month = aug,
   volume = 90,
   number = 3,
      eid = {035022},
    pages = {035022},
      doi = {10.1103/PhysRevD.90.035022},
   adsurl = {http://adsabs.harvard.edu/abs/2014PhRvD..90c5022F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006PhRvD..74j3509J,
   author = {{Jedamzik}, K.},
    title = "{Big bang nucleosynthesis constraints on hadronically and electromagnetically decaying relic neutral particles}",
  journal = {\prd},
   eprint = {hep-ph/0604251},
 keywords = {Particle-theory and field-theory models of the early Universe, Dark matter, Background radiations},
     year = 2006,
    month = nov,
   volume = 74,
   number = 10,
      eid = {103509},
    pages = {103509},
      doi = {10.1103/PhysRevD.74.103509},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhRvD..74j3509J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006NuPhB.756..100M,
   author = {{Mangano}, G. and {Miele}, G. and {Pastor}, S. and {Pinto}, T. and 
	{Pisanti}, O. and {Serpico}, P.~D.},
    title = "{Effects of non-standard neutrino electron interactions on relic neutrino decoupling}",
  journal = {Nuclear Physics B},
   eprint = {hep-ph/0607267},
     year = 2006,
    month = nov,
   volume = 756,
    pages = {100-116},
      doi = {10.1016/j.nuclphysb.2006.09.002},
   adsurl = {http://adsabs.harvard.edu/abs/2006NuPhB.756..100M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CF:88,
   author = {{Caughlan}, G.~R. and {Fowler}, W.~A.},
    title = "{Thermonuclear Reaction Rates V}",
  journal = {Atomic Data and Nuclear Data Tables},
     year = 1988,
   volume = 40,
    pages = {283},
      doi = {10.1016/0092-640X(88)90009-5},
   adsurl = {http://adsabs.harvard.edu/abs/1988ADNDT..40..283C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{xmelec,
   author = {{Grohs}, E. and {Fuller}, G.~M.},
    title = "{Insights into neutrino decoupling gleaned from considerations of the role of electron mass}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1706.03391},
 keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
     year = 2017,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170603391G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BRB:He3,
   author = {{Bania}, T.~M. and {Rood}, R.~T. and {Balser}, D.~S.},
    title = "{The cosmological density of baryons from observations of $^{3}$He$^{+}$ in the Milky Way}",
  journal = {\nat},
     year = 2002,
    month = jan,
   volume = 415,
    pages = {54-57},
      doi = {10.1038/415054a},
   adsurl = {http://adsabs.harvard.edu/abs/2002Natur.415...54B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AAGM:2017_vac,
   author = {{Adams}, F.~C. and {Alexander}, S. and {Grohs}, E. and {Mersini-Houghton}, L.
	},
    title = "{Constraints on vacuum energy from structure formation and Nucleosynthesis}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1701.03949},
     year = 2017,
    month = mar,
   volume = 3,
      eid = {021},
    pages = {021},
      doi = {10.1088/1475-7516/2017/03/021},
   adsurl = {http://adsabs.harvard.edu/abs/2017JCAP...03..021A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{HKP:2006_weakless,
   author = {{Harnik}, R. and {Kribs}, G.~D. and {Perez}, G.},
    title = "{A universe without weak interactions}",
  journal = {\prd},
   eprint = {hep-ph/0604027},
 keywords = {Models beyond the standard model},
     year = 2006,
    month = aug,
   volume = 74,
   number = 3,
      eid = {035006},
    pages = {035006},
      doi = {10.1103/PhysRevD.74.035006},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhRvD..74c5006H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{adams2016,
   author = {{Adams}, F.~C.},
    title = "{Constraints on alternate universes: stars and habitable planets with different fundamental constants}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1511.06958},
     year = 2016,
    month = feb,
   volume = 2,
      eid = {042},
    pages = {042},
      doi = {10.1088/1475-7516/2016/02/042},
   adsurl = {http://adsabs.harvard.edu/abs/2016JCAP...02..042A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{spirograph,
   author = {{Adams}, F.~C. and {Bloch}, A.~M.},
    title = "{Orbits in Extended Mass Distributions: General Results and the Spirographic Approximation}",
  journal = {\apj},
   eprint = {astro-ph/0504661},
 keywords = {Galaxies: Halos, Galaxies: Kinematics and Dynamics, Methods: Analytical, Stars: Formation, Stellar Dynamics},
     year = 2005,
    month = aug,
   volume = 629,
    pages = {204-218},
      doi = {10.1086/431455},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...629..204A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{adshu,
   author = {{Adams}, F.~C. and {Shu}, F.~H.},
    title = "{Ambipolar Diffusion In Molecular Cloud Cores and the Gravomagneto Catastrophe}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0708.4238},
 keywords = {Methods: Analytical, Magnetohydrodynamics: MHD, Stars: Formation},
     year = 2007,
    month = dec,
   volume = 671,
    pages = {497-517},
      doi = {10.1086/522925},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...671..497A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{bartip,
   author = {{Barrow}, J.~D. and {Tipler}, F.~J.},
    title = "{The anthropic cosmological principle}",
 keywords = {COSMOLOGY},
booktitle = "{The anthropic cosmological principle}",
     year = 1986,
   adsurl = {http://adsabs.harvard.edu/abs/1986acp..book.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{busha2005,
   author = {{Busha}, M.~T. and {Evrard}, A.~E. and {Adams}, F.~C. and {Wechsler}, R.~H.
	},
    title = "{The ultimate halo mass in a {$\Lambda$}CDM universe}",
  journal = {\mnras},
   eprint = {astro-ph/0412161},
 keywords = {cosmology: theory, dark matter, large-scale structure of Universe},
     year = 2005,
    month = oct,
   volume = 363,
    pages = {L11-L15},
      doi = {10.1111/j.1745-3933.2005.00072.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.363L..11B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{busha2007,
   author = {{Busha}, M.~T. and {Evrard}, A.~E. and {Adams}, F.~C.},
    title = "{The Asymptotic Form of Cosmic Structure: Small-Scale Power and Accretion History}",
  journal = {\apj},
   eprint = {astro-ph/0611930},
 keywords = {Cosmology: Theory, Cosmology: Dark Matter, Cosmology: Large-Scale Structure of Universe},
     year = 2007,
    month = aug,
   volume = 665,
    pages = {1-13},
      doi = {10.1086/518764},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...665....1B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{carr,
   author = {{Carr}, B.~J. and {Rees}, M.~J.},
    title = "{The anthropic principle and the structure of the physical world}",
  journal = {\nat},
 keywords = {Astrophysics, Constants, Cosmology, Fine Structure, Theoretical Physics, Universe, Asteroids, Black Holes (Astronomy), Dimensionless Numbers, Galaxies, Neutron Stars, Plancks Constant, Planets, Scaling Laws, White Dwarf Stars},
     year = 1979,
    month = apr,
   volume = 278,
    pages = {605-612},
      doi = {10.1038/278605a0},
   adsurl = {http://adsabs.harvard.edu/abs/1979Natur.278..605C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{carter,
   author = {{Carter}, B.},
    title = "{The Anthropic Principle and its Implications for Biological Evolution}",
  journal = {Philosophical Transactions of the Royal Society of London Series A},
     year = 1983,
    month = dec,
   volume = 310,
    pages = {347-363},
      doi = {10.1098/rsta.1983.0096},
   adsurl = {http://adsabs.harvard.edu/abs/1983RSPTA.310..347C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{galli,
   author = {{Galli}, D. and {Palla}, F.},
    title = "{The chemistry of the early Universe}",
  journal = {\aap},
   eprint = {astro-ph/9803315},
 keywords = {MOLECULAR PROCESSES, ATOMIC PROCESSES, EARLY UNIVERSE},
     year = 1998,
    month = jul,
   volume = 335,
    pages = {403-420},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...335..403G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hernquist,
   author = {{Hernquist}, L.},
    title = "{An analytical model for spherical galaxies and bulges}",
  journal = {\apj},
 keywords = {Computational Astrophysics, Elliptical Galaxies, Galactic Bulge, Galactic Structure, Astronomical Models, Astronomical Photometry, Brightness Distribution, Distribution Functions},
     year = 1990,
    month = jun,
   volume = 356,
    pages = {359-364},
      doi = {10.1086/168845},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...356..359H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hogan,
   author = {{Hogan}, C.~J.},
    title = "{Why the universe is just so}",
  journal = {Reviews of Modern Physics},
   eprint = {astro-ph/9909295},
 keywords = {Unified theories and models of strong and electroweak interactions, Unified theories and models of strong and electroweak interactions},
     year = 2000,
    month = oct,
   volume = 72,
    pages = {1149-1161},
      doi = {10.1103/RevModPhys.72.1149},
   adsurl = {http://adsabs.harvard.edu/abs/2000RvMP...72.1149H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{nfw,
   author = {{Navarro}, J.~F. and {Frenk}, C.~S. and {White}, S.~D.~M.},
    title = "{A Universal Density Profile from Hierarchical Clustering}",
  journal = {\apj},
   eprint = {astro-ph/9611107},
 keywords = {Cosmology: Theory, Cosmology: Dark Matter, Galaxies: Halos, Methods: Numerical},
     year = 1997,
    month = dec,
   volume = 490,
    pages = {493-508},
      doi = {10.1086/304888},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...490..493N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{reessix,
   author = {{Rees}, M.},
    title = "{Just six numbers : the deep forces that shape the universe}",
booktitle = {Just six numbers : the deep forces that shape the universe / Martin Rees.~New York : Basic Books, c2000.},
     year = 2000,
   adsurl = {http://adsabs.harvard.edu/abs/2000jsn..book.....R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sellwoodmag,
   author = {{Sellwood}, J.~A. and {McGaugh}, S.~S.},
    title = "{The Compression of Dark Matter Halos by Baryonic Infall}",
  journal = {\apj},
   eprint = {astro-ph/0507589},
 keywords = {Cosmology: Dark Matter, Galaxies: Formation, Galaxies: Halos, Galaxies: Kinematics and Dynamics},
     year = 2005,
    month = nov,
   volume = 634,
    pages = {70-76},
      doi = {10.1086/491731},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...634...70S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{ST:1983_co,
   author = {{Shapiro}, S.~L. and {Teukolsky}, S.~A.},
    title = "{Black holes, white dwarfs, and neutron stars: The physics of compact objects}",
 keywords = {Astrophysics, Black Holes (Astronomy), Neutron Stars, Textbooks, White Dwarf Stars, Accretion Disks, Elementary Particle Interactions, Gravitational Collapse, Gravitational Waves, Magnetohydrodynamic Stability, Nuclear Interactions, Pulsars, Relativity, Stellar Evolution, Stellar Magnetic Fields, Stellar Rotation, Stellar Temperature, Supermassive Stars, Supernovae, X Ray Sources},
booktitle = {Research supported by the National Science Foundation.~New York, Wiley-Interscience, 1983, 663 p.},
     year = 1983,
   adsurl = {http://adsabs.harvard.edu/abs/1983bhwd.book.....S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shu77,
   author = {{Shu}, F.~H.},
    title = "{Self-similar collapse of isothermal spheres and star formation}",
  journal = {\apj},
 keywords = {Density Distribution, Gravitational Collapse, Isothermal Flow, Protostars, Star Formation, Stellar Structure, Critical Point, Runge-Kutta Method, Similarity Theorem, Steady State, Stellar Envelopes},
     year = 1977,
    month = jun,
   volume = 214,
    pages = {488-497},
      doi = {10.1086/155274},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...214..488S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sal87,
   author = {{Shu}, F.~H. and {Adams}, F.~C. and {Lizano}, S.},
    title = "{Star formation in molecular clouds - Observation and theory}",
  journal = {\araa},
 keywords = {Astrophysics, Molecular Clouds, Star Formation, Stellar Models, Astronomical Maps, Binary Stars, Gravitational Collapse, Protostars, Star Clusters, Stellar Mass},
     year = 1987,
   volume = 25,
    pages = {23-81},
      doi = {10.1146/annurev.aa.25.090187.000323},
   adsurl = {http://adsabs.harvard.edu/abs/1987ARA%26A..25...23S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tegmark,
   author = {{Tegmark}, M. and {Aguirre}, A. and {Rees}, M.~J. and {Wilczek}, F.
	},
    title = "{Dimensionless constants, cosmology, and other dark matters}",
  journal = {\prd},
   eprint = {astro-ph/0511774},
 keywords = {Observational cosmology},
     year = 2006,
    month = jan,
   volume = 73,
   number = 2,
      eid = {023505},
    pages = {023505},
      doi = {10.1103/PhysRevD.73.023505},
   adsurl = {http://adsabs.harvard.edu/abs/2006PhRvD..73b3505T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tegrees,
   author = {{Tegmark}, M. and {Rees}, M.~J.},
    title = "{Why Is the Cosmic Microwave Background Fluctuation Level 10$^{-5}$?}",
  journal = {\apj},
   eprint = {astro-ph/9709058},
 keywords = {Cosmology: Theory, Cosmology: Large-Scale Structure of Universe},
     year = 1998,
    month = may,
   volume = 499,
    pages = {526-532},
      doi = {10.1086/305673},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...499..526T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{whiterees,
   author = {{White}, S.~D.~M. and {Rees}, M.~J.},
    title = "{Core condensation in heavy halos - A two-stage theory for galaxy formation and clustering}",
  journal = {\mnras},
 keywords = {Astronomical Models, Galactic Clusters, Galactic Evolution, Galactic Nuclei, Gravitational Effects, Halos, Critical Mass, Dark Matter, Dynamic Models, Interstellar Gas, Luminosity, Many Body Problem, Red Shift},
     year = 1978,
    month = may,
   volume = 183,
    pages = {341-358},
      doi = {10.1093/mnras/183.3.341},
   adsurl = {http://adsabs.harvard.edu/abs/1978MNRAS.183..341W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MESA:2011,
   author = {{Paxton}, B. and {Bildsten}, L. and {Dotter}, A. and {Herwig}, F. and 
	{Lesaffre}, P. and {Timmes}, F.},
    title = "{Modules for Experiments in Stellar Astrophysics (MESA)}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1009.1622},
 primaryClass = "astro-ph.SR",
 keywords = {methods: numerical, stars: evolution, stars: general},
     year = 2011,
    month = jan,
   volume = 192,
      eid = {3},
    pages = {3},
      doi = {10.1088/0067-0049/192/1/3},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..192....3P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MESA:2013,
   author = {{Paxton}, B. and {Cantiello}, M. and {Arras}, P. and {Bildsten}, L. and 
	{Brown}, E.~F. and {Dotter}, A. and {Mankovich}, C. and {Montgomery}, M.~H. and 
	{Stello}, D. and {Timmes}, F.~X. and {Townsend}, R.},
    title = "{Modules for Experiments in Stellar Astrophysics (MESA): Planets, Oscillations, Rotation, and Massive Stars}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1301.0319},
 primaryClass = "astro-ph.SR",
 keywords = {asteroseismology, methods: numerical, planets and satellites: physical evolution, stars: evolution, stars: massive, stars: rotation},
     year = 2013,
    month = sep,
   volume = 208,
      eid = {4},
    pages = {4},
      doi = {10.1088/0067-0049/208/1/4},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJS..208....4P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999A&A...342..426G,
   author = {{Gustafsson}, B. and {Karlsson}, T. and {Olsson}, E. and {Edvardsson}, B. and 
	{Ryde}, N.},
    title = "{The origin of carbon, investigated by spectral analysis of solar-type stars in the Galactic Disk}",
  journal = {\aap},
   eprint = {astro-ph/9811303},
 keywords = {GALAXIES: EVOLUTION, GALAXY: ABUNDANCES, STARS: ABUNDANCES, NUCLEAR REACTIONS, NUCLEOSYNTHESIS, ABUNDANCES},
     year = 1999,
    month = feb,
   volume = 342,
    pages = {426-439},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...342..426G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...541..660H,
   author = {{Henry}, R.~B.~C. and {Edmunds}, M.~G. and {K{\"o}ppen}, J.},
    title = "{On the Cosmic Origins of Carbon and Nitrogen}",
  journal = {\apj},
   eprint = {astro-ph/0004299},
 keywords = {Galaxies: Abundances, Galaxies: Evolution, Galaxy: Abundances, Galaxy: Evolution, ISM: Abundances, Nuclear Reactions, Nucleosynthesis, Abundances},
     year = 2000,
    month = oct,
   volume = 541,
    pages = {660-674},
      doi = {10.1086/309471},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...541..660H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000A&A...361L...1P,
   author = {{P{\'e}quignot}, D. and {Walsh}, J.~R. and {Zijlstra}, A.~A. and 
	{Dudziak}, G.},
    title = "{Third-dredge-up oxygen in planetary nebulae}",
  journal = {\aap},
   eprint = {astro-ph/0008443},
 keywords = {NUCLEAR REACTIONS, NUCLEOSYNTHESIS, ABUNDANCES, ISM: PLANETARY NEBULAE: GENERAL, GALAXIES: DWARF, GALAXIES: INDIVIDUAL: SAGITTARIUS},
     year = 2000,
    month = sep,
   volume = 361,
    pages = {L1-L4},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...361L...1P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJS..125..439I,
   author = {{Iwamoto}, K. and {Brachwitz}, F. and {Nomoto}, K. and {Kishimoto}, N. and 
	{Umeda}, H. and {Hix}, W.~R. and {Thielemann}, F.-K.},
    title = "{Nucleosynthesis in Chandrasekhar Mass Models for Type IA Supernovae and Constraints on Progenitor Systems and Burning-Front Propagation}",
  journal = {\apjs},
   eprint = {astro-ph/0002337},
 keywords = {NUCLEAR REACTIONS, NUCLEOSYNTHESIS, ABUNDANCES, STARS: INTERIORS, SUPERNOVAE: GENERAL, Nuclear Reactions, Nucleosynthesis, Abundances, Stars: Interiors, supernovae: general},
     year = 1999,
    month = dec,
   volume = 125,
    pages = {439-462},
      doi = {10.1086/313278},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJS..125..439I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...757..192J,
   author = {{Johnson}, T.~V. and {Mousis}, O. and {Lunine}, J.~I. and {Madhusudhan}, N.
	},
    title = "{Planetesimal Compositions in Exoplanet Systems}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1208.3289},
 primaryClass = "astro-ph.EP",
 keywords = {planets and satellites: formation, planets and satellites: general, protoplanetary disks},
     year = 2012,
    month = oct,
   volume = 757,
      eid = {192},
    pages = {192},
      doi = {10.1088/0004-637X/757/2/192},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...757..192J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ASSP...16..379L,
   author = {{Lodders}, K.},
    title = "{Solar System Abundances of the Elements}",
  journal = {Astrophysics and Space Science Proceedings},
archivePrefix = "arXiv",
   eprint = {1010.2746},
 primaryClass = "astro-ph.SR",
 keywords = {Physics},
     year = 2010,
   volume = 16,
    pages = {379},
      doi = {10.1007/978-3-642-10352-0_8},
   adsurl = {http://adsabs.harvard.edu/abs/2010ASSP...16..379L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article {NYAS:NYAS736,
author = {Thomson, John F.},
title = {PHYSIOLOGICAL EFFECTS OF D2O IN MAMMALS*},
journal = {Annals of the New York Academy of Sciences},
volume = {84},
number = {16},
publisher = {Blackwell Publishing Ltd},
issn = {1749-6632},
url = {http://dx.doi.org/10.1111/j.1749-6632.1960.tb39105.x},
doi = {10.1111/j.1749-6632.1960.tb39105.x},
pages = {736--744},
year = {1960},
}

@Article{F19757100980,
author ="Rao, C. N. Ramachandra",
title  ="Effect of deuteration on hydrogen bonds",
journal  ="J. Chem. Soc.{,} Faraday Trans. 1",
year  ="1975",
volume  ="71",
issue  ="0",
pages  ="980-983",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/F19757100980",
url  ="http://dx.doi.org/10.1039/F19757100980"
}

@article{KBD:1999_D2O,
author = {J Kushner, D and Baker, Alison and G Dunstall, T},
year = {1999},
month = {03},
pages = {79-88},
title = {Pharmacological use and perspectives of heavy water and deuterated compounds},
volume = {77},
booktitle = {Canadian journal of physiology and pharmacology}
}

@ARTICLE{2014ApJ...787L...2Y,
   author = {{Yang}, J. and {Bou{\'e}}, G. and {Fabrycky}, D.~C. and {Abbot}, D.~S.
	},
    title = "{Strong Dependence of the Inner Edge of the Habitable Zone on Planetary Rotation Rate}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1404.4992},
 primaryClass = "astro-ph.EP",
 keywords = {astrobiology, planets and satellites: atmospheres, planets and satellites: detection },
     year = 2014,
    month = may,
   volume = 787,
      eid = {L2},
    pages = {L2},
      doi = {10.1088/2041-8205/787/1/L2},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...787L...2Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006hep.ph....9050C,
   author = {{Clavelli}, L. and {White}, III, R.~E.},
    title = "{Problems in a weakless universe}",
  journal = {ArXiv High Energy Physics - Phenomenology e-prints},
   eprint = {hep-ph/0609050},
 keywords = {High Energy Physics - Phenomenology},
     year = 2006,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2006hep.ph....9050C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011PhRvD..83k5020G,
   author = {{Gedalia}, O. and {Jenkins}, A. and {Perez}, G.},
    title = "{Why do we observe a weak force? The hierarchy problem in the multiverse}",
  journal = {\prd},
archivePrefix = "arXiv",
   eprint = {1010.2626},
 primaryClass = "hep-ph",
 keywords = {Models beyond the standard model, Cosmology},
     year = 2011,
    month = jun,
   volume = 83,
   number = 11,
      eid = {115020},
    pages = {115020},
      doi = {10.1103/PhysRevD.83.115020},
   adsurl = {http://adsabs.harvard.edu/abs/2011PhRvD..83k5020G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012arXiv1207.4861G,
   author = {{Giudice}, G.~F. and {Perez}, G. and {Soreq}, Y.},
    title = "{Flavor Beyond the Standard Universe}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1207.4861},
 primaryClass = "hep-ph",
 keywords = {High Energy Physics - Phenomenology},
     year = 2012,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2012arXiv1207.4861G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2016JPhCS.665a2001C,
   author = {{Coc}, A.},
    title = "{Primordial Nucleosynthesis}",
booktitle = {Journal of Physics Conference Series},
     year = 2016,
   series = {Journal of Physics Conference Series},
   volume = 665,
archivePrefix = "arXiv",
   eprint = {1609.06048},
    month = jan,
      eid = {012001},
    pages = {012001},
      doi = {10.1088/1742-6596/665/1/012001},
   adsurl = {http://adsabs.harvard.edu/abs/2016JPhCS.665a2001C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015JCAP...12..050B,
   author = {{Barnes}, L.~A.},
    title = "{Binding the diproton in stars: anthropic limits on the strength of gravity}",
  journal = {\jcap},
archivePrefix = "arXiv",
   eprint = {1512.06090},
 primaryClass = "astro-ph.SR",
     year = 2015,
    month = dec,
   volume = 12,
      eid = {050},
    pages = {050},
      doi = {10.1088/1475-7516/2015/12/050},
   adsurl = {http://adsabs.harvard.edu/abs/2015JCAP...12..050B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1950PThPh...5..224H,
   author = {{Hayashi}, C.},
    title = "{Proton-Neutron Concentration Ratio in the Expanding Universe at the Stages preceding the Formation of the Elements}",
  journal = {Progress of Theoretical Physics},
     year = 1950,
    month = mar,
   volume = 5,
    pages = {224-235},
      doi = {10.1143/ptp/5.2.224},
   adsurl = {http://adsabs.harvard.edu/abs/1950PThPh...5..224H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017arXiv171100314R,
   author = {{Rezzolla}, L. and {Most}, E.~R. and {Weih}, L.~R.},
    title = "{Using gravitational-wave observations and quasi-universal relations to constrain the maximum mass of neutron stars}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1711.00314},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena, General Relativity and Quantum Cosmology},
     year = 2017,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv171100314R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{hansen,
   author = {{Hansen}, C.~J. and {Kawaler}, S.~D.},
    title = "{Stellar Interiors. Physical Principles, Structure, and Evolution.}",
 keywords = {STELLAR STRUCTURE, EVOLUTION, STELLAR INTERIORS, STELLAR STRUCTURE, STELLAR EVOLUTION},
booktitle = {``Stellar Interiors.~ Physical Principles, Structure, and Evolution, XIII, 445 pp.~84 figs.~3 1/2'' diskette.~ Springer-Verlag Berlin Heidelberg New York.~ Also Astronomy and Astrophysics Library``},
     year = 1994,
    pages = {84},
   adsurl = {http://adsabs.harvard.edu/abs/1994sipp.book.....H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{kippenhahn,
   author = {{Kippenhahn}, R. and {Weigert}, A.},
    title = "{Stellar Structure and Evolution}",
 keywords = {STELLAR STRUCTURE, STELLAR EVOLUTION},
booktitle = {Stellar Structure and Evolution, XVI, 468 pp.~192 figs..~ Springer-Verlag Berlin Heidelberg New York.~Also Astronomy and Astrophysics Library},
     year = 1990,
    pages = {192},
   adsurl = {http://adsabs.harvard.edu/abs/1990sse..book.....K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hayashione,
   author = {{Hayashi}, C.},
    title = "{Stellar evolution in early phases of gravitational contraction.}",
  journal = {\pasj},
     year = 1961,
   volume = 13,
   adsurl = {http://adsabs.harvard.edu/abs/1961PASJ...13..450H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hayashitwo,
   author = {{Hayashi}, C. and {Hoshi}, R.},
    title = "{The Outer Envelope of Giant Stars with Surface Convection Zone}",
  journal = {\pasj},
     year = 1961,
   volume = 13,
    pages = {442-449},
   adsurl = {http://adsabs.harvard.edu/abs/1961PASJ...13..442H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

